ECI-Cache: A High-Endurance and Cost-Efficient I/O Caching Scheme for Virtualized Platforms

In recent years, high interest in using Virtual Machines (VMs) in data centers and Cloud computing has significantly increased the demand for high-performance data storage systems. Recent studies suggest using SSDs as a caching layer for HDD-based storage subsystems in virtualization platforms. Such studies neglect to address the endurance and cost of SSDs, which can significantly affect the efficiency of I/O caching. Moreover, previous studies only configure the cache size to provide the required performance level for each VM, while neglecting other important parameters such as cache write policy and request type, which can adversely affect both performance-per-cost and endurance. In this paper, we present a new high-Endurance and Cost-efficient I/O Caching (ECI-Cache) scheme for virtualized platforms, which can significantly improve both the performance-per-cost and endurance of storage subsystems as opposed to previously proposed I/O caching schemes. Unlike traditional I/O caching schemes which allocate cache size only based on reuse distance of accesses, we propose a new metric, Useful Reuse Distance (URD), which considers the request type in reuse distance calculation, resulting in improved performance-per-cost and endurance for the SSD cache. Via online characterization of workloads and using URD, ECI-Cache partitions the SSD cache across VMs and is able to dynamically adjust the cache size and write policy for each VM. To evaluate the proposed scheme, we have implemented ECI-Cache in an open source hypervisor, QEMU (version 2.8.0), on a server running the CentOS 7 operating system (kernel version 3.10.0-327). Experimental results show that our proposed scheme improves the performance, performance-per-cost, and endurance of the SSD cache by 17%, 30% and 65%, respectively, compared to the state-of-the-art dynamic cache partitioning scheme.

==> Centaur_size_no_limit_table.tex <==
\begin{center}

	\tiny
%		
	\begin{longtable}{m{0.028\textwidth}|m{0.028\textwidth}m{0.035\textwidth}m{0.035\textwidth}m{0.035\textwidth}m{0.035\textwidth}m{0.035\textwidth}m{0.035\textwidth}m{0.035\textwidth}m{0.028\textwidth}m{0.035\textwidth}m{0.035\textwidth}m{0.035\textwidth}m{0.035\textwidth}m{0.035\textwidth}m{0.035\textwidth}m{0.038\textwidth}|m{0.035\textwidth}} 
\caption{Centaur size estimation in non-limited SSD‌ cache space.}\label{table:Centaur_non_limit}\\
		\hline
		time (min) & VM0 & VM1 & VM2 & VM3 & VM4 & VM5 & VM6 & VM7 & VM8 & VM9 & VM10 & VM11 & VM12 & VM13 & VM14 & VM15 & csum\\ \hline
10 & 2,832 & 2,072 & 1,971 & 4,203 & 1,166 & 2,207 & 1,434 & 2,557 & 2,602 & 8,396 & 6,084 & 1,606 & 1,635 & 2,394 & 2,367 & 4,511 & 48,037\\
20 & 4,489 & 4,530 & 6,542 & 5,892 & 2,401 & 2,784 & 4,392 & 3,424 & 3,739 & 10,611 & 13,468 & 2,684 & 5,426 & 4,740 & 11,235 & 4,507 & 90,864\\
30 & 5,374 & 11,230 & 7,187 & 6,854 & 2,940 & 4,889 & 5,764 & 3,529 & 7,720 & 16,327 & 25,290 & 3,803 & 6,721 & 13,564 & 11,235 & 17,353 & 149,780\\
40 & 7,129 & 11,562 & 8,043 & 8,245 & 2,940 & 7,204 & 15,256 & 4,120 & 9,452 & 21,457 & 36,333 & 5,289 & 11,185 & 20,936 & 11,235 & 15,949 & 196,335\\
50 & 8,911 & 21,942 & 8,064 & 9,421 & 3,019 & 8,888 & 23,395 & 5,977 & 9,452 & 21,442 & 41,436 & 6,078 & 16,153 & 31,433 & 11,234 & 15,940 & 242,785\\
60 & 9,820 & 22,046 & 9,385 & 9,420 & 2,986 & 9,117 & 31,644 & 6,170 & 11,194 & 31,283 & 45,112 & 8,137 & 26,409 & 33,726 & 11,234 & 17,353 & 285,036\\
70 & 9,861 & 56,835 & 9,641 & 11,440 & 3,375 & 10,168 & 33,166 & 6,326 & 11,810 & 40,401 & 52,972 & 8,597 & 32,001 & 34,993 & 11,234 & 49,137 & 381,957\\
80 & 10,587 & 65,409 & 11,155 & 12,246 & 3,387 & 11,401 & 33,748 & 7,041 & 13,289 & 41,780 & 53,616 & 8,304 & 41,192 & 35,293 & 11,233 & 67,667 & 427,348\\
90 & 12,663 & 68,197 & 11,175 & 13,777 & 3,377 & 12,742 & 35,750 & 7,309 & 15,507 & 45,558 & 52,780 & 8,671 & 45,037 & 35,620 & 11,235 & 67,811 & 447,209\\
100 & 12,748 & 71,577 & 13,707 & 13,777 & 3,760 & 12,727 & 36,553 & 7,341 & 16,214 & 47,046 & 52,694 & 8,788 & 61,379 & 39,182 & 11,233 & 68,169 & 476,895\\
110 & 14,021 & 73,331 & 14,268 & 13,777 & 3,787 & 14,080 & 37,914 & 8,083 & 17,185 & 47,047 & 52,694 & 11,892 & 63,467 & 40,060 & 11,230 & 78,990 & 501,826\\
120 & 16,111 & 73,324 & 14,372 & 14,831 & 4,296 & 13,627 & 39,346 & 7,826 & 17,859 & 53,418 & 54,499 & 12,542 & 63,511 & 40,571 & 11,231 & 82,962 & 520,326\\
130 & 17,990 & 75,061 & 14,375 & 16,214 & 5,323 & 15,280 & 40,413 & 8,077 & 19,993 & 54,545 & 72,428 & 12,542 & 63,854 & 41,690 & 11,230 & 78,985 & 548,000\\
140 & 18,245 & 75,056 & 15,715 & 16,918 & 5,199 & 15,280 & 42,245 & 8,786 & 20,049 & 57,086 & 72,937 & 12,542 & 66,833 & 44,067 & 11,235 & 78,985 & 561,178\\
150 & 19,997 & 76,194 & 15,843 & 16,916 & 5,215 & 16,663 & 45,829 & 8,786 & 21,591 & 58,181 & 81,641 & 14,796 & 67,149 & 47,096 & 11,230 & 100,675 & 607,802\\
160 & 21,228 & 77,398 & 15,856 & 18,328 & 5,215 & 16,604 & 48,909 & 8,279 & 22,709 & 61,281 & 83,401 & 14,797 & 71,616 & 47,794 & 130,834 & 96,548 & 740,797\\
170 & 21,800 & 0 & 15,862 & 18,773 & 5,546 & 18,636 & 49,562 & 8,279 & 22,768 & 61,770 & 94,006 & 15,043 & 72,365 & 47,818 & 132,739 & 96,623 & 681,590\\
180 & 22,181 & 0 & 17,052 & 19,457 & 6,101 & 18,642 & 48,904 & 8,786 & 23,579 & 64,777 & 97,021 & 15,553 & 72,376 & 47,810 & 141,448 & 100,675 & 704,362\\
190 & 22,311 & 0 & 17,153 & 20,715 & 6,101 & 18,634 & 49,455 & 8,395 & 24,037 & 61,767 & 107,394 & 15,505 & 74,580 & 47,787 & 132,342 & 113,789 & 719,965\\
200 & 22,317 & 0 & 17,150 & 21,009 & 6,021 & 18,654 & 52,987 & 9,627 & 24,052 & 61,767 & 110,258 & 16,031 & 75,233 & 47,806 & 151,893 & 97,270 & 732,075\\
210 & 24,319 & 0 & 25,053 & 22,116 & 6,037 & 20,583 & 54,710 & 9,408 & 25,555 & 66,508 & 110,447 & 17,901 & 75,004 & 47,813 & 0 & 98,848 & 604,302\\
220 & 24,342 & 0 & 27,777 & 22,616 & 6,039 & 20,539 & 54,744 & 10,983 & 25,518 & 62,822 & 111,359 & 17,911 & 75,023 & 47,794 & 0 & 96,556 & 604,023\\
230 & 24,340 & 0 & 40,636 & 22,776 & 6,101 & 20,582 & 56,685 & 10,961 & 26,164 & 64,815 & 111,359 & 17,955 & 79,182 & 48,986 & 0 & 98,002 & 628,544\\
240 & 25,217 & 0 & 46,918 & 23,106 & 6,302 & 20,533 & 56,657 & 9,756 & 26,608 & 62,824 & 111,359 & 17,936 & 79,178 & 48,985 & 0 & 100,956 & 636,335\\
250 & 25,227 & 0 & 58,106 & 24,480 & 6,023 & 21,468 & 56,663 & 9,756 & 26,893 & 70,002 & 111,488 & 17,955 & 79,179 & 51,128 & 0 & 96,978 & 655,346\\
260 & 26,840 & 0 & 68,202 & 24,480 & 6,037 & 21,722 & 57,750 & 9,661 & 26,900 & 66,508 & 111,487 & 19,609 & 79,193 & 51,399 & 0 & 113,789 & 683,577\\
270 & 27,357 & 0 & 77,672 & 25,042 & 6,416 & 21,751 & 57,763 & 9,627 & 27,649 & 63,078 & 111,359 & 19,610 & 80,946 & 53,840 & 0 & 96,978 & 679,088\\
280 & 27,458 & 0 & 86,538 & 25,064 & 6,438 & 23,109 & 58,813 & 11,140 & 27,635 & 63,009 & 111,359 & 19,607 & 81,093 & 55,927 & 0 & 140,807 & 737,997\\
290 & 27,536 & 0 & 94,335 & 25,650 & 6,432 & 23,137 & 58,813 & 10,331 & 27,981 & 71,688 & 138,973 & 19,608 & 81,090 & 55,926 & 0 & 138,936 & 780,436\\
300 & 27,689 & 0 & 107,137 & 25,678 & 6,511 & 22,498 & 59,125 & 9,635 & 27,954 & 67,445 & 166,236 & 21,076 & 81,111 & 57,203 & 0 & 160,271 & 839,569\\
310 & 27,604 & 0 & 112,427 & 26,117 & 6,498 & 23,932 & 60,604 & 10,381 & 28,954 & 71,723 & 172,389 & 21,089 & 81,296 & 57,717 & 0 & 130,137 & 830,868\\
320 & 28,849 & 0 & 121,378 & 26,126 & 6,547 & 23,792 & 60,224 & 10,981 & 28,593 & 71,813 & 178,971 & 21,148 & 84,025 & 57,784 & 0 & 167,667 & 887,898\\
330 & 29,268 & 0 & 137,853 & 26,563 & 6,469 & 23,833 & 60,528 & 9,635 & 28,624 & 74,389 & 181,801 & 21,143 & 83,998 & 58,738 & 0 & 148,778 & 891,620\\
340 & 29,243 & 0 & 148,780 & 27,077 & 6,507 & 23,937 & 60,616 & 9,635 & 29,535 & 71,749 & 185,126 & 21,149 & 84,484 & 58,738 & 0 & 167,667 & 924,243\\
350 & 29,268 & 0 & 159,082 & 27,832 & 6,287 & 24,636 & 61,729 & 10,381 & 29,689 & 71,792 & 188,578 & 21,154 & 84,532 & 61,348 & 0 & 219,337 & 995,645\\
360 & 29,276 & 0 & 150,511 & 28,289 & 6,434 & 24,642 & 61,773 & 10,023 & 29,701 & 73,839 & 191,541 & 22,243 & 86,692 & 62,438 & 0 & 156,662 & 934,064\\
370 & 30,295 & 0 & 163,938 & 28,677 & 6,434 & 24,063 & 61,837 & 10,981 & 30,598 & 73,714 & 197,329 & 22,241 & 93,059 & 62,213 & 0 & 219,337 & 1,024,716\\
380 & 30,342 & 0 & 185,631 & 28,677 & 6,483 & 24,064 & 62,538 & 9,620 & 30,283 & 77,273 & 197,859 & 23,433 & 101,260 & 62,709 & 0 & 191,951 & 1,032,123\\
390 & 30,342 & 0 & 196,197 & 29,053 & 6,434 & 25,217 & 62,397 & 10,985 & 30,598 & 74,389 & 205,471 & 24,416 & 110,052 & 64,393 & 0 & 252,659 & 1,122,603\\
400 & 30,333 & 0 & 204,712 & 29,113 & 6,507 & 24,677 & 62,547 & 12,675 & 31,092 & 82,471 & 208,855 & 25,723 & 115,951 & 64,860 & 0 & 245,658 & 1,145,174\\
410 & 31,230 & 0 & 207,607 & 29,528 & 6,455 & 24,839 & 62,554 & 11,201 & 31,057 & 82,471 & 211,152 & 28,083 & 130,613 & 72,389 & 0 & 252,658 & 1,181,837\\
420 & 31,704 & 0 & 215,142 & 29,324 & 6,507 & 26,047 & 66,618 & 12,265 & 31,707 & 85,568 & 211,191 & 28,083 & 137,174 & 80,585 & 0 & 197,970 & 1,159,885\\
430 & 31,764 & 0 & 237,896 & 29,526 & 6,701 & 25,423 & 74,599 & 10,961 & 31,693 & 87,969 & 215,046 & 28,057 & 139,776 & 87,788 & 0 & 216,363 & 1,223,562\\
440 & 31,765 & 0 & 238,025 & 30,109 & 6,432 & 25,414 & 83,743 & 12,668 & 31,705 & 87,917 & 215,046 & 28,051 & 139,656 & 91,193 & 0 & 359,362 & 1,381,086\\
450 & 31,937 & 0 & 241,975 & 30,069 & 6,111 & 26,043 & 85,270 & 11,775 & 31,706 & 90,042 & 229,608 & 28,930 & 151,771 & 91,327 & 0 & 263,873 & 1,320,437\\
460 & 32,645 & 0 & 254,905 & 33,935 & 6,515 & 25,926 & 85,276 & 11,193 & 32,022 & 87,406 & 228,465 & 29,405 & 152,044 & 92,212 & 0 & 318,922 & 1,390,871\\
470 & 32,736 & 0 & 257,629 & 36,043 & 6,515 & 26,037 & 85,282 & 10,381 & 31,927 & 87,412 & 228,986 & 28,952 & 167,602 & 92,218 & 0 & 335,927 & 1,427,647\\
480 & 32,790 & 0 & 271,759 & 37,515 & 6,515 & 26,046 & 85,282 & 12,675 & 32,257 & 93,769 & 229,244 & 29,422 & 170,033 & 92,217 & 0 & 368,234 & 1,487,758\\
490 & 32,730 & 0 & 296,602 & 36,635 & 6,604 & 26,793 & 85,276 & 11,990 & 32,399 & 90,042 & 234,157 & 30,573 & 184,247 & 95,326 & 0 & 245,658 & 1,409,032\\
500 & 32,726 & 0 & 303,176 & 37,811 & 6,220 & 27,115 & 87,338 & 14,507 & 32,255 & 90,054 & 233,960 & 30,505 & 192,573 & 95,223 & 0 & 252,659 & 1,436,122\\
510 & 32,793 & 0 & 308,298 & 38,719 & 6,438 & 26,814 & 85,281 & 14,492 & 32,418 & 90,410 & 235,833 & 32,292 & 199,189 & 95,223 & 0 & 325,524 & 1,523,724\\
520 & 33,407 & 0 & 305,972 & 38,715 & 6,075 & 31,150 & 87,335 & 17,131 & 33,066 & 90,244 & 244,492 & 32,293 & 204,967 & 95,323 & 0 & 250,512 & 1,470,682\\
530 & 33,413 & 0 & 329,184 & 38,719 & 6,498 & 44,733 & 85,282 & 14,114 & 33,725 & 92,809 & 255,008 & 32,620 & 211,642 & 95,227 & 0 & 381,961 & 1,654,935\\
540 & 34,036 & 0 & 346,259 & 38,719 & 6,075 & 53,560 & 87,462 & 12,852 & 33,066 & 93,670 & 260,240 & 33,897 & 215,097 & 95,223 & 0 & 388,312 & 1,698,468\\
550 & 33,416 & 0 & 357,716 & 38,717 & 6,483 & 61,698 & 87,342 & 18,399 & 33,161 & 93,427 & 265,556 & 33,328 & 215,097 & 95,222 & 0 & 284,507 & 1,624,069\\
560 & 33,905 & 0 & 363,293 & 40,628 & 6,430 & 72,221 & 90,424 & 17,106 & 33,351 & 93,422 & 273,558 & 33,904 & 215,035 & 95,230 & 0 & 390,922 & 1,759,429\\
570 & 34,083 & 0 & 376,735 & 39,228 & 6,351 & 81,698 & 91,206 & 15,072 & 33,704 & 93,428 & 273,279 & 33,974 & 217,742 & 95,250 & 0 & 391,485 & 1,783,235\\
580 & 33,991 & 0 & 376,735 & 39,819 & 6,284 & 84,042 & 90,628 & 19,527 & 33,717 & 93,429 & 273,283 & 33,975 & 219,048 & 95,417 & 0 & 309,089 & 1,708,984\\
590 & 34,100 & 0 & 389,982 & 41,086 & 6,110 & 84,170 & 90,422 & 19,397 & 34,340 & 93,426 & 273,714 & 33,974 & 220,365 & 95,311 & 0 & 445,264 & 1,861,661\\
600 & 34,700 & 0 & 393,125 & 41,598 & 6,284 & 88,910 & 90,696 & 19,497 & 34,345 & 93,722 & 273,661 & 34,828 & 222,712 & 95,227 & 0 & 359,362 & 1,788,667\\
610 & 34,634 & 0 & 418,620 & 40,628 & 0 & 105,871 & 92,357 & 19,495 & 34,989 & 101,785 & 279,567 & 34,668 & 223,114 & 95,419 & 0 & 459,845 & 1,940,992\\
620 & 35,238 & 0 & 426,162 & 41,336 & 0 & 108,485 & 90,672 & 19,513 & 35,014 & 101,787 & 281,381 & 34,491 & 223,207 & 98,749 & 0 & 385,567 & 1,881,602\\
630 & 35,828 & 0 & 433,315 & 41,458 & 0 & 107,988 & 90,422 & 14,492 & 35,039 & 101,785 & 287,353 & 34,829 & 223,172 & 98,740 & 0 & 381,611 & 1,886,032\\
640 & 35,994 & 0 & 443,773 & 41,657 & 0 & 108,479 & 90,549 & 14,503 & 35,492 & 101,787 & 287,402 & 34,450 & 223,928 & 98,610 & 0 & 440,568 & 1,957,192\\
650 & 36,530 & 0 & 445,140 & 41,756 & 0 & 109,019 & 90,567 & 18,353 & 35,039 & 101,787 & 287,392 & 34,450 & 224,292 & 98,734 & 0 & 452,309 & 1,975,368\\
660 & 36,925 & 0 & 445,510 & 41,794 & 0 & 108,484 & 94,849 & 19,542 & 35,040 & 101,789 & 290,335 & 34,504 & 224,473 & 98,660 & 0 & 411,771 & 1,943,676\\
670 & 37,160 & 0 & 463,478 & 42,936 & 0 & 109,176 & 93,905 & 15,239 & 35,675 & 104,395 & 293,378 & 34,558 & 223,930 & 101,219 & 0 & 454,999 & 2,010,048\\
680 & 37,056 & 0 & 484,131 & 43,090 & 0 & 109,178 & 92,357 & 17,478 & 35,753 & 102,800 & 295,657 & 35,587 & 224,403 & 101,334 & 0 & 440,568 & 2,019,392\\
690 & 37,095 & 0 & 489,331 & 43,282 & 0 & 109,177 & 93,430 & 22,883 & 35,729 & 102,792 & 295,660 & 39,587 & 225,328 & 100,712 & 0 & 539,102 & 2,134,108\\
700 & 37,160 & 0 & 490,748 & 44,497 & 0 & 109,176 & 92,705 & 23,428 & 35,724 & 109,507 & 295,657 & 38,203 & 225,379 & 101,362 & 0 & 541,096 & 2,144,642\\
710 & 37,465 & 0 & 498,285 & 43,325 & 0 & 109,176 & 94,849 & 24,257 & 35,737 & 109,488 & 295,659 & 39,498 & 225,348 & 101,199 & 0 & 539,105 & 2,153,391\\
720 & 37,170 & 0 & 504,337 & 44,341 & 0 & 109,628 & 92,640 & 24,254 & 35,741 & 109,506 & 295,660 & 40,993 & 226,845 & 101,199 & 0 & 578,184 & 2,200,498\\
730 & 37,542 & 0 & 533,139 & 43,727 & 0 & 110,034 & 100,641 & 24,196 & 35,773 & 109,488 & 301,121 & 40,407 & 226,849 & 103,553 & 0 & 539,116 & 2,205,586\\
740 & 37,543 & 0 & 533,731 & 43,656 & 0 & 109,644 & 100,127 & 26,864 & 36,458 & 109,506 & 295,659 & 41,186 & 226,799 & 103,696 & 0 & 539,116 & 2,203,985\\
750 & 37,335 & 0 & 538,181 & 43,865 & 0 & 111,139 & 100,642 & 24,771 & 35,765 & 109,502 & 306,836 & 42,364 & 226,840 & 103,411 & 0 & 608,677 & 2,289,328\\
760 & 37,574 & 0 & 548,456 & 44,063 & 0 & 111,134 & 100,133 & 26,130 & 36,901 & 109,508 & 310,317 & 42,729 & 227,490 & 105,820 & 0 & 554,130 & 2,254,385\\
770 & 38,056 & 0 & 548,456 & 44,427 & 0 & 111,077 & 100,140 & 26,451 & 36,162 & 111,139 & 310,373 & 44,166 & 226,826 & 103,678 & 0 & 578,201 & 2,279,152\\
780 & 37,751 & 0 & 573,096 & 43,926 & 0 & 111,137 & 100,644 & 28,132 & 36,713 & 109,497 & 310,525 & 43,615 & 227,603 & 103,511 & 0 & 605,674 & 2,331,824\\
790 & 38,159 & 0 & 573,666 & 45,461 & 0 & 111,172 & 102,162 & 26,555 & 36,425 & 109,506 & 310,556 & 45,628 & 227,424 & 105,740 & 0 & 574,569 & 2,307,023\\
800 & 40,383 & 0 & 573,265 & 44,431 & 0 & 111,382 & 101,740 & 27,838 & 35,796 & 109,488 & 310,558 & 45,209 & 227,925 & 105,873 & 0 & 660,596 & 2,394,484\\
810 & 37,958 & 0 & 596,544 & 45,455 & 0 & 111,461 & 101,739 & 29,327 & 36,142 & 110,731 & 313,873 & 45,916 & 229,309 & 103,696 & 0 & 673,671 & 2,435,822\\
820 & 39,769 & 0 & 602,074 & 45,518 & 0 & 111,144 & 103,740 & 26,768 & 37,336 & 110,732 & 314,579 & 48,174 & 228,257 & 103,696 & 0 & 683,446 & 2,455,233\\
830 & 39,404 & 0 & 627,562 & 46,768 & 0 & 111,144 & 103,781 & 27,838 & 37,714 & 111,272 & 323,850 & 53,165 & 231,454 & 105,288 & 0 & 684,550 & 2,503,790\\
840 & 40,776 & 0 & 624,029 & 45,838 & 0 & 111,422 & 103,781 & 29,672 & 37,730 & 110,732 & 324,798 & 56,909 & 231,406 & 104,900 & 0 & 704,906 & 2,526,899\\
850 & 41,237 & 0 & 629,128 & 45,559 & 0 & 111,536 & 103,781 & 27,994 & 37,548 & 110,732 & 327,238 & 56,222 & 229,309 & 104,883 & 0 & 695,734 & 2,520,901\\
860 & 40,826 & 0 & 645,313 & 47,817 & 0 & 111,144 & 103,780 & 27,626 & 37,896 & 111,255 & 346,510 & 65,383 & 228,781 & 104,936 & 0 & 710,700 & 2,581,967\\
870 & 40,780 & 0 & 645,313 & 47,890 & 0 & 111,143 & 103,780 & 27,190 & 37,754 & 110,735 & 349,237 & 60,196 & 230,243 & 104,943 & 0 & 721,451 & 2,590,655\\
880 & 41,485 & 0 & 670,418 & 47,720 & 0 & 111,143 & 103,781 & 30,124 & 37,737 & 111,122 & 349,044 & 68,273 & 230,584 & 105,851 & 0 & 728,244 & 2,635,526\\
890 & 41,848 & 0 & 667,933 & 50,426 & 0 & 111,426 & 103,878 & 30,123 & 37,737 & 110,741 & 349,239 & 68,731 & 229,640 & 108,006 & 0 & 733,753 & 2,643,481\\
900 & 41,254 & 0 & 679,022 & 49,024 & 0 & 112,351 & 104,674 & 30,101 & 38,831 & 110,741 & 349,090 & 68,525 & 231,712 & 108,605 & 0 & 721,451 & 2,645,381\\
910 & 41,556 & 0 & 678,507 & 49,075 & 0 & 111,383 & 103,781 & 30,462 & 38,824 & 113,114 & 354,768 & 68,955 & 231,454 & 108,606 & 0 & 760,219 & 2,690,704\\
920 & 41,848 & 0 & 667,913 & 48,547 & 0 & 112,473 & 103,877 & 30,126 & 39,144 & 110,735 & 380,991 & 70,110 & 232,085 & 108,365 & 0 & 783,932 & 2,730,146\\
930 & 41,351 & 0 & 706,580 & 48,509 & 0 & 111,524 & 103,874 & 30,126 & 37,766 & 111,251 & 349,317 & 70,830 & 231,668 & 108,561 & 0 & 784,311 & 2,735,668\\
940 & 41,887 & 0 & 680,148 & 48,319 & 0 & 112,348 & 104,294 & 30,126 & 38,041 & 113,113 & 352,519 & 71,991 & 231,658 & 108,600 & 0 & 792,911 & 2,725,955\\
950 & 41,736 & 0 & 745,094 & 48,734 & 0 & 111,524 & 103,781 & 30,127 & 38,056 & 116,736 & 356,164 & 71,559 & 232,659 & 110,346 & 0 & 792,923 & 2,799,439\\
960 & 41,978 & 0 & 747,014 & 49,217 & 0 & 112,179 & 103,781 & 30,231 & 38,041 & 115,164 & 350,829 & 71,595 & 232,699 & 111,856 & 0 & 784,307 & 2,788,891\\
970 & 45,459 & 0 & 768,933 & 50,124 & 0 & 112,242 & 104,294 & 30,481 & 38,506 & 116,126 & 355,117 & 71,991 & 232,689 & 112,031 & 0 & 822,922 & 2,860,915\\
980 & 42,019 & 0 & 760,514 & 48,549 & 0 & 111,676 & 103,782 & 30,584 & 39,978 & 116,143 & 363,636 & 71,257 & 233,959 & 112,031 & 0 & 849,389 & 2,883,517\\
990 & 45,127 & 0 & 789,864 & 49,364 & 0 & 111,673 & 108,463 & 31,782 & 38,739 & 115,682 & 409,662 & 71,629 & 233,958 & 112,031 & 0 & 855,637 & 2,973,611\\
1,000 & 42,077 & 0 & 789,864 & 48,745 & 0 & 111,575 & 110,270 & 32,159 & 38,480 & 120,974 & 370,553 & 72,036 & 233,958 & 112,031 & 0 & 858,813 & 2,941,535\\
1,010 & 45,956 & 0 & 809,615 & 49,024 & 0 & 112,348 & 112,989 & 30,405 & 41,263 & 120,975 & 374,580 & 71,595 & 234,679 & 112,162 & 0 & 864,265 & 2,979,856\\
1,020 & 45,458 & 0 & 808,755 & 50,142 & 0 & 111,575 & 110,102 & 31,063 & 41,263 & 120,975 & 410,255 & 72,408 & 234,463 & 112,032 & 0 & 864,585 & 3,013,076\\
1,030 & 44,715 & 0 & 812,172 & 53,607 & 0 & 111,808 & 121,050 & 32,860 & 41,268 & 120,974 & 394,519 & 72,168 & 234,660 & 113,618 & 0 & 864,584 & 3,018,003\\
1,040 & 45,458 & 0 & 811,135 & 50,142 & 0 & 111,674 & 113,172 & 33,937 & 41,262 & 120,975 & 407,319 & 72,191 & 234,704 & 112,032 & 0 & 861,467 & 3,015,468\\
1,050 & 45,556 & 0 & 849,919 & 52,298 & 0 & 112,734 & 117,197 & 33,512 & 41,279 & 123,741 & 433,022 & 72,234 & 236,216 & 112,032 & 0 & 855,531 & 3,085,271\\
1,060 & 45,708 & 0 & 848,518 & 52,365 & 0 & 112,785 & 126,100 & 33,931 & 41,270 & 120,975 & 432,222 & 72,866 & 234,473 & 112,031 & 0 & 870,203 & 3,103,447\\
1,070 & 46,739 & 0 & 868,177 & 53,702 & 0 & 112,348 & 131,264 & 33,336 & 41,998 & 123,779 & 431,863 & 71,992 & 234,679 & 113,152 & 0 & 856,539 & 3,119,568\\
1,080 & 45,259 & 0 & 878,542 & 55,434 & 0 & 113,403 & 131,265 & 33,654 & 41,736 & 123,734 & 412,927 & 72,810 & 235,552 & 112,032 & 0 & 866,760 & 3,123,108\\
1,090 & 46,151 & 0 & 879,342 & 54,437 & 0 & 112,400 & 138,769 & 33,897 & 42,533 & 120,975 & 411,445 & 72,790 & 235,324 & 113,640 & 0 & 925,854 & 3,187,557\\
1,100 & 46,318 & 0 & 875,749 & 53,996 & 0 & 112,287 & 140,513 & 33,495 & 41,740 & 125,168 & 411,231 & 73,529 & 236,698 & 113,142 & 0 & 855,644 & 3,119,510\\
1,110 & 46,138 & 0 & 878,147 & 53,155 & 0 & 112,505 & 141,639 & 33,775 & 41,533 & 125,164 & 431,384 & 75,140 & 236,698 & 112,163 & 0 & 856,537 & 3,143,978\\
1,120 & 46,914 & 0 & 917,028 & 54,785 & 0 & 113,562 & 130,470 & 34,018 & 41,903 & 125,165 & 411,908 & 73,529 & 237,513 & 112,162 & 0 & 856,553 & 3,155,510\\
1,130 & 46,296 & 0 & 919,413 & 55,844 & 0 & 113,189 & 145,784 & 33,775 & 42,022 & 125,164 & 449,700 & 75,933 & 237,512 & 113,640 & 0 & 856,542 & 3,214,814\\
1,140 & 46,597 & 0 & 931,599 & 55,443 & 0 & 113,687 & 168,490 & 33,530 & 42,601 & 125,167 & 498,070 & 75,132 & 237,488 & 113,773 & 0 & 972,429 & 3,414,006\\
1,150 & 0 & 0 & 946,680 & 57,447 & 0 & 112,502 & 151,778 & 33,999 & 41,739 & 125,163 & 497,994 & 74,721 & 238,824 & 114,073 & 0 & 918,807 & 3,313,727\\
1,160 & 0 & 0 & 946,868 & 58,579 & 0 & 113,703 & 183,175 & 33,775 & 41,997 & 125,162 & 498,061 & 74,740 & 237,647 & 113,773 & 0 & 864,101 & 3,291,581\\
1,170 & 0 & 0 & 946,533 & 60,133 & 0 & 113,703 & 190,682 & 34,717 & 42,283 & 125,161 & 498,068 & 73,830 & 238,649 & 113,467 & 0 & 913,488 & 3,350,714\\
1,180 & 0 & 0 & 972,122 & 58,587 & 0 & 113,580 & 190,529 & 34,039 & 42,944 & 125,160 & 498,000 & 73,891 & 239,854 & 113,525 & 0 & 998,202 & 3,460,433\\
1,190 & 0 & 0 & 956,609 & 57,104 & 0 & 113,643 & 191,414 & 33,842 & 42,003 & 125,164 & 498,070 & 74,607 & 240,839 & 116,531 & 0 & 903,650 & 3,353,476\\
1,200 & 0 & 0 & 964,864 & 57,054 & 0 & 114,447 & 199,116 & 34,786 & 42,726 & 125,161 & 514,941 & 74,804 & 243,240 & 118,507 & 0 & 980,745 & 3,470,391\\
1,210 & 0 & 0 & 974,035 & 57,734 & 0 & 113,385 & 204,807 & 34,027 & 42,230 & 125,165 & 514,919 & 75,881 & 244,082 & 116,121 & 0 & 998,202 & 3,500,588\\
1,220 & 0 & 0 & 992,599 & 60,306 & 0 & 0 & 204,620 & 36,567 & 42,903 & 125,161 & 515,199 & 75,929 & 246,612 & 114,556 & 0 & 875,368 & 3,289,820\\
1,230 & 0 & 0 & 980,037 & 58,998 & 0 & 0 & 204,563 & 35,009 & 44,218 & 125,167 & 515,199 & 75,025 & 244,084 & 115,564 & 0 & 918,807 & 3,316,671\\
1,240 & 0 & 0 & 999,888 & 58,993 & 0 & 0 & 213,693 & 34,410 & 43,269 & 125,168 & 515,702 & 76,462 & 246,417 & 115,967 & 0 & 952,818 & 3,382,787\\
1,250 & 0 & 0 & 972,545 & 62,082 & 0 & 0 & 207,163 & 34,018 & 42,794 & 125,160 & 516,781 & 75,601 & 244,486 & 115,754 & 0 & 965,940 & 3,362,324\\
1,260 & 0 & 0 & 979,469 & 60,416 & 0 & 0 & 208,145 & 34,839 & 44,741 & 125,165 & 547,846 & 75,441 & 246,942 & 116,805 & 0 & 965,940 & 3,405,749\\
1,270 & 0 & 0 & 999,888 & 62,798 & 0 & 0 & 213,363 & 34,284 & 43,266 & 125,163 & 518,410 & 76,329 & 244,088 & 119,949 & 0 & 944,590 & 3,382,128\\
1,280 & 0 & 0 & 999,888 & 61,286 & 0 & 0 & 209,570 & 36,567 & 44,741 & 125,166 & 541,551 & 75,933 & 245,328 & 116,804 & 0 & 901,358 & 3,358,192\\
1,290 & 0 & 0 & 999,888 & 64,781 & 0 & 0 & 211,241 & 36,413 & 43,143 & 125,168 & 552,322 & 75,791 & 247,978 & 121,084 & 0 & 865,952 & 3,343,761\\
1,300 & 0 & 0 & 999,888 & 61,084 & 0 & 0 & 215,577 & 35,780 & 44,134 & 125,163 & 551,527 & 76,192 & 244,062 & 120,923 & 0 & 998,202 & 3,472,532\\
1,310 & 0 & 0 & 999,888 & 67,561 & 0 & 0 & 214,363 & 38,192 & 43,630 & 125,160 & 553,093 & 76,159 & 245,166 & 118,393 & 0 & 953,333 & 3,434,938\\
1,320 & 0 & 0 & 999,888 & 67,917 & 0 & 0 & 215,273 & 37,647 & 43,269 & 125,165 & 541,889 & 77,286 & 244,362 & 123,179 & 0 & 998,202 & 3,474,077\\
1,330 & 0 & 0 & 999,888 & 67,660 & 0 & 0 & 222,271 & 37,587 & 43,166 & 125,163 & 551,949 & 78,664 & 245,018 & 118,610 & 0 & 980,745 & 3,470,721\\
1,340 & 0 & 0 & 999,888 & 73,218 & 0 & 0 & 216,695 & 37,394 & 45,199 & 125,168 & 542,823 & 77,399 & 246,902 & 119,283 & 0 & 998,202 & 3,482,171\\
1,350 & 0 & 0 & 999,888 & 80,132 & 0 & 0 & 218,195 & 36,888 & 44,908 & 129,094 & 542,385 & 76,284 & 247,433 & 121,158 & 0 & 995,938 & 3,492,303\\
1,360 & 0 & 0 & 999,888 & 79,556 & 0 & 0 & 216,496 & 36,593 & 44,752 & 125,165 & 550,187 & 76,472 & 250,522 & 124,106 & 0 & 998,202 & 3,501,939\\
1,370 & 0 & 0 & 999,888 & 80,540 & 0 & 0 & 219,922 & 36,447 & 44,163 & 129,094 & 558,263 & 77,154 & 248,354 & 119,170 & 0 & 935,100 & 3,448,095\\
1,380 & 0 & 0 & 999,888 & 80,398 & 0 & 0 & 220,552 & 40,831 & 44,163 & 129,070 & 555,235 & 76,815 & 249,403 & 120,845 & 0 & 998,202 & 3,515,402\\
1,390 & 0 & 0 & 999,888 & 80,540 & 0 & 0 & 222,318 & 40,386 & 44,240 & 125,165 & 569,028 & 79,468 & 249,492 & 123,324 & 0 & 998,202 & 3,532,051\\
1,400 & 0 & 0 & 999,888 & 81,585 & 0 & 0 & 220,528 & 40,347 & 44,240 & 128,856 & 569,011 & 80,026 & 247,980 & 123,412 & 0 & 998,202 & 3,534,075\\
1,410 & 0 & 0 & 999,888 & 82,193 & 0 & 0 & 223,000 & 40,386 & 44,472 & 125,168 & 569,257 & 80,666 & 249,491 & 124,688 & 0 & 998,202 & 3,537,411\\
1,420 & 0 & 0 & 999,888 & 86,759 & 0 & 0 & 223,004 & 40,423 & 44,646 & 125,166 & 564,345 & 80,169 & 250,458 & 123,516 & 0 & 998,202 & 3,536,576\\
1,430 & 0 & 0 & 999,888 & 86,515 & 0 & 0 & 223,053 & 40,406 & 44,742 & 128,846 & 563,292 & 79,187 & 248,357 & 124,388 & 0 & 998,202 & 3,536,876\\
1,440 & 0 & 0 & 999,888 & 85,048 & 0 & 0 & 223,053 & 40,347 & 0 & 129,074 & 558,252 & 80,247 & 248,243 & 125,640 & 0 & 998,202 & 3,487,994\\
1,450 & 0 & 0 & 999,888 & 85,069 & 0 & 0 & 225,799 & 40,338 & 0 & 128,998 & 569,014 & 79,454 & 249,115 & 125,175 & 0 & 998,202 & 3,501,052\\
1,460 & 0 & 0 & 999,888 & 84,978 & 0 & 0 & 226,520 & 40,353 & 0 & 129,080 & 569,144 & 80,349 & 249,084 & 124,007 & 0 & 998,202 & 3,501,605\\
1,470 & 0 & 0 & 999,888 & 85,763 & 0 & 0 & 233,978 & 40,352 & 0 & 129,094 & 569,248 & 79,943 & 248,482 & 126,346 & 0 & 998,202 & 3,511,296\\
1,480 & 0 & 0 & 999,888 & 84,882 & 0 & 0 & 233,979 & 40,430 & 0 & 128,850 & 569,075 & 81,054 & 249,106 & 126,234 & 0 & 998,202 & 3,511,700\\
1,490 & 0 & 0 & 999,888 & 85,763 & 0 & 0 & 226,888 & 40,448 & 0 & 125,166 & 569,087 & 80,448 & 249,247 & 126,345 & 0 & 998,202 & 3,501,482\\
1,500 & 0 & 0 & 999,888 & 86,125 & 0 & 0 & 234,424 & 40,353 & 0 & 128,998 & 558,146 & 80,330 & 252,544 & 126,345 & 0 & 998,202 & 3,505,355\\
1,510 & 0 & 0 & 999,888 & 84,978 & 0 & 0 & 229,986 & 38,730 & 0 & 125,168 & 558,263 & 80,176 & 253,145 & 129,196 & 0 & 998,202 & 3,497,732\\
1,520 & 0 & 0 & 999,888 & 86,757 & 0 & 0 & 228,718 & 38,735 & 0 & 130,562 & 558,098 & 79,921 & 252,282 & 124,864 & 0 & 998,202 & 3,498,027\\
1,530 & 0 & 0 & 999,888 & 85,533 & 0 & 0 & 227,865 & 38,770 & 0 & 130,568 & 577,185 & 80,336 & 252,708 & 125,430 & 0 & 998,202 & 3,516,485\\
1,540 & 0 & 0 & 999,888 & 89,504 & 0 & 0 & 227,401 & 38,872 & 0 & 131,975 & 577,167 & 81,306 & 252,281 & 125,416 & 0 & 998,202 & 3,522,012\\
1,550 & 0 & 0 & 999,888 & 86,050 & 0 & 0 & 229,098 & 38,914 & 0 & 130,618 & 577,168 & 79,644 & 252,732 & 125,407 & 0 & 998,202 & 3,517,721\\
1,560 & 0 & 0 & 999,888 & 85,097 & 0 & 0 & 229,247 & 39,420 & 0 & 131,975 & 577,186 & 0 & 252,282 & 127,334 & 0 & 998,202 & 3,440,631\\
1,570 & 0 & 0 & 999,888 & 89,292 & 0 & 0 & 232,453 & 39,442 & 0 & 131,973 & 602,904 & 0 & 252,280 & 125,174 & 0 & 998,202 & 3,471,608\\
1,580 & 0 & 0 & 999,888 & 88,549 & 0 & 0 & 230,762 & 42,554 & 0 & 130,648 & 602,904 & 0 & 252,279 & 125,405 & 0 & 998,202 & 3,471,191\\
1,590 & 0 & 0 & 999,888 & 91,570 & 0 & 0 & 231,442 & 42,750 & 0 & 132,089 & 602,902 & 0 & 252,280 & 125,400 & 0 & 998,202 & 3,476,523\\
1,600 & 0 & 0 & 999,888 & 91,570 & 0 & 0 & 234,499 & 42,554 & 0 & 144,295 & 602,902 & 0 & 252,282 & 128,951 & 0 & 998,202 & 3,495,143\\
1,610 & 0 & 0 & 999,888 & 91,154 & 0 & 0 & 241,170 & 42,554 & 0 & 130,635 & 602,901 & 0 & 252,545 & 129,949 & 0 & 998,202 & 3,488,998\\
1,620 & 0 & 0 & 999,888 & 91,569 & 0 & 0 & 236,568 & 42,555 & 0 & 135,402 & 602,903 & 0 & 253,301 & 128,283 & 0 & 998,202 & 3,488,671\\
1,630 & 0 & 0 & 999,888 & 91,570 & 0 & 0 & 233,213 & 42,732 & 0 & 141,152 & 602,901 & 0 & 253,219 & 129,447 & 0 & 998,202 & 3,492,324\\
1,640 & 0 & 0 & 999,888 & 91,570 & 0 & 0 & 233,823 & 42,749 & 0 & 141,227 & 602,901 & 0 & 254,410 & 132,050 & 0 & 0 & 2,498,618\\
1,650 & 0 & 0 & 999,996 & 91,597 & 0 & 0 & 234,426 & 42,554 & 0 & 145,349 & 602,904 & 0 & 254,067 & 132,050 & 0 & 0 & 2,502,943\\
1,660 & 0 & 0 & 999,996 & 91,597 & 0 & 0 & 235,026 & 42,555 & 0 & 148,595 & 602,904 & 0 & 254,067 & 126,851 & 0 & 0 & 2,501,591\\
1,670 & 0 & 0 & 999,996 & 91,598 & 0 & 0 & 241,166 & 42,732 & 0 & 145,405 & 610,007 & 0 & 254,019 & 132,452 & 0 & 0 & 2,517,375\\
1,680 & 0 & 0 & 999,996 & 91,913 & 0 & 0 & 242,049 & 43,011 & 0 & 141,153 & 602,904 & 0 & 254,073 & 127,612 & 0 & 0 & 2,502,711\\
1,690 & 0 & 0 & 999,996 & 91,569 & 0 & 0 & 242,060 & 42,554 & 0 & 143,762 & 602,906 & 0 & 253,300 & 127,612 & 0 & 0 & 2,503,759\\
1,700 & 0 & 0 & 999,996 & 91,572 & 0 & 0 & 235,026 & 42,555 & 0 & 145,123 & 603,380 & 0 & 254,019 & 134,553 & 0 & 0 & 2,506,224\\
1,710 & 0 & 0 & 999,996 & 91,593 & 0 & 0 & 237,561 & 42,732 & 0 & 145,592 & 602,903 & 0 & 255,017 & 131,156 & 0 & 0 & 2,506,550\\
1,720 & 0 & 0 & 999,996 & 91,597 & 0 & 0 & 237,945 & 42,991 & 0 & 146,772 & 602,904 & 0 & 254,297 & 129,447 & 0 & 0 & 2,505,949\\
1,730 & 0 & 0 & 999,996 & 91,570 & 0 & 0 & 239,156 & 42,554 & 0 & 145,883 & 602,902 & 0 & 253,364 & 130,151 & 0 & 0 & 2,505,576\\
1,740 & 0 & 0 & 999,996 & 91,597 & 0 & 0 & 241,148 & 42,701 & 0 & 144,295 & 602,901 & 0 & 257,256 & 133,432 & 0 & 0 & 2,513,326\\
1,750 & 0 & 0 & 999,996 & 91,570 & 0 & 0 & 241,866 & 42,976 & 0 & 145,589 & 602,904 & 0 & 253,974 & 138,864 & 0 & 0 & 2,517,739\\
1,760 & 0 & 0 & 999,996 & 91,569 & 0 & 0 & 240,187 & 42,554 & 0 & 146,261 & 602,906 & 0 & 254,062 & 131,518 & 0 & 0 & 2,509,053\\
1,770 & 0 & 0 & 999,996 & 91,598 & 0 & 0 & 241,145 & 42,555 & 0 & 146,297 & 602,903 & 0 & 254,177 & 134,488 & 0 & 0 & 2,513,159\\
1,780 & 0 & 0 & 999,996 & 91,597 & 0 & 0 & 238,649 & 42,750 & 0 & 146,560 & 602,901 & 0 & 254,394 & 129,677 & 0 & 0 & 2,506,524\\
1,790 & 0 & 0 & 999,996 & 93,617 & 0 & 0 & 239,796 & 42,719 & 0 & 149,269 & 602,901 & 0 & 255,284 & 134,280 & 0 & 0 & 2,517,862\\
1,800 & 0 & 0 & 999,996 & 91,597 & 0 & 0 & 241,754 & 42,999 & 0 & 145,120 & 602,905 & 0 & 253,959 & 129,196 & 0 & 0 & 2,507,526\\
1,810 & 0 & 0 & 999,996 & 0 & 0 & 0 & 241,159 & 46,045 & 0 & 145,404 & 602,904 & 0 & 253,957 & 134,483 & 0 & 0 & 2,423,948\\
1,820 & 0 & 0 & 999,996 & 0 & 0 & 0 & 241,323 & 42,734 & 0 & 148,006 & 602,904 & 0 & 254,780 & 135,075 & 0 & 0 & 2,424,818\\
1,830 & 0 & 0 & 999,996 & 0 & 0 & 0 & 242,051 & 43,393 & 0 & 145,596 & 602,904 & 0 & 256,386 & 135,018 & 0 & 0 & 2,425,344\\
1,840 & 0 & 0 & 999,996 & 0 & 0 & 0 & 241,700 & 46,081 & 0 & 146,719 & 611,940 & 0 & 253,697 & 135,466 & 0 & 0 & 2,435,599\\
1,850 & 0 & 0 & 999,996 & 0 & 0 & 0 & 241,684 & 45,455 & 0 & 145,722 & 602,901 & 0 & 254,394 & 138,865 & 0 & 0 & 2,429,017\\
1,860 & 0 & 0 & 999,996 & 0 & 0 & 0 & 243,046 & 46,685 & 0 & 151,656 & 620,604 & 0 & 255,283 & 135,329 & 0 & 0 & 2,452,599\\
1,870 & 0 & 0 & 999,996 & 0 & 0 & 0 & 242,166 & 48,232 & 0 & 146,695 & 604,749 & 0 & 254,193 & 143,262 & 0 & 0 & 2,439,293\\
1,880 & 0 & 0 & 999,996 & 0 & 0 & 0 & 241,754 & 46,144 & 0 & 146,056 & 602,904 & 0 & 256,000 & 134,972 & 0 & 0 & 2,427,826\\
1,890 & 0 & 0 & 999,996 & 0 & 0 & 0 & 241,701 & 46,678 & 0 & 145,597 & 610,808 & 0 & 257,317 & 135,453 & 0 & 0 & 2,437,550\\
1,900 & 0 & 0 & 999,996 & 0 & 0 & 0 & 244,512 & 47,984 & 0 & 145,664 & 602,901 & 0 & 259,159 & 136,567 & 0 & 0 & 2,436,783\\
1,910 & 0 & 0 & 999,996 & 0 & 0 & 0 & 244,683 & 48,156 & 0 & 0 & 604,749 & 0 & 257,269 & 139,055 & 0 & 0 & 2,293,908\\
1,920 & 0 & 0 & 999,996 & 0 & 0 & 0 & 244,022 & 46,740 & 0 & 0 & 602,904 & 0 & 257,310 & 137,000 & 0 & 0 & 2,287,972\\
1,930 & 0 & 0 & 999,996 & 0 & 0 & 0 & 243,982 & 47,532 & 0 & 0 & 602,906 & 0 & 257,345 & 140,372 & 0 & 0 & 2,292,133\\
1,940 & 0 & 0 & 999,996 & 0 & 0 & 0 & 245,957 & 47,960 & 0 & 0 & 602,901 & 0 & 258,416 & 137,012 & 0 & 0 & 2,292,242\\
1,950 & 0 & 0 & 999,996 & 0 & 0 & 0 & 242,687 & 48,116 & 0 & 0 & 623,114 & 0 & 257,305 & 137,022 & 0 & 0 & 2,308,240\\
1,960 & 0 & 0 & 999,996 & 0 & 0 & 0 & 242,282 & 49,061 & 0 & 0 & 634,773 & 0 & 258,770 & 136,982 & 0 & 0 & 2,321,864\\
1,970 & 0 & 0 & 999,996 & 0 & 0 & 0 & 245,039 & 47,467 & 0 & 0 & 618,942 & 0 & 258,096 & 136,782 & 0 & 0 & 2,306,322\\
1,980 & 0 & 0 & 999,996 & 0 & 0 & 0 & 255,711 & 47,693 & 0 & 0 & 618,868 & 0 & 257,363 & 136,785 & 0 & 0 & 2,316,416\\
1,990 & 0 & 0 & 999,996 & 0 & 0 & 0 & 249,862 & 48,124 & 0 & 0 & 634,773 & 0 & 258,981 & 138,195 & 0 & 0 & 2,329,931\\
2,000 & 0 & 0 & 999,996 & 0 & 0 & 0 & 246,463 & 49,060 & 0 & 0 & 620,862 & 0 & 258,934 & 137,086 & 0 & 0 & 2,312,401\\
2,010 & 0 & 0 & 999,996 & 0 & 0 & 0 & 243,982 & 48,109 & 0 & 0 & 616,553 & 0 & 258,752 & 139,904 & 0 & 0 & 2,307,296\\
2,020 & 0 & 0 & 999,996 & 0 & 0 & 0 & 250,318 & 48,928 & 0 & 0 & 647,906 & 0 & 258,729 & 141,979 & 0 & 0 & 2,347,856\\
2,030 & 0 & 0 & 999,996 & 0 & 0 & 0 & 245,942 & 51,439 & 0 & 0 & 634,773 & 0 & 0 & 148,710 & 0 & 0 & 2,080,860\\
2,040 & 0 & 0 & 999,996 & 0 & 0 & 0 & 244,561 & 48,015 & 0 & 0 & 619,027 & 0 & 0 & 147,518 & 0 & 0 & 2,059,117\\
2,050 & 0 & 0 & 999,996 & 0 & 0 & 0 & 259,984 & 48,619 & 0 & 0 & 619,145 & 0 & 0 & 148,293 & 0 & 0 & 2,076,037\\
2,060 & 0 & 0 & 999,996 & 0 & 0 & 0 & 246,271 & 49,764 & 0 & 0 & 622,607 & 0 & 0 & 137,023 & 0 & 0 & 2,055,661\\
2,070 & 0 & 0 & 999,996 & 0 & 0 & 0 & 250,218 & 47,999 & 0 & 0 & 618,627 & 0 & 0 & 137,449 & 0 & 0 & 2,054,289\\
2,080 & 0 & 0 & 999,996 & 0 & 0 & 0 & 248,460 & 48,515 & 0 & 0 & 621,211 & 0 & 0 & 141,827 & 0 & 0 & 2,060,009\\
2,090 & 0 & 0 & 999,996 & 0 & 0 & 0 & 252,543 & 49,258 & 0 & 0 & 625,789 & 0 & 0 & 147,134 & 0 & 0 & 2,074,720\\
2,100 & 0 & 0 & 999,996 & 0 & 0 & 0 & 245,942 & 47,910 & 0 & 0 & 629,446 & 0 & 0 & 148,727 & 0 & 0 & 2,072,021\\
2,110 & 0 & 0 & 999,996 & 0 & 0 & 0 & 262,144 & 48,567 & 0 & 0 & 627,595 & 0 & 0 & 137,153 & 0 & 0 & 2,075,455\\
2,120 & 0 & 0 & 999,996 & 0 & 0 & 0 & 243,636 & 49,908 & 0 & 0 & 636,360 & 0 & 0 & 137,379 & 0 & 0 & 2,067,279\\
2,130 & 0 & 0 & 999,996 & 0 & 0 & 0 & 254,470 & 48,120 & 0 & 0 & 632,565 & 0 & 0 & 140,380 & 0 & 0 & 2,075,531\\
2,140 & 0 & 0 & 999,996 & 0 & 0 & 0 & 247,867 & 49,131 & 0 & 0 & 633,224 & 0 & 0 & 145,721 & 0 & 0 & 2,075,939\\
2,150 & 0 & 0 & 999,996 & 0 & 0 & 0 & 249,233 & 54,694 & 0 & 0 & 658,655 & 0 & 0 & 139,136 & 0 & 0 & 2,101,714\\
2,160 & 0 & 0 & 999,996 & 0 & 0 & 0 & 264,590 & 48,482 & 0 & 0 & 632,096 & 0 & 0 & 137,254 & 0 & 0 & 2,082,418\\
2,170 & 0 & 0 & 999,996 & 0 & 0 & 0 & 249,126 & 48,619 & 0 & 0 & 631,700 & 0 & 0 & 146,380 & 0 & 0 & 2,075,821\\
2,180 & 0 & 0 & 999,996 & 0 & 0 & 0 & 243,538 & 50,318 & 0 & 0 & 634,444 & 0 & 0 & 148,089 & 0 & 0 & 2,076,385\\
2,190 & 0 & 0 & 999,996 & 0 & 0 & 0 & 252,185 & 48,420 & 0 & 0 & 632,770 & 0 & 0 & 138,710 & 0 & 0 & 2,072,081\\
2,200 & 0 & 0 & 0 & 0 & 0 & 0 & 249,302 & 50,106 & 0 & 0 & 633,234 & 0 & 0 & 148,294 & 0 & 0 & 1,080,936\\
2,210 & 0 & 0 & 0 & 0 & 0 & 0 & 243,965 & 54,549 & 0 & 0 & 634,799 & 0 & 0 & 151,078 & 0 & 0 & 1,084,391\\
2,220 & 0 & 0 & 0 & 0 & 0 & 0 & 243,965 & 50,145 & 0 & 0 & 650,155 & 0 & 0 & 140,022 & 0 & 0 & 1,084,287\\
2,230 & 0 & 0 & 0 & 0 & 0 & 0 & 260,108 & 53,636 & 0 & 0 & 668,514 & 0 & 0 & 140,022 & 0 & 0 & 1,122,280\\
2,240 & 0 & 0 & 0 & 0 & 0 & 0 & 260,229 & 50,078 & 0 & 0 & 658,678 & 0 & 0 & 0 & 0 & 0 & 968,985\\
2,250 & 0 & 0 & 0 & 0 & 0 & 0 & 258,559 & 53,281 & 0 & 0 & 655,520 & 0 & 0 & 0 & 0 & 0 & 967,360\\
2,260 & 0 & 0 & 0 & 0 & 0 & 0 & 259,987 & 50,216 & 0 & 0 & 637,933 & 0 & 0 & 0 & 0 & 0 & 948,136\\
2,270 & 0 & 0 & 0 & 0 & 0 & 0 & 260,229 & 53,375 & 0 & 0 & 678,310 & 0 & 0 & 0 & 0 & 0 & 991,914\\
2,280 & 0 & 0 & 0 & 0 & 0 & 0 & 259,984 & 56,277 & 0 & 0 & 672,549 & 0 & 0 & 0 & 0 & 0 & 988,810\\
2,290 & 0 & 0 & 0 & 0 & 0 & 0 & 251,529 & 53,203 & 0 & 0 & 672,142 & 0 & 0 & 0 & 0 & 0 & 976,874\\
2,300 & 0 & 0 & 0 & 0 & 0 & 0 & 259,989 & 55,058 & 0 & 0 & 677,636 & 0 & 0 & 0 & 0 & 0 & 992,683\\
2,310 & 0 & 0 & 0 & 0 & 0 & 0 & 262,868 & 53,187 & 0 & 0 & 640,249 & 0 & 0 & 0 & 0 & 0 & 956,304\\
2,320 & 0 & 0 & 0 & 0 & 0 & 0 & 247,867 & 54,292 & 0 & 0 & 654,298 & 0 & 0 & 0 & 0 & 0 & 956,457\\
2,330 & 0 & 0 & 0 & 0 & 0 & 0 & 250,976 & 53,066 & 0 & 0 & 678,463 & 0 & 0 & 0 & 0 & 0 & 982,505\\
2,340 & 0 & 0 & 0 & 0 & 0 & 0 & 258,264 & 53,647 & 0 & 0 & 655,520 & 0 & 0 & 0 & 0 & 0 & 967,431\\
2,350 & 0 & 0 & 0 & 0 & 0 & 0 & 245,133 & 52,923 & 0 & 0 & 639,402 & 0 & 0 & 0 & 0 & 0 & 937,458\\
2,360 & 0 & 0 & 0 & 0 & 0 & 0 & 256,575 & 53,558 & 0 & 0 & 679,750 & 0 & 0 & 0 & 0 & 0 & 989,883\\
2,370 & 0 & 0 & 0 & 0 & 0 & 0 & 262,292 & 52,784 & 0 & 0 & 671,996 & 0 & 0 & 0 & 0 & 0 & 987,072\\
2,380 & 0 & 0 & 0 & 0 & 0 & 0 & 256,662 & 53,359 & 0 & 0 & 668,515 & 0 & 0 & 0 & 0 & 0 & 978,536\\
2,390 & 0 & 0 & 0 & 0 & 0 & 0 & 249,862 & 55,270 & 0 & 0 & 672,120 & 0 & 0 & 0 & 0 & 0 & 977,252\\
2,400 & 0 & 0 & 0 & 0 & 0 & 0 & 250,319 & 53,257 & 0 & 0 & 654,317 & 0 & 0 & 0 & 0 & 0 & 957,893\\
2,410 & 0 & 0 & 0 & 0 & 0 & 0 & 245,941 & 55,058 & 0 & 0 & 653,977 & 0 & 0 & 0 & 0 & 0 & 954,976\\
2,420 & 0 & 0 & 0 & 0 & 0 & 0 & 265,286 & 57,589 & 0 & 0 & 640,779 & 0 & 0 & 0 & 0 & 0 & 963,654\\
2,430 & 0 & 0 & 0 & 0 & 0 & 0 & 257,675 & 60,610 & 0 & 0 & 675,852 & 0 & 0 & 0 & 0 & 0 & 994,137\\
2,440 & 0 & 0 & 0 & 0 & 0 & 0 & 254,932 & 58,430 & 0 & 0 & 655,888 & 0 & 0 & 0 & 0 & 0 & 969,250\\
2,450 & 0 & 0 & 0 & 0 & 0 & 0 & 249,310 & 57,589 & 0 & 0 & 638,619 & 0 & 0 & 0 & 0 & 0 & 945,518\\
2,460 & 0 & 0 & 0 & 0 & 0 & 0 & 249,305 & 59,476 & 0 & 0 & 638,223 & 0 & 0 & 0 & 0 & 0 & 947,004\\
2,470 & 0 & 0 & 0 & 0 & 0 & 0 & 257,675 & 59,927 & 0 & 0 & 673,921 & 0 & 0 & 0 & 0 & 0 & 991,523\\
2,480 & 0 & 0 & 0 & 0 & 0 & 0 & 253,326 & 60,842 & 0 & 0 & 658,695 & 0 & 0 & 0 & 0 & 0 & 972,863\\
2,490 & 0 & 0 & 0 & 0 & 0 & 0 & 247,673 & 60,755 & 0 & 0 & 680,851 & 0 & 0 & 0 & 0 & 0 & 989,279\\
2,500 & 0 & 0 & 0 & 0 & 0 & 0 & 265,822 & 61,229 & 0 & 0 & 653,583 & 0 & 0 & 0 & 0 & 0 & 980,634\\
2,510 & 0 & 0 & 0 & 0 & 0 & 0 & 255,430 & 62,211 & 0 & 0 & 639,402 & 0 & 0 & 0 & 0 & 0 & 957,043\\
2,520 & 0 & 0 & 0 & 0 & 0 & 0 & 254,932 & 62,247 & 0 & 0 & 672,122 & 0 & 0 & 0 & 0 & 0 & 989,301\\
2,530 & 0 & 0 & 0 & 0 & 0 & 0 & 261,254 & 61,776 & 0 & 0 & 639,347 & 0 & 0 & 0 & 0 & 0 & 962,377\\
2,540 & 0 & 0 & 0 & 0 & 0 & 0 & 262,292 & 61,595 & 0 & 0 & 654,317 & 0 & 0 & 0 & 0 & 0 & 978,204\\
2,550 & 0 & 0 & 0 & 0 & 0 & 0 & 246,690 & 61,465 & 0 & 0 & 677,886 & 0 & 0 & 0 & 0 & 0 & 986,041\\
2,560 & 0 & 0 & 0 & 0 & 0 & 0 & 257,319 & 60,930 & 0 & 0 & 681,548 & 0 & 0 & 0 & 0 & 0 & 999,797\\
2,570 & 0 & 0 & 0 & 0 & 0 & 0 & 255,754 & 63,139 & 0 & 0 & 655,594 & 0 & 0 & 0 & 0 & 0 & 974,487\\
2,580 & 0 & 0 & 0 & 0 & 0 & 0 & 254,469 & 62,051 & 0 & 0 & 639,402 & 0 & 0 & 0 & 0 & 0 & 955,922\\
2,590 & 0 & 0 & 0 & 0 & 0 & 0 & 255,711 & 61,763 & 0 & 0 & 676,660 & 0 & 0 & 0 & 0 & 0 & 994,134\\
2,600 & 0 & 0 & 0 & 0 & 0 & 0 & 259,781 & 63,880 & 0 & 0 & 666,267 & 0 & 0 & 0 & 0 & 0 & 989,928\\
2,610 & 0 & 0 & 0 & 0 & 0 & 0 & 259,990 & 62,426 & 0 & 0 & 641,832 & 0 & 0 & 0 & 0 & 0 & 964,248\\
2,620 & 0 & 0 & 0 & 0 & 0 & 0 & 262,004 & 65,285 & 0 & 0 & 642,067 & 0 & 0 & 0 & 0 & 0 & 969,356\\
2,630 & 0 & 0 & 0 & 0 & 0 & 0 & 265,056 & 62,654 & 0 & 0 & 663,394 & 0 & 0 & 0 & 0 & 0 & 991,104\\
2,640 & 0 & 0 & 0 & 0 & 0 & 0 & 247,268 & 64,475 & 0 & 0 & 658,759 & 0 & 0 & 0 & 0 & 0 & 970,502\\
2,650 & 0 & 0 & 0 & 0 & 0 & 0 & 250,151 & 65,823 & 0 & 0 & 651,855 & 0 & 0 & 0 & 0 & 0 & 967,829\\
2,660 & 0 & 0 & 0 & 0 & 0 & 0 & 255,035 & 63,050 & 0 & 0 & 668,511 & 0 & 0 & 0 & 0 & 0 & 986,596\\
2,670 & 0 & 0 & 0 & 0 & 0 & 0 & 258,264 & 64,693 & 0 & 0 & 656,372 & 0 & 0 & 0 & 0 & 0 & 979,329\\
2,680 & 0 & 0 & 0 & 0 & 0 & 0 & 263,317 & 65,741 & 0 & 0 & 644,274 & 0 & 0 & 0 & 0 & 0 & 973,332\\
2,690 & 0 & 0 & 0 & 0 & 0 & 0 & 251,100 & 64,264 & 0 & 0 & 655,888 & 0 & 0 & 0 & 0 & 0 & 971,252\\
2,700 & 0 & 0 & 0 & 0 & 0 & 0 & 257,808 & 66,618 & 0 & 0 & 653,516 & 0 & 0 & 0 & 0 & 0 & 977,942\\
2,710 & 0 & 0 & 0 & 0 & 0 & 0 & 264,538 & 64,717 & 0 & 0 & 645,096 & 0 & 0 & 0 & 0 & 0 & 974,351\\
2,720 & 0 & 0 & 0 & 0 & 0 & 0 & 250,091 & 62,525 & 0 & 0 & 672,639 & 0 & 0 & 0 & 0 & 0 & 985,255\\
2,730 & 0 & 0 & 0 & 0 & 0 & 0 & 259,984 & 64,878 & 0 & 0 & 681,950 & 0 & 0 & 0 & 0 & 0 & 1,006,812\\
2,740 & 0 & 0 & 0 & 0 & 0 & 0 & 246,539 & 67,088 & 0 & 0 & 658,678 & 0 & 0 & 0 & 0 & 0 & 972,305\\
2,750 & 0 & 0 & 0 & 0 & 0 & 0 & 256,772 & 64,026 & 0 & 0 & 692,689 & 0 & 0 & 0 & 0 & 0 & 1,013,487\\
2,760 & 0 & 0 & 0 & 0 & 0 & 0 & 245,940 & 65,539 & 0 & 0 & 692,465 & 0 & 0 & 0 & 0 & 0 & 1,003,944\\
2,770 & 0 & 0 & 0 & 0 & 0 & 0 & 258,673 & 63,062 & 0 & 0 & 658,967 & 0 & 0 & 0 & 0 & 0 & 980,702\\
2,780 & 0 & 0 & 0 & 0 & 0 & 0 & 250,976 & 64,909 & 0 & 0 & 665,942 & 0 & 0 & 0 & 0 & 0 & 981,827\\
2,790 & 0 & 0 & 0 & 0 & 0 & 0 & 262,655 & 67,820 & 0 & 0 & 672,122 & 0 & 0 & 0 & 0 & 0 & 1,002,597\\
2,800 & 0 & 0 & 0 & 0 & 0 & 0 & 256,637 & 64,036 & 0 & 0 & 684,682 & 0 & 0 & 0 & 0 & 0 & 1,005,355\\
2,810 & 0 & 0 & 0 & 0 & 0 & 0 & 250,976 & 65,824 & 0 & 0 & 659,003 & 0 & 0 & 0 & 0 & 0 & 975,803\\
2,820 & 0 & 0 & 0 & 0 & 0 & 0 & 264,539 & 63,619 & 0 & 0 & 670,557 & 0 & 0 & 0 & 0 & 0 & 998,715\\
2,830 & 0 & 0 & 0 & 0 & 0 & 0 & 256,917 & 65,164 & 0 & 0 & 692,464 & 0 & 0 & 0 & 0 & 0 & 1,014,545\\
2,840 & 0 & 0 & 0 & 0 & 0 & 0 & 250,814 & 62,654 & 0 & 0 & 668,514 & 0 & 0 & 0 & 0 & 0 & 981,982\\
2,850 & 0 & 0 & 0 & 0 & 0 & 0 & 247,852 & 64,890 & 0 & 0 & 692,689 & 0 & 0 & 0 & 0 & 0 & 1,005,431\\
2,860 & 0 & 0 & 0 & 0 & 0 & 0 & 256,179 & 67,572 & 0 & 0 & 671,996 & 0 & 0 & 0 & 0 & 0 & 995,747\\
2,870 & 0 & 0 & 0 & 0 & 0 & 0 & 259,986 & 64,412 & 0 & 0 & 664,389 & 0 & 0 & 0 & 0 & 0 & 988,787\\
2,880 & 0 & 0 & 0 & 0 & 0 & 0 & 259,984 & 66,687 & 0 & 0 & 693,794 & 0 & 0 & 0 & 0 & 0 & 1,020,465\\
2,890 & 0 & 0 & 0 & 0 & 0 & 0 & 257,815 & 65,187 & 0 & 0 & 686,879 & 0 & 0 & 0 & 0 & 0 & 1,009,881\\
2,900 & 0 & 0 & 0 & 0 & 0 & 0 & 257,675 & 64,906 & 0 & 0 & 681,718 & 0 & 0 & 0 & 0 & 0 & 1,004,299\\
2,910 & 0 & 0 & 0 & 0 & 0 & 0 & 267,368 & 68,286 & 0 & 0 & 681,793 & 0 & 0 & 0 & 0 & 0 & 1,017,447\\
2,920 & 0 & 0 & 0 & 0 & 0 & 0 & 267,368 & 64,906 & 0 & 0 & 678,212 & 0 & 0 & 0 & 0 & 0 & 1,010,486\\
2,930 & 0 & 0 & 0 & 0 & 0 & 0 & 267,259 & 68,304 & 0 & 0 & 681,664 & 0 & 0 & 0 & 0 & 0 & 1,017,227\\
2,940 & 0 & 0 & 0 & 0 & 0 & 0 & 265,068 & 64,910 & 0 & 0 & 691,514 & 0 & 0 & 0 & 0 & 0 & 1,021,492\\
2,950 & 0 & 0 & 0 & 0 & 0 & 0 & 264,476 & 67,665 & 0 & 0 & 657,346 & 0 & 0 & 0 & 0 & 0 & 989,487\\
2,960 & 0 & 0 & 0 & 0 & 0 & 0 & 268,820 & 64,890 & 0 & 0 & 665,558 & 0 & 0 & 0 & 0 & 0 & 999,268\\
2,970 & 0 & 0 & 0 & 0 & 0 & 0 & 268,820 & 67,518 & 0 & 0 & 677,636 & 0 & 0 & 0 & 0 & 0 & 1,013,974\\
2,980 & 0 & 0 & 0 & 0 & 0 & 0 & 268,822 & 64,681 & 0 & 0 & 662,265 & 0 & 0 & 0 & 0 & 0 & 995,768\\
2,990 & 0 & 0 & 0 & 0 & 0 & 0 & 268,884 & 66,941 & 0 & 0 & 681,778 & 0 & 0 & 0 & 0 & 0 & 1,017,603\\
3,000 & 0 & 0 & 0 & 0 & 0 & 0 & 266,607 & 64,803 & 0 & 0 & 670,519 & 0 & 0 & 0 & 0 & 0 & 1,001,929\\
3,010 & 0 & 0 & 0 & 0 & 0 & 0 & 267,379 & 66,887 & 0 & 0 & 692,679 & 0 & 0 & 0 & 0 & 0 & 1,026,945\\
3,020 & 0 & 0 & 0 & 0 & 0 & 0 & 267,379 & 64,312 & 0 & 0 & 666,461 & 0 & 0 & 0 & 0 & 0 & 998,152\\
3,030 & 0 & 0 & 0 & 0 & 0 & 0 & 267,380 & 66,385 & 0 & 0 & 661,309 & 0 & 0 & 0 & 0 & 0 & 995,074\\
3,040 & 0 & 0 & 0 & 0 & 0 & 0 & 268,728 & 63,953 & 0 & 0 & 670,365 & 0 & 0 & 0 & 0 & 0 & 1,003,046\\
3,050 & 0 & 0 & 0 & 0 & 0 & 0 & 268,865 & 66,248 & 0 & 0 & 695,230 & 0 & 0 & 0 & 0 & 0 & 1,030,343\\
3,060 & 0 & 0 & 0 & 0 & 0 & 0 & 267,115 & 64,908 & 0 & 0 & 687,808 & 0 & 0 & 0 & 0 & 0 & 1,019,831\\
3,070 & 0 & 0 & 0 & 0 & 0 & 0 & 267,260 & 67,491 & 0 & 0 & 681,582 & 0 & 0 & 0 & 0 & 0 & 1,016,333\\
3,080 & 0 & 0 & 0 & 0 & 0 & 0 & 267,372 & 64,890 & 0 & 0 & 681,582 & 0 & 0 & 0 & 0 & 0 & 1,013,844\\
3,090 & 0 & 0 & 0 & 0 & 0 & 0 & 268,593 & 67,581 & 0 & 0 & 694,913 & 0 & 0 & 0 & 0 & 0 & 1,031,087\\
3,100 & 0 & 0 & 0 & 0 & 0 & 0 & 268,847 & 64,906 & 0 & 0 & 690,954 & 0 & 0 & 0 & 0 & 0 & 1,024,707\\
3,110 & 0 & 0 & 0 & 0 & 0 & 0 & 267,360 & 67,765 & 0 & 0 & 681,287 & 0 & 0 & 0 & 0 & 0 & 1,016,412\\
3,120 & 0 & 0 & 0 & 0 & 0 & 0 & 267,761 & 64,927 & 0 & 0 & 677,896 & 0 & 0 & 0 & 0 & 0 & 1,010,584\\
3,130 & 0 & 0 & 0 & 0 & 0 & 0 & 268,864 & 68,340 & 0 & 0 & 668,142 & 0 & 0 & 0 & 0 & 0 & 1,005,346\\
3,140 & 0 & 0 & 0 & 0 & 0 & 0 & 268,761 & 64,927 & 0 & 0 & 667,473 & 0 & 0 & 0 & 0 & 0 & 1,001,161\\
3,150 & 0 & 0 & 0 & 0 & 0 & 0 & 267,260 & 67,863 & 0 & 0 & 667,251 & 0 & 0 & 0 & 0 & 0 & 1,002,374\\
3,160 & 0 & 0 & 0 & 0 & 0 & 0 & 267,377 & 64,967 & 0 & 0 & 667,287 & 0 & 0 & 0 & 0 & 0 & 999,631\\
3,170 & 0 & 0 & 0 & 0 & 0 & 0 & 268,731 & 65,218 & 0 & 0 & 669,969 & 0 & 0 & 0 & 0 & 0 & 1,003,918\\
3,180 & 0 & 0 & 0 & 0 & 0 & 0 & 267,260 & 65,092 & 0 & 0 & 671,459 & 0 & 0 & 0 & 0 & 0 & 1,003,811\\
3,190 & 0 & 0 & 0 & 0 & 0 & 0 & 268,708 & 68,616 & 0 & 0 & 677,939 & 0 & 0 & 0 & 0 & 0 & 1,015,263\\
3,200 & 0 & 0 & 0 & 0 & 0 & 0 & 267,260 & 65,768 & 0 & 0 & 686,017 & 0 & 0 & 0 & 0 & 0 & 1,019,045\\
3,210 & 0 & 0 & 0 & 0 & 0 & 0 & 268,705 & 69,765 & 0 & 0 & 695,964 & 0 & 0 & 0 & 0 & 0 & 1,034,434\\
3,220 & 0 & 0 & 0 & 0 & 0 & 0 & 267,259 & 66,481 & 0 & 0 & 668,925 & 0 & 0 & 0 & 0 & 0 & 1,002,665\\
3,230 & 0 & 0 & 0 & 0 & 0 & 0 & 268,708 & 64,883 & 0 & 0 & 677,636 & 0 & 0 & 0 & 0 & 0 & 1,011,227\\
3,240 & 0 & 0 & 0 & 0 & 0 & 0 & 267,260 & 67,672 & 0 & 0 & 692,465 & 0 & 0 & 0 & 0 & 0 & 1,027,397\\
3,250 & 0 & 0 & 0 & 0 & 0 & 0 & 268,761 & 65,411 & 0 & 0 & 669,547 & 0 & 0 & 0 & 0 & 0 & 1,003,719\\
3,260 & 0 & 0 & 0 & 0 & 0 & 0 & 267,370 & 69,702 & 0 & 0 & 683,458 & 0 & 0 & 0 & 0 & 0 & 1,020,530\\
3,270 & 0 & 0 & 0 & 0 & 0 & 0 & 268,819 & 66,494 & 0 & 0 & 666,506 & 0 & 0 & 0 & 0 & 0 & 1,001,819\\
3,280 & 0 & 0 & 0 & 0 & 0 & 0 & 267,376 & 64,890 & 0 & 0 & 683,497 & 0 & 0 & 0 & 0 & 0 & 1,015,763\\
3,290 & 0 & 0 & 0 & 0 & 0 & 0 & 272,746 & 67,895 & 0 & 0 & 668,361 & 0 & 0 & 0 & 0 & 0 & 1,009,002\\
3,300 & 0 & 0 & 0 & 0 & 0 & 0 & 268,694 & 65,696 & 0 & 0 & 691,472 & 0 & 0 & 0 & 0 & 0 & 1,025,862\\
3,310 & 0 & 0 & 0 & 0 & 0 & 0 & 267,374 & 69,906 & 0 & 0 & 671,459 & 0 & 0 & 0 & 0 & 0 & 1,008,739\\
3,320 & 0 & 0 & 0 & 0 & 0 & 0 & 268,874 & 66,687 & 0 & 0 & 663,558 & 0 & 0 & 0 & 0 & 0 & 999,119\\
3,330 & 0 & 0 & 0 & 0 & 0 & 0 & 267,377 & 64,910 & 0 & 0 & 686,879 & 0 & 0 & 0 & 0 & 0 & 1,019,166\\
3,340 & 0 & 0 & 0 & 0 & 0 & 0 & 267,260 & 68,576 & 0 & 0 & 672,557 & 0 & 0 & 0 & 0 & 0 & 1,008,393\\
3,350 & 0 & 0 & 0 & 0 & 0 & 0 & 268,847 & 65,968 & 0 & 0 & 667,333 & 0 & 0 & 0 & 0 & 0 & 1,002,148\\
3,360 & 0 & 0 & 0 & 0 & 0 & 0 & 267,648 & 71,509 & 0 & 0 & 698,519 & 0 & 0 & 0 & 0 & 0 & 1,037,676\\
3,370 & 0 & 0 & 0 & 0 & 0 & 0 & 267,370 & 67,581 & 0 & 0 & 692,460 & 0 & 0 & 0 & 0 & 0 & 1,027,411\\
3,380 & 0 & 0 & 0 & 0 & 0 & 0 & 273,649 & 65,539 & 0 & 0 & 685,950 & 0 & 0 & 0 & 0 & 0 & 1,025,138\\
3,390 & 0 & 0 & 0 & 0 & 0 & 0 & 268,842 & 69,478 & 0 & 0 & 681,664 & 0 & 0 & 0 & 0 & 0 & 1,019,984\\
3,400 & 0 & 0 & 0 & 0 & 0 & 0 & 268,216 & 66,639 & 0 & 0 & 677,896 & 0 & 0 & 0 & 0 & 0 & 1,012,751\\
3,410 & 0 & 0 & 0 & 0 & 0 & 0 & 267,360 & 64,911 & 0 & 0 & 676,400 & 0 & 0 & 0 & 0 & 0 & 1,008,671\\
3,420 & 0 & 0 & 0 & 0 & 0 & 0 & 268,868 & 68,991 & 0 & 0 & 677,636 & 0 & 0 & 0 & 0 & 0 & 1,015,495\\
3,430 & 0 & 0 & 0 & 0 & 0 & 0 & 267,623 & 66,296 & 0 & 0 & 681,889 & 0 & 0 & 0 & 0 & 0 & 1,015,808\\
3,440 & 0 & 0 & 0 & 0 & 0 & 0 & 267,379 & 74,282 & 0 & 0 & 698,626 & 0 & 0 & 0 & 0 & 0 & 1,040,287\\
3,450 & 0 & 0 & 0 & 0 & 0 & 0 & 267,369 & 65,767 & 0 & 0 & 665,954 & 0 & 0 & 0 & 0 & 0 & 999,090\\
3,460 & 0 & 0 & 0 & 0 & 0 & 0 & 266,496 & 66,248 & 0 & 0 & 669,348 & 0 & 0 & 0 & 0 & 0 & 1,002,092\\
3,470 & 0 & 0 & 0 & 0 & 0 & 0 & 268,845 & 67,673 & 0 & 0 & 681,920 & 0 & 0 & 0 & 0 & 0 & 1,018,438\\
3,480 & 0 & 0 & 0 & 0 & 0 & 0 & 267,380 & 66,774 & 0 & 0 & 671,099 & 0 & 0 & 0 & 0 & 0 & 1,005,253\\
3,490 & 0 & 0 & 0 & 0 & 0 & 0 & 267,373 & 74,148 & 0 & 0 & 685,851 & 0 & 0 & 0 & 0 & 0 & 1,027,372\\
3,500 & 0 & 0 & 0 & 0 & 0 & 0 & 267,259 & 69,436 & 0 & 0 & 666,463 & 0 & 0 & 0 & 0 & 0 & 1,003,158\\
3,510 & 0 & 0 & 0 & 0 & 0 & 0 & 273,649 & 74,375 & 0 & 0 & 672,664 & 0 & 0 & 0 & 0 & 0 & 1,020,688\\
3,520 & 0 & 0 & 0 & 0 & 0 & 0 & 268,884 & 73,968 & 0 & 0 & 698,777 & 0 & 0 & 0 & 0 & 0 & 1,041,629\\
3,530 & 0 & 0 & 0 & 0 & 0 & 0 & 268,841 & 75,086 & 0 & 0 & 672,610 & 0 & 0 & 0 & 0 & 0 & 1,016,537\\
3,540 & 0 & 0 & 0 & 0 & 0 & 0 & 268,729 & 74,384 & 0 & 0 & 668,511 & 0 & 0 & 0 & 0 & 0 & 1,011,624\\
3,550 & 0 & 0 & 0 & 0 & 0 & 0 & 268,682 & 73,975 & 0 & 0 & 694,559 & 0 & 0 & 0 & 0 & 0 & 1,037,216\\
3,560 & 0 & 0 & 0 & 0 & 0 & 0 & 268,844 & 74,516 & 0 & 0 & 680,912 & 0 & 0 & 0 & 0 & 0 & 1,024,272\\
3,570 & 0 & 0 & 0 & 0 & 0 & 0 & 268,845 & 74,279 & 0 & 0 & 692,679 & 0 & 0 & 0 & 0 & 0 & 1,035,803\\
3,580 & 0 & 0 & 0 & 0 & 0 & 0 & 268,842 & 75,000 & 0 & 0 & 670,557 & 0 & 0 & 0 & 0 & 0 & 1,014,399\\
3,590 & 0 & 0 & 0 & 0 & 0 & 0 & 268,730 & 74,483 & 0 & 0 & 685,950 & 0 & 0 & 0 & 0 & 0 & 1,029,163\\
3,600 & 0 & 0 & 0 & 0 & 0 & 0 & 268,708 & 74,148 & 0 & 0 & 692,465 & 0 & 0 & 0 & 0 & 0 & 1,035,321\\
3,610 & 0 & 0 & 0 & 0 & 0 & 0 & 268,593 & 74,501 & 0 & 0 & 691,688 & 0 & 0 & 0 & 0 & 0 & 1,034,782\\
3,620 & 0 & 0 & 0 & 0 & 0 & 0 & 268,593 & 74,382 & 0 & 0 & 694,425 & 0 & 0 & 0 & 0 & 0 & 1,037,400\\
3,630 & 0 & 0 & 0 & 0 & 0 & 0 & 268,593 & 74,535 & 0 & 0 & 698,799 & 0 & 0 & 0 & 0 & 0 & 1,041,927\\
3,640 & 0 & 0 & 0 & 0 & 0 & 0 & 268,841 & 74,487 & 0 & 0 & 671,700 & 0 & 0 & 0 & 0 & 0 & 1,015,028\\
3,650 & 0 & 0 & 0 & 0 & 0 & 0 & 268,819 & 74,271 & 0 & 0 & 700,991 & 0 & 0 & 0 & 0 & 0 & 1,044,081\\
3,660 & 0 & 0 & 0 & 0 & 0 & 0 & 268,819 & 74,496 & 0 & 0 & 692,464 & 0 & 0 & 0 & 0 & 0 & 1,035,779\\
3,670 & 0 & 0 & 0 & 0 & 0 & 0 & 268,843 & 74,370 & 0 & 0 & 681,849 & 0 & 0 & 0 & 0 & 0 & 1,025,062\\
3,680 & 0 & 0 & 0 & 0 & 0 & 0 & 268,865 & 74,508 & 0 & 0 & 675,274 & 0 & 0 & 0 & 0 & 0 & 1,018,647\\
3,690 & 0 & 0 & 0 & 0 & 0 & 0 & 269,709 & 74,476 & 0 & 0 & 672,089 & 0 & 0 & 0 & 0 & 0 & 1,016,274\\
3,700 & 0 & 0 & 0 & 0 & 0 & 0 & 266,607 & 75,107 & 0 & 0 & 671,015 & 0 & 0 & 0 & 0 & 0 & 1,012,729\\
3,710 & 0 & 0 & 0 & 0 & 0 & 0 & 267,372 & 74,494 & 0 & 0 & 704,486 & 0 & 0 & 0 & 0 & 0 & 1,046,352\\
3,720 & 0 & 0 & 0 & 0 & 0 & 0 & 267,375 & 74,313 & 0 & 0 & 698,919 & 0 & 0 & 0 & 0 & 0 & 1,040,607\\
3,730 & 0 & 0 & 0 & 0 & 0 & 0 & 267,379 & 74,503 & 0 & 0 & 698,338 & 0 & 0 & 0 & 0 & 0 & 1,040,220\\
3,740 & 0 & 0 & 0 & 0 & 0 & 0 & 268,593 & 74,458 & 0 & 0 & 698,318 & 0 & 0 & 0 & 0 & 0 & 1,041,369\\
3,750 & 0 & 0 & 0 & 0 & 0 & 0 & 268,707 & 75,557 & 0 & 0 & 698,474 & 0 & 0 & 0 & 0 & 0 & 1,042,738\\
3,760 & 0 & 0 & 0 & 0 & 0 & 0 & 268,765 & 74,315 & 0 & 0 & 700,150 & 0 & 0 & 0 & 0 & 0 & 1,043,230\\
3,770 & 0 & 0 & 0 & 0 & 0 & 0 & 268,843 & 74,796 & 0 & 0 & 707,620 & 0 & 0 & 0 & 0 & 0 & 1,051,259\\
3,780 & 0 & 0 & 0 & 0 & 0 & 0 & 268,875 & 74,495 & 0 & 0 & 671,317 & 0 & 0 & 0 & 0 & 0 & 1,014,687\\
3,790 & 0 & 0 & 0 & 0 & 0 & 0 & 271,305 & 74,373 & 0 & 0 & 672,742 & 0 & 0 & 0 & 0 & 0 & 1,018,420\\
3,800 & 0 & 0 & 0 & 0 & 0 & 0 & 266,304 & 74,532 & 0 & 0 & 681,361 & 0 & 0 & 0 & 0 & 0 & 1,022,197\\
3,810 & 0 & 0 & 0 & 0 & 0 & 0 & 267,260 & 74,493 & 0 & 0 & 687,278 & 0 & 0 & 0 & 0 & 0 & 1,029,031\\
3,820 & 0 & 0 & 0 & 0 & 0 & 0 & 267,372 & 74,799 & 0 & 0 & 692,469 & 0 & 0 & 0 & 0 & 0 & 1,034,640\\
3,830 & 0 & 0 & 0 & 0 & 0 & 0 & 265,370 & 74,524 & 0 & 0 & 699,906 & 0 & 0 & 0 & 0 & 0 & 1,039,800\\
3,840 & 0 & 0 & 0 & 0 & 0 & 0 & 267,256 & 74,490 & 0 & 0 & 672,040 & 0 & 0 & 0 & 0 & 0 & 1,013,786\\
3,850 & 0 & 0 & 0 & 0 & 0 & 0 & 267,370 & 74,748 & 0 & 0 & 681,718 & 0 & 0 & 0 & 0 & 0 & 1,023,836\\
3,860 & 0 & 0 & 0 & 0 & 0 & 0 & 267,378 & 74,529 & 0 & 0 & 697,758 & 0 & 0 & 0 & 0 & 0 & 1,039,665\\
3,870 & 0 & 0 & 0 & 0 & 0 & 0 & 268,694 & 75,063 & 0 & 0 & 672,089 & 0 & 0 & 0 & 0 & 0 & 1,015,846\\
3,880 & 0 & 0 & 0 & 0 & 0 & 0 & 268,846 & 74,644 & 0 & 0 & 692,305 & 0 & 0 & 0 & 0 & 0 & 1,035,795\\
3,890 & 0 & 0 & 0 & 0 & 0 & 0 & 265,067 & 74,504 & 0 & 0 & 672,020 & 0 & 0 & 0 & 0 & 0 & 1,011,591\\
3,900 & 0 & 0 & 0 & 0 & 0 & 0 & 267,376 & 74,774 & 0 & 0 & 692,333 & 0 & 0 & 0 & 0 & 0 & 1,034,483\\
3,910 & 0 & 0 & 0 & 0 & 0 & 0 & 268,634 & 74,617 & 0 & 0 & 673,920 & 0 & 0 & 0 & 0 & 0 & 1,017,171\\
3,920 & 0 & 0 & 0 & 0 & 0 & 0 & 268,846 & 74,504 & 0 & 0 & 692,464 & 0 & 0 & 0 & 0 & 0 & 1,035,814\\
3,930 & 0 & 0 & 0 & 0 & 0 & 0 & 266,596 & 74,780 & 0 & 0 & 671,459 & 0 & 0 & 0 & 0 & 0 & 1,012,835\\
3,940 & 0 & 0 & 0 & 0 & 0 & 0 & 267,370 & 74,643 & 0 & 0 & 694,927 & 0 & 0 & 0 & 0 & 0 & 1,036,940\\
3,950 & 0 & 0 & 0 & 0 & 0 & 0 & 268,842 & 74,508 & 0 & 0 & 674,274 & 0 & 0 & 0 & 0 & 0 & 1,017,624\\
3,960 & 0 & 0 & 0 & 0 & 0 & 0 & 267,370 & 74,784 & 0 & 0 & 694,043 & 0 & 0 & 0 & 0 & 0 & 1,036,197\\
3,970 & 0 & 0 & 0 & 0 & 0 & 0 & 268,875 & 74,643 & 0 & 0 & 675,280 & 0 & 0 & 0 & 0 & 0 & 1,018,798\\
3,980 & 0 & 0 & 0 & 0 & 0 & 0 & 265,548 & 74,504 & 0 & 0 & 698,558 & 0 & 0 & 0 & 0 & 0 & 1,038,610\\
3,990 & 0 & 0 & 0 & 0 & 0 & 0 & 268,216 & 74,780 & 0 & 0 & 685,983 & 0 & 0 & 0 & 0 & 0 & 1,028,979\\
4,000 & 0 & 0 & 0 & 0 & 0 & 0 & 267,374 & 74,624 & 0 & 0 & 670,995 & 0 & 0 & 0 & 0 & 0 & 1,012,993\\
4,010 & 0 & 0 & 0 & 0 & 0 & 0 & 268,729 & 74,504 & 0 & 0 & 692,464 & 0 & 0 & 0 & 0 & 0 & 1,035,697\\
4,020 & 0 & 0 & 0 & 0 & 0 & 0 & 269,748 & 75,053 & 0 & 0 & 691,475 & 0 & 0 & 0 & 0 & 0 & 1,036,276\\
4,030 & 0 & 0 & 0 & 0 & 0 & 0 & 268,846 & 74,772 & 0 & 0 & 682,642 & 0 & 0 & 0 & 0 & 0 & 1,026,260\\
4,040 & 0 & 0 & 0 & 0 & 0 & 0 & 268,695 & 74,619 & 0 & 0 & 676,624 & 0 & 0 & 0 & 0 & 0 & 1,019,938\\
4,050 & 0 & 0 & 0 & 0 & 0 & 0 & 268,865 & 74,511 & 0 & 0 & 672,024 & 0 & 0 & 0 & 0 & 0 & 1,015,400\\
4,060 & 0 & 0 & 0 & 0 & 0 & 0 & 268,862 & 74,784 & 0 & 0 & 672,061 & 0 & 0 & 0 & 0 & 0 & 1,015,707\\
4,070 & 0 & 0 & 0 & 0 & 0 & 0 & 266,589 & 74,658 & 0 & 0 & 701,069 & 0 & 0 & 0 & 0 & 0 & 1,042,316\\
4,080 & 0 & 0 & 0 & 0 & 0 & 0 & 267,259 & 74,518 & 0 & 0 & 700,991 & 0 & 0 & 0 & 0 & 0 & 1,042,768\\
4,090 & 0 & 0 & 0 & 0 & 0 & 0 & 269,709 & 74,867 & 0 & 0 & 694,889 & 0 & 0 & 0 & 0 & 0 & 1,039,465\\
4,100 & 0 & 0 & 0 & 0 & 0 & 0 & 266,598 & 74,659 & 0 & 0 & 685,051 & 0 & 0 & 0 & 0 & 0 & 1,026,308\\
4,110 & 0 & 0 & 0 & 0 & 0 & 0 & 267,380 & 74,528 & 0 & 0 & 685,983 & 0 & 0 & 0 & 0 & 0 & 1,027,891\\
4,120 & 0 & 0 & 0 & 0 & 0 & 0 & 268,843 & 75,417 & 0 & 0 & 684,664 & 0 & 0 & 0 & 0 & 0 & 1,028,924\\
4,130 & 0 & 0 & 0 & 0 & 0 & 0 & 265,815 & 74,728 & 0 & 0 & 678,606 & 0 & 0 & 0 & 0 & 0 & 1,019,149\\
4,140 & 0 & 0 & 0 & 0 & 0 & 0 & 273,034 & 74,586 & 0 & 0 & 674,283 & 0 & 0 & 0 & 0 & 0 & 1,021,903\\
4,150 & 0 & 0 & 0 & 0 & 0 & 0 & 267,360 & 77,652 & 0 & 0 & 690,521 & 0 & 0 & 0 & 0 & 0 & 1,035,533\\
4,160 & 0 & 0 & 0 & 0 & 0 & 0 & 268,847 & 74,776 & 0 & 0 & 685,544 & 0 & 0 & 0 & 0 & 0 & 1,029,167\\
4,170 & 0 & 0 & 0 & 0 & 0 & 0 & 267,378 & 74,642 & 0 & 0 & 683,883 & 0 & 0 & 0 & 0 & 0 & 1,025,903\\
4,180 & 0 & 0 & 0 & 0 & 0 & 0 & 268,845 & 74,514 & 0 & 0 & 672,142 & 0 & 0 & 0 & 0 & 0 & 1,015,501\\
4,190 & 0 & 0 & 0 & 0 & 0 & 0 & 267,260 & 74,958 & 0 & 0 & 682,726 & 0 & 0 & 0 & 0 & 0 & 1,024,944\\
4,200 & 0 & 0 & 0 & 0 & 0 & 0 & 268,708 & 74,703 & 0 & 0 & 681,689 & 0 & 0 & 0 & 0 & 0 & 1,025,100\\
4,210 & 0 & 0 & 0 & 0 & 0 & 0 & 269,540 & 74,590 & 0 & 0 & 684,274 & 0 & 0 & 0 & 0 & 0 & 1,028,404\\
4,220 & 0 & 0 & 0 & 0 & 0 & 0 & 272,575 & 76,581 & 0 & 0 & 678,788 & 0 & 0 & 0 & 0 & 0 & 1,027,944\\
4,230 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 75,184 & 0 & 0 & 686,340 & 0 & 0 & 0 & 0 & 0 & 761,524\\
4,240 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,731 & 0 & 0 & 672,396 & 0 & 0 & 0 & 0 & 0 & 747,127\\
4,250 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,619 & 0 & 0 & 692,679 & 0 & 0 & 0 & 0 & 0 & 767,298\\
4,260 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,511 & 0 & 0 & 698,777 & 0 & 0 & 0 & 0 & 0 & 773,288\\
4,270 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,802 & 0 & 0 & 700,991 & 0 & 0 & 0 & 0 & 0 & 775,793\\
4,280 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,681 & 0 & 0 & 707,662 & 0 & 0 & 0 & 0 & 0 & 782,343\\
4,290 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,564 & 0 & 0 & 706,626 & 0 & 0 & 0 & 0 & 0 & 781,190\\
4,300 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 77,707 & 0 & 0 & 690,500 & 0 & 0 & 0 & 0 & 0 & 768,207\\
4,310 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,780 & 0 & 0 & 707,536 & 0 & 0 & 0 & 0 & 0 & 782,316\\
4,320 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,652 & 0 & 0 & 681,890 & 0 & 0 & 0 & 0 & 0 & 756,542\\
4,330 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,535 & 0 & 0 & 690,645 & 0 & 0 & 0 & 0 & 0 & 765,180\\
4,340 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 76,437 & 0 & 0 & 695,230 & 0 & 0 & 0 & 0 & 0 & 771,667\\
4,350 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,773 & 0 & 0 & 710,686 & 0 & 0 & 0 & 0 & 0 & 785,459\\
4,360 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,645 & 0 & 0 & 680,350 & 0 & 0 & 0 & 0 & 0 & 754,995\\
4,370 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,529 & 0 & 0 & 686,311 & 0 & 0 & 0 & 0 & 0 & 760,840\\
4,380 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 76,092 & 0 & 0 & 694,920 & 0 & 0 & 0 & 0 & 0 & 771,012\\
4,390 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,767 & 0 & 0 & 718,674 & 0 & 0 & 0 & 0 & 0 & 793,441\\
4,400 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,636 & 0 & 0 & 683,425 & 0 & 0 & 0 & 0 & 0 & 758,061\\
4,410 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,528 & 0 & 0 & 683,283 & 0 & 0 & 0 & 0 & 0 & 757,811\\
4,420 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 75,956 & 0 & 0 & 691,688 & 0 & 0 & 0 & 0 & 0 & 767,644\\
4,430 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,773 & 0 & 0 & 683,372 & 0 & 0 & 0 & 0 & 0 & 758,145\\
4,440 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,637 & 0 & 0 & 692,466 & 0 & 0 & 0 & 0 & 0 & 767,103\\
4,450 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,528 & 0 & 0 & 711,607 & 0 & 0 & 0 & 0 & 0 & 786,135\\
4,460 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 76,186 & 0 & 0 & 683,425 & 0 & 0 & 0 & 0 & 0 & 759,611\\
4,470 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,772 & 0 & 0 & 685,775 & 0 & 0 & 0 & 0 & 0 & 760,547\\
4,480 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,631 & 0 & 0 & 692,465 & 0 & 0 & 0 & 0 & 0 & 767,096\\
4,490 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,510 & 0 & 0 & 678,463 & 0 & 0 & 0 & 0 & 0 & 752,973\\
4,500 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 75,211 & 0 & 0 & 683,466 & 0 & 0 & 0 & 0 & 0 & 758,677\\
4,510 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,696 & 0 & 0 & 697,955 & 0 & 0 & 0 & 0 & 0 & 772,651\\
4,520 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,558 & 0 & 0 & 684,395 & 0 & 0 & 0 & 0 & 0 & 758,953\\
4,530 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 77,692 & 0 & 0 & 698,519 & 0 & 0 & 0 & 0 & 0 & 776,211\\
4,540 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,774 & 0 & 0 & 683,628 & 0 & 0 & 0 & 0 & 0 & 758,402\\
4,550 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,626 & 0 & 0 & 698,558 & 0 & 0 & 0 & 0 & 0 & 773,184\\
4,560 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,504 & 0 & 0 & 684,689 & 0 & 0 & 0 & 0 & 0 & 759,193\\
4,570 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,806 & 0 & 0 & 678,212 & 0 & 0 & 0 & 0 & 0 & 753,018\\
4,580 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,664 & 0 & 0 & 694,425 & 0 & 0 & 0 & 0 & 0 & 769,089\\
4,590 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,532 & 0 & 0 & 683,202 & 0 & 0 & 0 & 0 & 0 & 757,734\\
4,600 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 76,186 & 0 & 0 & 698,589 & 0 & 0 & 0 & 0 & 0 & 774,775\\
4,610 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,748 & 0 & 0 & 685,775 & 0 & 0 & 0 & 0 & 0 & 760,523\\
4,620 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,617 & 0 & 0 & 718,889 & 0 & 0 & 0 & 0 & 0 & 793,506\\
4,630 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,503 & 0 & 0 & 694,412 & 0 & 0 & 0 & 0 & 0 & 768,915\\
4,640 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,574 & 0 & 0 & 683,425 & 0 & 0 & 0 & 0 & 0 & 769,999\\
4,650 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 77,543 & 0 & 0 & 707,652 & 0 & 0 & 0 & 0 & 0 & 785,195\\
4,660 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,781 & 0 & 0 & 694,528 & 0 & 0 & 0 & 0 & 0 & 769,309\\
4,670 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,683 & 0 & 0 & 694,927 & 0 & 0 & 0 & 0 & 0 & 769,610\\
4,680 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,575 & 0 & 0 & 692,465 & 0 & 0 & 0 & 0 & 0 & 779,040\\
4,690 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 77,652 & 0 & 0 & 693,647 & 0 & 0 & 0 & 0 & 0 & 771,299\\
4,700 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,785 & 0 & 0 & 692,464 & 0 & 0 & 0 & 0 & 0 & 767,249\\
4,710 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,657 & 0 & 0 & 692,206 & 0 & 0 & 0 & 0 & 0 & 766,863\\
4,720 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,291 & 0 & 0 & 694,674 & 0 & 0 & 0 & 0 & 0 & 780,965\\
4,730 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 77,543 & 0 & 0 & 692,256 & 0 & 0 & 0 & 0 & 0 & 769,799\\
4,740 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,806 & 0 & 0 & 684,019 & 0 & 0 & 0 & 0 & 0 & 758,825\\
4,750 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,697 & 0 & 0 & 708,533 & 0 & 0 & 0 & 0 & 0 & 783,230\\
4,760 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,573 & 0 & 0 & 685,349 & 0 & 0 & 0 & 0 & 0 & 771,922\\
4,770 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 82,967 & 0 & 0 & 694,287 & 0 & 0 & 0 & 0 & 0 & 777,254\\
4,780 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 75,732 & 0 & 0 & 684,333 & 0 & 0 & 0 & 0 & 0 & 760,065\\
4,790 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,773 & 0 & 0 & 698,334 & 0 & 0 & 0 & 0 & 0 & 773,107\\
4,800 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,648 & 0 & 0 & 688,826 & 0 & 0 & 0 & 0 & 0 & 763,474\\
4,810 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 83,905 & 0 & 0 & 685,349 & 0 & 0 & 0 & 0 & 0 & 769,254\\
4,820 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 77,708 & 0 & 0 & 684,057 & 0 & 0 & 0 & 0 & 0 & 761,765\\
4,830 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 75,184 & 0 & 0 & 692,465 & 0 & 0 & 0 & 0 & 0 & 767,649\\
4,840 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,741 & 0 & 0 & 710,686 & 0 & 0 & 0 & 0 & 0 & 785,427\\
4,850 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 87,318 & 0 & 0 & 685,349 & 0 & 0 & 0 & 0 & 0 & 772,667\\
4,860 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 84,149 & 0 & 0 & 692,464 & 0 & 0 & 0 & 0 & 0 & 776,613\\
4,870 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 76,581 & 0 & 0 & 717,893 & 0 & 0 & 0 & 0 & 0 & 794,474\\
4,880 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,858 & 0 & 0 & 707,011 & 0 & 0 & 0 & 0 & 0 & 781,869\\
4,890 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,705 & 0 & 0 & 698,558 & 0 & 0 & 0 & 0 & 0 & 773,263\\
4,900 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,576 & 0 & 0 & 699,506 & 0 & 0 & 0 & 0 & 0 & 786,082\\
4,910 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 83,388 & 0 & 0 & 694,682 & 0 & 0 & 0 & 0 & 0 & 778,070\\
4,920 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 76,111 & 0 & 0 & 692,465 & 0 & 0 & 0 & 0 & 0 & 768,576\\
4,930 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,783 & 0 & 0 & 694,707 & 0 & 0 & 0 & 0 & 0 & 769,490\\
4,940 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,681 & 0 & 0 & 696,314 & 0 & 0 & 0 & 0 & 0 & 770,995\\
4,950 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,574 & 0 & 0 & 694,832 & 0 & 0 & 0 & 0 & 0 & 781,406\\
4,960 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 82,983 & 0 & 0 & 694,345 & 0 & 0 & 0 & 0 & 0 & 777,328\\
4,970 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 75,967 & 0 & 0 & 685,497 & 0 & 0 & 0 & 0 & 0 & 761,464\\
4,980 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 75,107 & 0 & 0 & 685,349 & 0 & 0 & 0 & 0 & 0 & 760,456\\
4,990 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,763 & 0 & 0 & 687,929 & 0 & 0 & 0 & 0 & 0 & 762,692\\
5,000 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,579 & 0 & 0 & 689,266 & 0 & 0 & 0 & 0 & 0 & 775,845\\
5,010 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 83,449 & 0 & 0 & 688,831 & 0 & 0 & 0 & 0 & 0 & 772,280\\
5,020 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 77,543 & 0 & 0 & 688,822 & 0 & 0 & 0 & 0 & 0 & 766,365\\
5,030 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 75,612 & 0 & 0 & 695,474 & 0 & 0 & 0 & 0 & 0 & 771,086\\
5,040 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,768 & 0 & 0 & 753,927 & 0 & 0 & 0 & 0 & 0 & 828,695\\
5,050 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,576 & 0 & 0 & 694,002 & 0 & 0 & 0 & 0 & 0 & 780,578\\
5,060 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 84,150 & 0 & 0 & 696,143 & 0 & 0 & 0 & 0 & 0 & 780,293\\
5,070 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 81,046 & 0 & 0 & 704,489 & 0 & 0 & 0 & 0 & 0 & 785,535\\
5,080 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 75,955 & 0 & 0 & 706,583 & 0 & 0 & 0 & 0 & 0 & 782,538\\
5,090 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,781 & 0 & 0 & 707,757 & 0 & 0 & 0 & 0 & 0 & 782,538\\
5,100 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,576 & 0 & 0 & 716,970 & 0 & 0 & 0 & 0 & 0 & 803,546\\
5,110 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 83,470 & 0 & 0 & 730,730 & 0 & 0 & 0 & 0 & 0 & 814,200\\
5,120 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 81,191 & 0 & 0 & 706,583 & 0 & 0 & 0 & 0 & 0 & 787,774\\
5,130 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 76,010 & 0 & 0 & 710,686 & 0 & 0 & 0 & 0 & 0 & 786,696\\
5,140 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74,799 & 0 & 0 & 723,220 & 0 & 0 & 0 & 0 & 0 & 798,019\\
5,150 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,576 & 0 & 0 & 755,220 & 0 & 0 & 0 & 0 & 0 & 841,796\\
5,160 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 83,667 & 0 & 0 & 700,991 & 0 & 0 & 0 & 0 & 0 & 784,658\\
5,170 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 81,513 & 0 & 0 & 706,581 & 0 & 0 & 0 & 0 & 0 & 788,094\\
5,180 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 83,019 & 0 & 0 & 708,151 & 0 & 0 & 0 & 0 & 0 & 791,170\\
5,190 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 75,326 & 0 & 0 & 719,019 & 0 & 0 & 0 & 0 & 0 & 794,345\\
5,200 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 81,394 & 0 & 0 & 754,648 & 0 & 0 & 0 & 0 & 0 & 836,042\\
5,210 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 76,077 & 0 & 0 & 704,019 & 0 & 0 & 0 & 0 & 0 & 780,096\\
5,220 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 75,694 & 0 & 0 & 706,583 & 0 & 0 & 0 & 0 & 0 & 782,277\\
5,230 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,575 & 0 & 0 & 715,928 & 0 & 0 & 0 & 0 & 0 & 802,503\\
5,240 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 83,639 & 0 & 0 & 750,619 & 0 & 0 & 0 & 0 & 0 & 834,258\\
5,250 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 81,730 & 0 & 0 & 705,634 & 0 & 0 & 0 & 0 & 0 & 787,364\\
5,260 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 77,675 & 0 & 0 & 712,010 & 0 & 0 & 0 & 0 & 0 & 789,685\\
5,270 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 75,914 & 0 & 0 & 727,469 & 0 & 0 & 0 & 0 & 0 & 803,383\\
5,280 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 90,034 & 0 & 0 & 703,931 & 0 & 0 & 0 & 0 & 0 & 793,965\\
5,290 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 85,714 & 0 & 0 & 706,583 & 0 & 0 & 0 & 0 & 0 & 792,297\\
5,300 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 82,527 & 0 & 0 & 724,242 & 0 & 0 & 0 & 0 & 0 & 806,769\\
5,310 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 82,957 & 0 & 0 & 705,506 & 0 & 0 & 0 & 0 & 0 & 788,463\\
5,320 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,472 & 0 & 0 & 713,640 & 0 & 0 & 0 & 0 & 0 & 800,112\\
5,330 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 84,228 & 0 & 0 & 755,223 & 0 & 0 & 0 & 0 & 0 & 839,451\\
5,340 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,289 & 0 & 0 & 710,534 & 0 & 0 & 0 & 0 & 0 & 796,823\\
5,350 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 76,684 & 0 & 0 & 745,819 & 0 & 0 & 0 & 0 & 0 & 822,503\\
5,360 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 81,319 & 0 & 0 & 708,533 & 0 & 0 & 0 & 0 & 0 & 789,852\\
5,370 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 82,062 & 0 & 0 & 726,715 & 0 & 0 & 0 & 0 & 0 & 808,777\\
5,380 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 81,860 & 0 & 0 & 706,583 & 0 & 0 & 0 & 0 & 0 & 788,443\\
5,390 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 84,914 & 0 & 0 & 715,536 & 0 & 0 & 0 & 0 & 0 & 800,450\\
5,400 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 87,812 & 0 & 0 & 754,249 & 0 & 0 & 0 & 0 & 0 & 842,061\\
5,410 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 77,293 & 0 & 0 & 710,764 & 0 & 0 & 0 & 0 & 0 & 788,057\\
5,420 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 77,691 & 0 & 0 & 755,223 & 0 & 0 & 0 & 0 & 0 & 832,914\\
5,430 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 78,001 & 0 & 0 & 712,819 & 0 & 0 & 0 & 0 & 0 & 790,820\\
5,440 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 81,263 & 0 & 0 & 737,941 & 0 & 0 & 0 & 0 & 0 & 819,204\\
5,450 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 78,780 & 0 & 0 & 712,834 & 0 & 0 & 0 & 0 & 0 & 791,614\\
5,460 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 79,962 & 0 & 0 & 706,583 & 0 & 0 & 0 & 0 & 0 & 786,545\\
5,470 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 78,776 & 0 & 0 & 726,113 & 0 & 0 & 0 & 0 & 0 & 804,889\\
5,480 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 88,575 & 0 & 0 & 754,894 & 0 & 0 & 0 & 0 & 0 & 843,469\\
5,490 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 81,519 & 0 & 0 & 706,583 & 0 & 0 & 0 & 0 & 0 & 788,102\\
5,500 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 81,270 & 0 & 0 & 721,904 & 0 & 0 & 0 & 0 & 0 & 803,174\\
5,510 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 85,632 & 0 & 0 & 706,583 & 0 & 0 & 0 & 0 & 0 & 792,215\\
5,520 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,576 & 0 & 0 & 755,224 & 0 & 0 & 0 & 0 & 0 & 841,800\\
5,530 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,573 & 0 & 0 & 764,977 & 0 & 0 & 0 & 0 & 0 & 851,550\\
5,540 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,894 & 0 & 0 & 770,845 & 0 & 0 & 0 & 0 & 0 & 857,739\\
5,550 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,575 & 0 & 0 & 727,227 & 0 & 0 & 0 & 0 & 0 & 813,802\\
5,560 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,575 & 0 & 0 & 737,466 & 0 & 0 & 0 & 0 & 0 & 824,041\\
5,570 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,861 & 0 & 0 & 765,471 & 0 & 0 & 0 & 0 & 0 & 852,332\\
5,580 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,573 & 0 & 0 & 779,781 & 0 & 0 & 0 & 0 & 0 & 866,354\\
5,590 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,580 & 0 & 0 & 728,597 & 0 & 0 & 0 & 0 & 0 & 815,177\\
5,600 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,572 & 0 & 0 & 754,787 & 0 & 0 & 0 & 0 & 0 & 841,359\\
5,610 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 84,150 & 0 & 0 & 762,034 & 0 & 0 & 0 & 0 & 0 & 846,184\\
5,620 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,576 & 0 & 0 & 852,409 & 0 & 0 & 0 & 0 & 0 & 938,985\\
5,630 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,287 & 0 & 0 & 784,723 & 0 & 0 & 0 & 0 & 0 & 871,010\\
5,640 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 85,774 & 0 & 0 & 758,824 & 0 & 0 & 0 & 0 & 0 & 844,598\\
5,650 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 83,326 & 0 & 0 & 872,746 & 0 & 0 & 0 & 0 & 0 & 956,072\\
5,660 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 81,864 & 0 & 0 & 838,511 & 0 & 0 & 0 & 0 & 0 & 920,375\\
5,670 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 94,570 & 0 & 0 & 864,926 & 0 & 0 & 0 & 0 & 0 & 959,496\\
5,680 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 82,434 & 0 & 0 & 760,567 & 0 & 0 & 0 & 0 & 0 & 843,001\\
5,690 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 82,097 & 0 & 0 & 734,777 & 0 & 0 & 0 & 0 & 0 & 816,874\\
5,700 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 82,184 & 0 & 0 & 755,224 & 0 & 0 & 0 & 0 & 0 & 837,408\\
5,710 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 92,125 & 0 & 0 & 908,445 & 0 & 0 & 0 & 0 & 0 & 1,000,570\\
5,720 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 89,279 & 0 & 0 & 790,889 & 0 & 0 & 0 & 0 & 0 & 880,168\\
5,730 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,882 & 0 & 0 & 876,105 & 0 & 0 & 0 & 0 & 0 & 962,987\\
5,740 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,538 & 0 & 0 & 934,965 & 0 & 0 & 0 & 0 & 0 & 1,021,503\\
5,750 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 84,165 & 0 & 0 & 792,282 & 0 & 0 & 0 & 0 & 0 & 876,447\\
5,760 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 82,983 & 0 & 0 & 890,925 & 0 & 0 & 0 & 0 & 0 & 973,908\\
5,770 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 82,911 & 0 & 0 & 865,283 & 0 & 0 & 0 & 0 & 0 & 948,194\\
5,780 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 82,833 & 0 & 0 & 922,679 & 0 & 0 & 0 & 0 & 0 & 1,005,512\\
5,790 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 92,962 & 0 & 0 & 954,443 & 0 & 0 & 0 & 0 & 0 & 1,047,405\\
5,800 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 89,278 & 0 & 0 & 829,482 & 0 & 0 & 0 & 0 & 0 & 918,760\\
5,810 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,795 & 0 & 0 & 995,462 & 0 & 0 & 0 & 0 & 0 & 1,082,257\\
5,820 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,791 & 0 & 0 & 903,693 & 0 & 0 & 0 & 0 & 0 & 990,484\\
5,830 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 84,877 & 0 & 0 & 846,517 & 0 & 0 & 0 & 0 & 0 & 931,394\\
5,840 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 83,649 & 0 & 0 & 917,649 & 0 & 0 & 0 & 0 & 0 & 1,001,298\\
5,850 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 83,738 & 0 & 0 & 999,909 & 0 & 0 & 0 & 0 & 0 & 1,083,647\\
5,860 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 83,427 & 0 & 0 & 898,374 & 0 & 0 & 0 & 0 & 0 & 981,801\\
5,870 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,789 & 0 & 0 & 998,852 & 0 & 0 & 0 & 0 & 0 & 1,098,641\\
5,880 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 92,904 & 0 & 0 & 971,761 & 0 & 0 & 0 & 0 & 0 & 1,064,665\\
5,890 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 92,395 & 0 & 0 & 960,588 & 0 & 0 & 0 & 0 & 0 & 1,052,983\\
5,900 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 88,579 & 0 & 0 & 931,762 & 0 & 0 & 0 & 0 & 0 & 1,020,341\\
5,910 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,573 & 0 & 0 & 967,654 & 0 & 0 & 0 & 0 & 0 & 1,054,227\\
5,920 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,278 & 0 & 0 & 993,976 & 0 & 0 & 0 & 0 & 0 & 1,080,254\\
5,930 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 84,149 & 0 & 0 & 999,909 & 0 & 0 & 0 & 0 & 0 & 1,084,058\\
5,940 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 97,803 & 0 & 0 & 910,671 & 0 & 0 & 0 & 0 & 0 & 1,008,474\\
5,950 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 91,703 & 0 & 0 & 993,867 & 0 & 0 & 0 & 0 & 0 & 1,085,570\\
5,960 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 87,892 & 0 & 0 & 987,170 & 0 & 0 & 0 & 0 & 0 & 1,075,062\\
5,970 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,907 & 0 & 0 & 999,909 & 0 & 0 & 0 & 0 & 0 & 1,086,816\\
5,980 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,538 & 0 & 0 & 966,775 & 0 & 0 & 0 & 0 & 0 & 1,053,313\\
5,990 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 85,610 & 0 & 0 & 989,803 & 0 & 0 & 0 & 0 & 0 & 1,075,413\\
6,000 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 84,509 & 0 & 0 & 982,926 & 0 & 0 & 0 & 0 & 0 & 1,067,435\\
6,010 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 84,539 & 0 & 0 & 979,646 & 0 & 0 & 0 & 0 & 0 & 1,064,185\\
6,020 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 84,245 & 0 & 0 & 996,570 & 0 & 0 & 0 & 0 & 0 & 1,080,815\\
6,030 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 93,511 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,093,504\\
6,040 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 88,048 & 0 & 0 & 985,097 & 0 & 0 & 0 & 0 & 0 & 1,073,145\\
6,050 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,570 & 0 & 0 & 983,250 & 0 & 0 & 0 & 0 & 0 & 1,069,820\\
6,060 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 84,851 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,084,844\\
6,070 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 94,962 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,094,955\\
6,080 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 89,222 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,089,215\\
6,090 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,571 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,086,564\\
6,100 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 84,829 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,084,822\\
6,110 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 94,822 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,094,815\\
6,120 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 89,244 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,089,237\\
6,130 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,569 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,086,562\\
6,140 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 84,850 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,084,843\\
6,150 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 94,570 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,094,563\\
6,160 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 88,996 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,088,989\\
6,170 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,537 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,086,530\\
6,180 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 84,797 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,084,790\\
6,190 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,023 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,016\\
6,200 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 89,729 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,089,722\\
6,210 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 86,576 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,086,569\\
6,220 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 84,900 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,084,893\\
6,230 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,838 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,831\\
6,240 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,582 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,575\\
6,250 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,577 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,570\\
6,260 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
6,270 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,586 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,579\\
6,280 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,579 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,572\\
6,290 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,575 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,568\\
6,300 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
6,310 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 103,429 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,103,422\\
6,320 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,592 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,585\\
6,330 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,582 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,575\\
6,340 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,578 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,571\\
6,350 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,575 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,568\\
6,360 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
6,370 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 103,045 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,103,038\\
6,380 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,586 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,579\\
6,390 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,580 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,573\\
6,400 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,575 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,568\\
6,410 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
6,420 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,571 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,564\\
6,430 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,593 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,586\\
6,440 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,582 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,575\\
6,450 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,578 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,571\\
6,460 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,574 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,567\\
6,470 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
6,480 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 103,451 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,103,444\\
6,490 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,586 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,579\\
6,500 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,579 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,572\\
6,510 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,575 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,568\\
6,520 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
6,530 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 101,812 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,101,805\\
6,540 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,586 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,579\\
6,550 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,578 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,571\\
6,560 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
6,570 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,571 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,564\\
6,580 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,749 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,742\\
6,590 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,583 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,576\\
6,600 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,578 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,571\\
6,610 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
6,620 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,571 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,564\\
6,630 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,722 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,715\\
6,640 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,582 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,575\\
6,650 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,575 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,568\\
6,660 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
6,670 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 105,631 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,105,624\\
6,680 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,586 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,579\\
6,690 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,579 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,572\\
6,700 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
6,710 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,571 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,564\\
6,720 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,754 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,747\\
6,730 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,581 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,574\\
6,740 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,575 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,568\\
6,750 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
6,760 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,571 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,564\\
6,770 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,761 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,754\\
6,780 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,584 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,577\\
6,790 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,577 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,570\\
6,800 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
6,810 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,571 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,564\\
6,820 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,653 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,646\\
6,830 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,581 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,574\\
6,840 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,575 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,568\\
6,850 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
6,860 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 105,369 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,105,362\\
6,870 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,722 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,715\\
6,880 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,585 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,578\\
6,890 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,578 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,571\\
6,900 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,575 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,568\\
6,910 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
6,920 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,571 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,564\\
6,930 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 106,632 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,106,625\\
6,940 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,722 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,715\\
6,950 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,582 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,575\\
6,960 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,576 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,569\\
6,970 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
6,980 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,571 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,564\\
6,990 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 105,369 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,105,362\\
7,000 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,753 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,746\\
7,010 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,586 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,579\\
7,020 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,580 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,573\\
7,030 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,576 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,569\\
7,040 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
7,050 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,571 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,564\\
7,060 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 103,413 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,103,406\\
7,070 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,722 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,715\\
7,080 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,585 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,578\\
7,090 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,578 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,571\\
7,100 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
7,110 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
7,120 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 103,514 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,103,507\\
7,130 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,691 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,684\\
7,140 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,581 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,574\\
7,150 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,578 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,571\\
7,160 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
7,170 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,571 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,564\\
7,180 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 104,917 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,104,910\\
7,190 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,725 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,718\\
7,200 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,585 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,578\\
7,210 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,578 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,571\\
7,220 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,575 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,568\\
7,230 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
7,240 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,571 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,564\\
7,250 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 107,069 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,107,062\\
7,260 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,795 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,788\\
7,270 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,586 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,579\\
7,280 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,583 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,576\\
7,290 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,579 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,572\\
7,300 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,575 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,568\\
7,310 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
7,320 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,571 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,564\\
7,330 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 101,048 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,101,041\\
7,340 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,747 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,740\\
7,350 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 101,736 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,101,729\\
7,360 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,571 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,564\\
7,370 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
7,380 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,571 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,564\\
7,390 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,570 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,563\\
7,400 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 101,736 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,101,729\\
7,410 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,753 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,746\\
7,420 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,586 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,579\\
7,430 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,582 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,575\\
7,440 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,579 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,572\\
7,450 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,575 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,568\\
7,460 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,573 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,566\\
7,470 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
7,480 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,571 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,564\\
7,490 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,571 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,564\\
7,500 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 105,071 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,105,064\\
7,510 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 100,310 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,100,303\\
7,520 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,653 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,646\\
7,530 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,586 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,579\\
7,540 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,580 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,573\\
7,550 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,578 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,571\\
7,560 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,575 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,568\\
7,570 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
7,580 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
7,590 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,571 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,564\\
7,600 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,570 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,563\\
7,610 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 106,587 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,106,580\\
7,620 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 100,628 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,100,621\\
7,630 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,691 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,684\\
7,640 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,586 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,579\\
7,650 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,580 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,573\\
7,660 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,578 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,571\\
7,670 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,575 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,568\\
7,680 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
7,690 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
7,700 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,571 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,564\\
7,710 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,571 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,564\\
7,720 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,313 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,306\\
7,730 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 101,736 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,101,729\\
7,740 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,759 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,752\\
7,750 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,586 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,579\\
7,760 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,584 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,577\\
7,770 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,579 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,572\\
7,780 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,578 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,571\\
7,790 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,575 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,568\\
7,800 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
7,810 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
7,820 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,571 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,564\\
7,830 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,782 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,775\\
7,840 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 103,473 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,103,466\\
7,850 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,797 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,790\\
7,860 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,593 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,586\\
7,870 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,586 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,579\\
7,880 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,580 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,573\\
7,890 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,579 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,572\\
7,900 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
7,910 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,586 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,579\\
7,920 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,585 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,578\\
7,930 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,579 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,572\\
7,940 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,578 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,571\\
7,950 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,575 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,568\\
7,960 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
7,970 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
7,980 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,571 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,564\\
7,990 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,100 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,110,093\\
8,000 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,296 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,289\\
8,010 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 101,728 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,101,721\\
8,020 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,760 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,753\\
8,030 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,586 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,579\\
8,040 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,584 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,577\\
8,050 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,579 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,572\\
8,060 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,578 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,571\\
8,070 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,575 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,568\\
8,080 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
8,090 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
8,100 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,571 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,564\\
8,110 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,154 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,110,147\\
8,120 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,311 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,304\\
8,130 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 102,426 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,102,419\\
8,140 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,792 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,785\\
8,150 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,591 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,584\\
8,160 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,586 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,579\\
8,170 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,580 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,573\\
8,180 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,578 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,571\\
8,190 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,575 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,568\\
8,200 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
8,210 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
8,220 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,571 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,564\\
8,230 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,571 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,564\\
8,240 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,769 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,762\\
8,250 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 106,587 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,106,580\\
8,260 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 101,180 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,101,173\\
8,270 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,753 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,746\\
8,280 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,586 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,579\\
8,290 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,584 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,577\\
8,300 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,579 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,572\\
8,310 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,578 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,571\\
8,320 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,575 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,568\\
8,330 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
8,340 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
8,350 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,571 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,564\\
8,360 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,078 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,071\\
8,370 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,748 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,741\\
8,380 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 108,518 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,108,511\\
8,390 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 101,728 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,101,721\\
8,400 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,760 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,753\\
8,410 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 105,048 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,105,041\\
8,420 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,586 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,579\\
8,430 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,579 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,572\\
8,440 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,577 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,570\\
8,450 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
8,460 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 117,117 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,117,110\\
8,470 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,818 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,811\\
8,480 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 108,518 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,108,511\\
8,490 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 101,050 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,101,043\\
8,500 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,591 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,584\\
8,510 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,581 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,574\\
8,520 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,579 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,572\\
8,530 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,576 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,569\\
8,540 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,575 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,568\\
8,550 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
8,560 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 118,602 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,118,595\\
8,570 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,103 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,110,096\\
8,580 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,620 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,613\\
8,590 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 103,339 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,103,332\\
8,600 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 101,055 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,101,048\\
8,610 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,722 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,715\\
8,620 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,583 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,576\\
8,630 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,578 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,571\\
8,640 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,574 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,567\\
8,650 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 121,411 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,121,404\\
8,660 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,182 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,175\\
8,670 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,125 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,110,118\\
8,680 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,571 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,564\\
8,690 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 101,970 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,101,963\\
8,700 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,760 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,753\\
8,710 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,585 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,578\\
8,720 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 101,783 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,101,776\\
8,730 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,722 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,715\\
8,740 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,585 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,578\\
8,750 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,578 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,571\\
8,760 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,578 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,571\\
8,770 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,575 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,568\\
8,780 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,572 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,565\\
8,790 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 117,955 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,117,948\\
8,800 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,765 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,111,758\\
8,810 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,973 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,966\\
8,820 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,667 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,660\\
8,830 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 106,640 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,106,633\\
8,840 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 101,941 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,101,934\\
8,850 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,724 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,717\\
8,860 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 106,680 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,106,673\\
8,870 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 102,938 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,102,931\\
8,880 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 101,143 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,101,136\\
8,890 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,779 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,772\\
8,900 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,592 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,585\\
8,910 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,586 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,579\\
8,920 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,580 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,573\\
8,930 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,578 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,571\\
8,940 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,575 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,568\\
8,950 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 117,966 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,117,959\\
8,960 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 120,042 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,120,035\\
8,970 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,182 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,175\\
8,980 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,658 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,111,651\\
8,990 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,855 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,848\\
9,000 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,472 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,465\\
9,010 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 105,676 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,105,669\\
9,020 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 104,788 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,104,781\\
9,030 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 102,874 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,102,867\\
9,040 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 101,143 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,101,136\\
9,050 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,761 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,754\\
9,060 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,589 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,582\\
9,070 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,586 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,579\\
9,080 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,580 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,573\\
9,090 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 120,042 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,120,035\\
9,100 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,017 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,113,010\\
9,110 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,017 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,010\\
9,120 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,640 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,110,633\\
9,130 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,787 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,780\\
9,140 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,304 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,297\\
9,150 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 106,288 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,106,281\\
9,160 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 104,859 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,104,852\\
9,170 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 103,144 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,103,137\\
9,180 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 101,255 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,101,248\\
9,190 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,795 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,788\\
9,200 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,685 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,678\\
9,210 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,586 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,579\\
9,220 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 119,983 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,119,976\\
9,230 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,706 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,699\\
9,240 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,238 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,231\\
9,250 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,755 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,111,748\\
9,260 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,970 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,963\\
9,270 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,620 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,613\\
9,280 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 107,275 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,107,268\\
9,290 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 106,387 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,106,380\\
9,300 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 105,886 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,105,879\\
9,310 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 104,984 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,104,977\\
9,320 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 103,404 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,103,397\\
9,330 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,472 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,465\\
9,340 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,156 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,149\\
9,350 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,939 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,932\\
9,360 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 108,917 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,108,910\\
9,370 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 106,061 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,106,054\\
9,380 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 104,749 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,104,742\\
9,390 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 101,143 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,101,136\\
9,400 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,792 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,785\\
9,410 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 120,145 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,120,138\\
9,420 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,380 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,373\\
9,430 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,152 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,145\\
9,440 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,076 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,110,069\\
9,450 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,648 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,641\\
9,460 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 107,401 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,107,394\\
9,470 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 106,612 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,106,605\\
9,480 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 105,735 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,105,728\\
9,490 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 104,920 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,104,913\\
9,500 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 103,045 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,103,038\\
9,510 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 101,172 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,101,165\\
9,520 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,938 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,931\\
9,530 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,721 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,714\\
9,540 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 120,033 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,120,026\\
9,550 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 116,253 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,116,246\\
9,560 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,355 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,348\\
9,570 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,182 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,175\\
9,580 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 100,133 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,100,126\\
9,590 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,754 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,747\\
9,600 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 122,039 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,122,032\\
9,610 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 117,920 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,117,913\\
9,620 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 103,413 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,103,406\\
9,630 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 101,772 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,101,765\\
9,640 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 100,222 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,100,215\\
9,650 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99,797 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,099,790\\
9,660 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 123,716 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,123,709\\
9,670 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 119,457 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,119,450\\
9,680 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,017 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,113,010\\
9,690 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,372 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,365\\
9,700 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,238 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,231\\
9,710 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,791 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,111,784\\
9,720 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,187 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,110,180\\
9,730 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,782 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,775\\
9,740 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,312 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,305\\
9,750 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 107,184 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,107,177\\
9,760 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 106,456 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,106,449\\
9,770 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 105,149 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,105,142\\
9,780 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 106,440 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,106,433\\
9,790 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 106,640 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,106,633\\
9,800 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 105,813 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,105,806\\
9,810 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 104,842 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,104,835\\
9,820 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 102,426 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,102,419\\
9,830 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 101,050 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,101,043\\
9,840 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 128,199 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,128,192\\
9,850 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 119,983 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,119,976\\
9,860 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 115,233 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,115,226\\
9,870 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,509 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,113,502\\
9,880 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,383 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,376\\
9,890 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,238 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,231\\
9,900 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,765 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,111,758\\
9,910 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,087 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,110,080\\
9,920 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,692 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,685\\
9,930 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 108,664 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,108,657\\
9,940 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 106,640 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,106,633\\
9,950 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 105,688 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,105,681\\
9,960 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 104,899 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,104,892\\
9,970 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 102,951 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,102,944\\
9,980 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 101,299 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,101,292\\
9,990 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 130,571 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,130,564\\
10,000 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 119,992 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,119,985\\
10,010 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 114,325 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,114,318\\
10,020 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,417 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,113,410\\
10,030 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,394 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,387\\
10,040 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,235 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,228\\
10,050 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,726 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,111,719\\
10,060 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,905 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,898\\
10,070 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,452 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,445\\
10,080 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 107,246 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,107,239\\
10,090 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 106,288 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,106,281\\
10,100 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 105,108 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,105,101\\
10,110 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 103,473 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,103,466\\
10,120 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 101,831 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,101,824\\
10,130 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 100,310 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,100,303\\
10,140 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 123,191 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,123,184\\
10,150 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 117,919 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,117,912\\
10,160 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,511 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,113,504\\
10,170 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,511 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,113,504\\
10,180 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,388 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,113,381\\
10,190 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,651 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,644\\
10,200 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,351 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,344\\
10,210 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,221 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,214\\
10,220 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,829 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,111,822\\
10,230 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,215 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,110,208\\
10,240 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,813 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,806\\
10,250 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,391 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,384\\
10,260 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 108,073 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,108,066\\
10,270 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 106,723 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,106,716\\
10,280 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 105,990 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,105,983\\
10,290 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 105,102 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,105,095\\
10,300 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 104,717 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,104,710\\
10,310 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 102,529 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,102,522\\
10,320 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 101,143 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,101,136\\
10,330 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 123,584 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,123,577\\
10,340 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 119,983 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,119,976\\
10,350 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 117,576 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,117,569\\
10,360 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,511 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,113,504\\
10,370 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,393 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,113,386\\
10,380 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,940 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,933\\
10,390 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,553 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,546\\
10,400 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,341 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,334\\
10,410 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,156 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,149\\
10,420 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,717 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,111,710\\
10,430 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,126 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,110,119\\
10,440 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,763 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,756\\
10,450 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,312 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,305\\
10,460 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 107,239 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,107,232\\
10,470 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 106,595 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,106,588\\
10,480 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 105,813 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,105,806\\
10,490 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 105,048 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,105,041\\
10,500 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 104,067 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,104,060\\
10,510 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 101,941 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,101,934\\
10,520 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 123,580 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,123,573\\
10,530 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 119,959 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,119,952\\
10,540 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 117,457 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,117,450\\
10,550 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,511 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,113,504\\
10,560 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,376 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,113,369\\
10,570 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,940 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,933\\
10,580 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,683 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,676\\
10,590 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 130,571 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,130,564\\
10,600 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 105,224 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,105,217\\
10,610 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,391 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,384\\
10,620 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,830 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,111,823\\
10,630 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,221 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,214\\
10,640 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,649 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,642\\
10,650 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,254 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,113,247\\
10,660 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,511 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,113,504\\
10,670 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 117,347 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,117,340\\
10,680 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 138,603 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,138,596\\
10,690 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 104,740 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,104,733\\
10,700 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 104,266 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,104,259\\
10,710 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 131,268 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,131,261\\
10,720 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,312 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,305\\
10,730 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,409 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,402\\
10,740 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 108,664 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,108,657\\
10,750 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,311 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,304\\
10,760 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,312 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,305\\
10,770 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,742 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,735\\
10,780 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,862 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,855\\
10,790 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,650 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,643\\
10,800 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 108,579 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,108,572\\
10,810 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 106,595 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,106,588\\
10,820 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 105,324 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,105,317\\
10,830 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 133,181 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,133,174\\
10,840 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 121,090 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,121,083\\
10,850 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 117,385 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,117,378\\
10,860 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,511 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,113,504\\
10,870 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,910 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,903\\
10,880 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,378 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,371\\
10,890 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,045 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,038\\
10,900 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,187 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,110,180\\
10,910 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,571 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,564\\
10,920 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 107,112 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,107,105\\
10,930 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 105,841 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,105,834\\
10,940 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 104,647 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,104,640\\
10,950 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 123,238 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,123,231\\
10,960 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 117,950 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,117,943\\
10,970 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 119,357 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,119,350\\
10,980 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 121,499 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,121,492\\
10,990 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 118,222 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,118,215\\
11,000 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 116,302 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,116,295\\
11,010 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,511 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,113,504\\
11,020 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,394 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,113,387\\
11,030 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,726 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,719\\
11,040 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,374 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,367\\
11,050 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,869 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,111,862\\
11,060 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,936 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,929\\
11,070 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,405 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,398\\
11,080 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 107,115 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,107,108\\
11,090 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 105,928 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,105,921\\
11,100 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 104,899 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,104,892\\
11,110 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 125,024 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,125,017\\
11,120 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 120,042 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,120,035\\
11,130 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 117,862 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,117,855\\
11,140 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 114,127 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,114,120\\
11,150 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,400 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,113,393\\
11,160 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,870 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,863\\
11,170 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,341 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,112,334\\
11,180 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,787 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,111,780\\
11,190 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,954 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,947\\
11,200 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,370 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,109,363\\
11,210 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 106,812 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,106,805\\
11,220 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 105,499 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,105,492\\
11,230 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 126,710 & 0 & 0 & 999,993 & 0 & 0 & 0 & 0 & 0 & 1,126,703\\
11,240 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 119,655 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 119,655\\
11,250 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 116,323 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 116,323\\
11,260 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 114,303 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 114,303\\
11,270 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,511 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,511\\
11,280 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,120 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,120\\
11,290 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,686 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,686\\
11,300 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,348 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,348\\
11,310 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,245 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,245\\
11,320 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,969 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,969\\
11,330 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,476 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,476\\
11,340 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,165 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,165\\
11,350 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,224 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,224\\
11,360 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,216 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,216\\
11,370 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,393 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,393\\
11,380 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,319 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,319\\
11,390 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,035 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,035\\
11,400 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,690 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,690\\
11,410 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,215 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,215\\
11,420 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,815 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,815\\
11,430 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,137 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,137\\
11,440 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,755 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,755\\
11,450 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,311 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,311\\
11,460 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,845 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,845\\
11,470 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,648 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,648\\
11,480 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,327 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,327\\
11,490 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,322 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,322\\
11,500 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,321 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,321\\
11,510 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 145,285 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 145,285\\
11,520 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,002 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,002\\
11,530 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,485 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,485\\
11,540 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,640 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,640\\
11,550 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,864 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,864\\
11,560 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,712 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,712\\
11,570 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,329 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,329\\
11,580 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,323 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,323\\
11,590 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 140,075 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 140,075\\
11,600 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 127,625 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 127,625\\
11,610 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 123,250 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 123,250\\
11,620 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 119,998 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 119,998\\
11,630 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 117,981 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 117,981\\
11,640 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 116,811 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 116,811\\
11,650 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 116,014 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 116,014\\
11,660 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 115,247 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 115,247\\
11,670 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 114,386 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 114,386\\
11,680 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,954 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,954\\
11,690 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,820 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,820\\
11,700 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,511 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,511\\
11,710 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,376 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,376\\
11,720 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,964 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,964\\
11,730 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,703 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,703\\
11,740 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,383 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,383\\
11,750 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,317 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,317\\
11,760 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,035 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,035\\
11,770 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,695 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,695\\
11,780 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,201 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,201\\
11,790 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,813 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,813\\
11,800 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,571 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,571\\
11,810 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,327 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,327\\
11,820 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,322 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,322\\
11,830 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 133,543 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 133,543\\
11,840 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 125,707 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 125,707\\
11,850 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 123,019 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 123,019\\
11,860 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 119,828 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 119,828\\
11,870 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 117,920 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 117,920\\
11,880 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 116,774 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 116,774\\
11,890 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 116,069 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 116,069\\
11,900 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 115,275 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 115,275\\
11,910 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 114,391 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 114,391\\
11,920 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,956 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,956\\
11,930 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,820 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,820\\
11,940 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,511 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,511\\
11,950 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,402 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,402\\
11,960 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,017 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,017\\
11,970 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,733 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,733\\
11,980 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,205 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,205\\
11,990 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,901 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,901\\
12,000 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,649 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,649\\
12,010 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,371 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,371\\
12,020 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,246 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,246\\
12,030 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,970 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,970\\
12,040 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,612 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,612\\
12,050 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,256 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,256\\
12,060 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,650 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,650\\
12,070 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,648 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,648\\
12,080 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,327 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,327\\
12,090 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 152,682 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 152,682\\
12,100 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,552 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,552\\
12,110 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,327 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,327\\
12,120 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 152,708 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 152,708\\
12,130 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 130,840 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 130,840\\
12,140 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 125,501 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 125,501\\
12,150 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 119,977 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 119,977\\
12,160 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 116,707 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 116,707\\
12,170 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 115,835 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 115,835\\
12,180 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 114,325 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 114,325\\
12,190 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,813 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,813\\
12,200 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,402 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,402\\
12,210 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,893 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,893\\
12,220 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,633 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,633\\
12,230 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,342 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,342\\
12,240 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,137 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,137\\
12,250 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,216 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,216\\
12,260 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,624 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,624\\
12,270 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 152,787 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 152,787\\
12,280 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 126,967 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 126,967\\
12,290 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 122,051 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 122,051\\
12,300 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 119,460 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 119,460\\
12,310 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 117,706 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 117,706\\
12,320 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 116,447 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 116,447\\
12,330 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 116,117 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 116,117\\
12,340 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 115,545 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 115,545\\
12,350 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 114,375 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 114,375\\
12,360 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,570 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,570\\
12,370 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,336 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,336\\
12,380 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,708 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,708\\
12,390 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,342 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,342\\
12,400 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,839 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,839\\
12,410 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,221 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,221\\
12,420 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,742 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,742\\
12,430 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 135,416 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 135,416\\
12,440 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 123,291 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 123,291\\
12,450 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 118,687 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 118,687\\
12,460 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 116,429 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 116,429\\
12,470 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 115,698 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 115,698\\
12,480 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 114,412 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 114,412\\
12,490 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,956 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,956\\
12,500 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,511 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,511\\
12,510 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,377 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,377\\
12,520 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\
		\hline
	\end{longtable}
\end{center}

==> ECI_size_no_limit_table.tex <==
\begin{center}

	\tiny
	%		
	\begin{longtable}{m{0.028\textwidth}|m{0.028\textwidth}m{0.035\textwidth}m{0.035\textwidth}m{0.035\textwidth}m{0.035\textwidth}m{0.035\textwidth}m{0.035\textwidth}m{0.035\textwidth}m{0.028\textwidth}m{0.035\textwidth}m{0.035\textwidth}m{0.035\textwidth}m{0.035\textwidth}m{0.035\textwidth}m{0.035\textwidth}m{0.038\textwidth}|m{0.035\textwidth}} 
\caption{ECI-Cache size estimation in non-limited SSD‌ cache space.}\label{table:ECI_non_limit}\\
		\hline
		time (min) & VM0 & VM1 & VM2 & VM3 & VM4 & VM5 & VM6 & VM7 & VM8 & VM9 & VM10 & VM11 & VM12 & VM13 & VM14 & VM15 & csum\\ \hline
		10 & 1,166 & 4,511 & 1,434 & 2,602 & 8,396 & 1,971 & 2,394 & 2,832 & 2,072 & 2,207 & 6,084 & 2,557 & 2,367 & 1,606 & 4,203 & 1,635 & 48,037\\
		20 & 2,401 & 4,507 & 4,392 & 3,739 & 10,611 & 6,542 & 4,740 & 4,489 & 4,530 & 2,784 & 13,468 & 3,424 & 11,235 & 2,684 & 5,892 & 5,426 & 90,864\\
		30 & 2,940 & 17,353 & 5,764 & 7,720 & 16,327 & 7,187 & 13,564 & 5,374 & 11,230 & 4,889 & 25,290 & 3,529 & 11,235 & 3,803 & 6,854 & 6,721 & 149,780\\
		40 & 2,940 & 15,949 & 15,256 & 9,452 & 21,457 & 8,043 & 20,936 & 7,129 & 11,562 & 7,204 & 36,333 & 4,120 & 11,235 & 5,289 & 8,245 & 11,185 & 196,335\\
		50 & 3,019 & 15,940 & 23,395 & 9,452 & 21,442 & 8,064 & 31,433 & 8,911 & 21,942 & 8,888 & 41,436 & 5,977 & 11,234 & 6,078 & 9,421 & 16,153 & 242,785\\
		60 & 2,986 & 17,353 & 31,644 & 11,194 & 31,283 & 9,385 & 33,726 & 9,820 & 22,046 & 9,117 & 45,112 & 6,170 & 11,234 & 8,137 & 9,420 & 26,409 & 285,036\\
		70 & 3,375 & 49,137 & 33,166 & 11,810 & 40,401 & 9,641 & 34,993 & 9,861 & 56,835 & 10,168 & 52,972 & 6,326 & 11,234 & 8,597 & 11,440 & 32,001 & 381,957\\
		80 & 3,387 & 67,667 & 33,748 & 13,289 & 41,780 & 11,155 & 35,293 & 10,587 & 65,409 & 11,401 & 53,616 & 7,041 & 11,233 & 8,304 & 12,246 & 41,192 & 427,348\\
		90 & 3,377 & 67,811 & 35,750 & 15,507 & 45,558 & 11,175 & 35,620 & 12,663 & 68,197 & 12,742 & 52,780 & 7,309 & 11,235 & 8,671 & 13,777 & 45,037 & 447,209\\
		100 & 3,760 & 68,169 & 36,553 & 16,214 & 47,046 & 13,707 & 39,182 & 12,748 & 71,577 & 12,727 & 52,694 & 7,341 & 11,233 & 8,788 & 13,777 & 61,379 & 476,895\\
		110 & 3,787 & 78,990 & 37,914 & 17,185 & 47,047 & 14,268 & 40,060 & 14,021 & 73,331 & 14,080 & 52,694 & 8,083 & 11,230 & 11,892 & 13,777 & 63,467 & 501,826\\
		120 & 4,296 & 82,962 & 39,346 & 17,859 & 53,418 & 14,372 & 40,571 & 16,111 & 73,324 & 13,627 & 54,499 & 7,826 & 11,231 & 12,542 & 14,831 & 63,511 & 520,326\\
		130 & 5,323 & 78,985 & 40,413 & 19,993 & 54,545 & 14,375 & 41,690 & 17,990 & 75,061 & 15,280 & 72,428 & 8,077 & 11,230 & 12,542 & 16,214 & 63,854 & 548,000\\
		140 & 5,199 & 78,985 & 42,245 & 20,049 & 57,086 & 15,715 & 44,067 & 18,245 & 75,056 & 15,280 & 72,937 & 8,786 & 11,235 & 12,542 & 16,918 & 66,833 & 561,178\\
		150 & 5,215 & 100,675 & 45,829 & 21,591 & 58,181 & 15,843 & 47,096 & 19,997 & 76,194 & 16,663 & 81,641 & 8,786 & 11,230 & 14,796 & 16,916 & 67,149 & 607,802\\
		160 & 5,215 & 96,548 & 48,909 & 22,709 & 61,281 & 15,856 & 47,794 & 21,228 & 77,398 & 16,604 & 83,401 & 8,279 & 130,834 & 14,797 & 18,328 & 71,616 & 740,797\\
		170 & 5,546 & 96,623 & 49,562 & 22,768 & 61,770 & 15,862 & 47,818 & 21,800 & 0 & 18,636 & 94,006 & 8,279 & 132,739 & 15,043 & 18,773 & 72,365 & 681,590\\
		180 & 6,101 & 100,675 & 48,904 & 23,579 & 64,777 & 17,052 & 47,810 & 22,181 & 0 & 18,642 & 97,021 & 8,786 & 141,448 & 15,553 & 19,457 & 72,376 & 704,362\\
		190 & 6,101 & 113,789 & 49,455 & 24,037 & 61,767 & 17,153 & 47,787 & 22,311 & 0 & 18,634 & 107,394 & 8,395 & 132,342 & 15,505 & 20,715 & 74,580 & 719,965\\
		200 & 6,021 & 97,270 & 52,987 & 24,052 & 61,767 & 17,150 & 47,806 & 22,317 & 0 & 18,654 & 110,258 & 9,627 & 151,893 & 16,031 & 21,009 & 75,233 & 732,075\\
		210 & 6,037 & 98,848 & 54,710 & 25,555 & 66,508 & 25,053 & 47,813 & 24,319 & 0 & 20,583 & 110,447 & 9,408 & 0 & 17,901 & 22,116 & 75,004 & 604,302\\
		220 & 6,039 & 96,556 & 54,744 & 25,518 & 62,822 & 27,777 & 47,794 & 24,342 & 0 & 20,539 & 111,359 & 10,983 & 0 & 17,911 & 22,616 & 75,023 & 604,023\\
		230 & 6,101 & 98,002 & 56,685 & 26,164 & 64,815 & 40,636 & 48,986 & 24,340 & 0 & 20,582 & 111,359 & 10,961 & 0 & 17,955 & 22,776 & 79,182 & 628,544\\
		240 & 6,302 & 100,956 & 56,657 & 26,608 & 62,824 & 46,918 & 48,985 & 25,217 & 0 & 20,533 & 111,359 & 9,756 & 0 & 17,936 & 23,106 & 79,178 & 636,335\\
		250 & 6,023 & 96,978 & 56,663 & 26,893 & 70,002 & 58,106 & 51,128 & 25,227 & 0 & 21,468 & 111,488 & 9,756 & 0 & 17,955 & 24,480 & 79,179 & 655,346\\
		260 & 6,037 & 113,789 & 57,750 & 26,900 & 66,508 & 68,202 & 51,399 & 26,840 & 0 & 21,722 & 111,487 & 9,661 & 0 & 19,609 & 24,480 & 79,193 & 683,577\\
		270 & 6,416 & 96,978 & 57,763 & 27,649 & 63,078 & 77,672 & 53,840 & 27,357 & 0 & 21,751 & 111,359 & 9,627 & 0 & 19,610 & 25,042 & 80,946 & 679,088\\
		280 & 6,438 & 140,807 & 58,813 & 27,635 & 63,009 & 86,538 & 55,927 & 27,458 & 0 & 23,109 & 111,359 & 11,140 & 0 & 19,607 & 25,064 & 81,093 & 737,997\\
		290 & 6,432 & 138,936 & 58,813 & 27,981 & 71,688 & 94,335 & 55,926 & 27,536 & 0 & 23,137 & 138,973 & 10,331 & 0 & 19,608 & 25,650 & 81,090 & 780,436\\
		300 & 6,511 & 160,271 & 59,125 & 27,954 & 67,445 & 107,137 & 57,203 & 27,689 & 0 & 22,498 & 166,236 & 9,635 & 0 & 21,076 & 25,678 & 81,111 & 839,569\\
		310 & 6,498 & 130,137 & 60,604 & 28,954 & 71,723 & 112,427 & 57,717 & 27,604 & 0 & 23,932 & 172,389 & 10,381 & 0 & 21,089 & 26,117 & 81,296 & 830,868\\
		320 & 6,547 & 167,667 & 60,224 & 28,593 & 71,813 & 121,378 & 57,784 & 28,849 & 0 & 23,792 & 178,971 & 10,981 & 0 & 21,148 & 26,126 & 84,025 & 887,898\\
		330 & 6,469 & 148,778 & 60,528 & 28,624 & 74,389 & 137,853 & 58,738 & 29,268 & 0 & 23,833 & 181,801 & 9,635 & 0 & 21,143 & 26,563 & 83,998 & 891,620\\
		340 & 6,507 & 167,667 & 60,616 & 29,535 & 71,749 & 148,780 & 58,738 & 29,243 & 0 & 23,937 & 185,126 & 9,635 & 0 & 21,149 & 27,077 & 84,484 & 924,243\\
		350 & 6,287 & 219,337 & 61,729 & 29,689 & 71,792 & 159,082 & 61,348 & 29,268 & 0 & 24,636 & 188,578 & 10,381 & 0 & 21,154 & 27,832 & 84,532 & 995,645\\
		360 & 6,434 & 156,662 & 61,773 & 29,701 & 73,839 & 150,511 & 62,438 & 29,276 & 0 & 24,642 & 191,541 & 10,023 & 0 & 22,243 & 28,289 & 86,692 & 934,064\\
		370 & 6,434 & 219,337 & 61,837 & 30,598 & 73,714 & 163,938 & 62,213 & 30,295 & 0 & 24,063 & 197,329 & 10,981 & 0 & 22,241 & 28,677 & 93,059 & 1,024,716\\
		380 & 6,483 & 191,951 & 62,538 & 30,283 & 77,273 & 185,631 & 62,709 & 30,342 & 0 & 24,064 & 197,859 & 9,620 & 0 & 23,433 & 28,677 & 101,260 & 1,032,123\\
		390 & 6,434 & 252,659 & 62,397 & 30,598 & 74,389 & 196,197 & 64,393 & 30,342 & 0 & 25,217 & 205,471 & 10,985 & 0 & 24,416 & 29,053 & 110,052 & 1,122,603\\
		400 & 6,507 & 245,658 & 62,547 & 31,092 & 82,471 & 204,712 & 64,860 & 30,333 & 0 & 24,677 & 208,855 & 12,675 & 0 & 25,723 & 29,113 & 115,951 & 1,145,174\\
		410 & 6,455 & 252,658 & 62,554 & 31,057 & 82,471 & 207,607 & 72,389 & 31,230 & 0 & 24,839 & 211,152 & 11,201 & 0 & 28,083 & 29,528 & 130,613 & 1,181,837\\
		420 & 6,507 & 197,970 & 66,618 & 31,707 & 85,568 & 215,142 & 80,585 & 31,704 & 0 & 26,047 & 211,191 & 12,265 & 0 & 28,083 & 29,324 & 137,174 & 1,159,885\\
		430 & 6,701 & 216,363 & 74,599 & 31,693 & 87,969 & 237,896 & 87,788 & 31,764 & 0 & 25,423 & 215,046 & 10,961 & 0 & 28,057 & 29,526 & 139,776 & 1,223,562\\
		440 & 6,432 & 359,362 & 83,743 & 31,705 & 87,917 & 238,025 & 91,193 & 31,765 & 0 & 25,414 & 215,046 & 12,668 & 0 & 28,051 & 30,109 & 139,656 & 1,381,086\\
		450 & 6,111 & 263,873 & 85,270 & 31,706 & 90,042 & 241,975 & 91,327 & 31,937 & 0 & 26,043 & 229,608 & 11,775 & 0 & 28,930 & 30,069 & 151,771 & 1,320,437\\
		460 & 6,515 & 318,922 & 85,276 & 32,022 & 87,406 & 254,905 & 92,212 & 32,645 & 0 & 25,926 & 228,465 & 11,193 & 0 & 29,405 & 33,935 & 152,044 & 1,390,871\\
		470 & 6,515 & 335,927 & 85,282 & 31,927 & 87,412 & 257,629 & 92,218 & 32,736 & 0 & 26,037 & 228,986 & 10,381 & 0 & 28,952 & 36,043 & 167,602 & 1,427,647\\
		480 & 6,515 & 368,234 & 85,282 & 32,257 & 93,769 & 271,759 & 92,217 & 32,790 & 0 & 26,046 & 229,244 & 12,675 & 0 & 29,422 & 37,515 & 170,033 & 1,487,758\\
		490 & 6,604 & 245,658 & 85,276 & 32,399 & 90,042 & 296,602 & 95,326 & 32,730 & 0 & 26,793 & 234,157 & 11,990 & 0 & 30,573 & 36,635 & 184,247 & 1,409,032\\
		500 & 6,220 & 252,659 & 87,338 & 32,255 & 90,054 & 303,176 & 95,223 & 32,726 & 0 & 27,115 & 233,960 & 14,507 & 0 & 30,505 & 37,811 & 192,573 & 1,436,122\\
		510 & 6,438 & 325,524 & 85,281 & 32,418 & 90,410 & 308,298 & 95,223 & 32,793 & 0 & 26,814 & 235,833 & 14,492 & 0 & 32,292 & 38,719 & 199,189 & 1,523,724\\
		520 & 6,075 & 250,512 & 87,335 & 33,066 & 90,244 & 305,972 & 95,323 & 33,407 & 0 & 31,150 & 244,492 & 17,131 & 0 & 32,293 & 38,715 & 204,967 & 1,470,682\\
		530 & 6,498 & 381,961 & 85,282 & 33,725 & 92,809 & 329,184 & 95,227 & 33,413 & 0 & 44,733 & 255,008 & 14,114 & 0 & 32,620 & 38,719 & 211,642 & 1,654,935\\
		540 & 6,075 & 388,312 & 87,462 & 33,066 & 93,670 & 346,259 & 95,223 & 34,036 & 0 & 53,560 & 260,240 & 12,852 & 0 & 33,897 & 38,719 & 215,097 & 1,698,468\\
		550 & 6,483 & 284,507 & 87,342 & 33,161 & 93,427 & 357,716 & 95,222 & 33,416 & 0 & 61,698 & 265,556 & 18,399 & 0 & 33,328 & 38,717 & 215,097 & 1,624,069\\
		560 & 6,430 & 390,922 & 90,424 & 33,351 & 93,422 & 363,293 & 95,230 & 33,905 & 0 & 72,221 & 273,558 & 17,106 & 0 & 33,904 & 40,628 & 215,035 & 1,759,429\\
		570 & 6,351 & 391,485 & 91,206 & 33,704 & 93,428 & 376,735 & 95,250 & 34,083 & 0 & 81,698 & 273,279 & 15,072 & 0 & 33,974 & 39,228 & 217,742 & 1,783,235\\
		580 & 6,284 & 309,089 & 90,628 & 33,717 & 93,429 & 376,735 & 95,417 & 33,991 & 0 & 84,042 & 273,283 & 19,527 & 0 & 33,975 & 39,819 & 219,048 & 1,708,984\\
		590 & 6,110 & 445,264 & 90,422 & 34,340 & 93,426 & 389,982 & 95,311 & 34,100 & 0 & 84,170 & 273,714 & 19,397 & 0 & 33,974 & 41,086 & 220,365 & 1,861,661\\
		600 & 6,284 & 359,362 & 90,696 & 34,345 & 93,722 & 393,125 & 95,227 & 34,700 & 0 & 88,910 & 273,661 & 19,497 & 0 & 34,828 & 41,598 & 222,712 & 1,788,667\\
		610 & 0 & 459,845 & 92,357 & 34,989 & 101,785 & 418,620 & 95,419 & 34,634 & 0 & 105,871 & 279,567 & 19,495 & 0 & 34,668 & 40,628 & 223,114 & 1,940,992\\
		620 & 0 & 385,567 & 90,672 & 35,014 & 101,787 & 426,162 & 98,749 & 35,238 & 0 & 108,485 & 281,381 & 19,513 & 0 & 34,491 & 41,336 & 223,207 & 1,881,602\\
		630 & 0 & 381,611 & 90,422 & 35,039 & 101,785 & 433,315 & 98,740 & 35,828 & 0 & 107,988 & 287,353 & 14,492 & 0 & 34,829 & 41,458 & 223,172 & 1,886,032\\
		640 & 0 & 440,568 & 90,549 & 35,492 & 101,787 & 443,773 & 98,610 & 35,994 & 0 & 108,479 & 287,402 & 14,503 & 0 & 34,450 & 41,657 & 223,928 & 1,957,192\\
		650 & 0 & 452,309 & 90,567 & 35,039 & 101,787 & 445,140 & 98,734 & 36,530 & 0 & 109,019 & 287,392 & 18,353 & 0 & 34,450 & 41,756 & 224,292 & 1,975,368\\
		660 & 0 & 411,771 & 94,849 & 35,040 & 101,789 & 445,510 & 98,660 & 36,925 & 0 & 108,484 & 290,335 & 19,542 & 0 & 34,504 & 41,794 & 224,473 & 1,943,676\\
		670 & 0 & 454,999 & 93,905 & 35,675 & 104,395 & 463,478 & 101,219 & 37,160 & 0 & 109,176 & 293,378 & 15,239 & 0 & 34,558 & 42,936 & 223,930 & 2,010,048\\
		680 & 0 & 440,568 & 92,357 & 35,753 & 102,800 & 484,131 & 101,334 & 37,056 & 0 & 109,178 & 295,657 & 17,478 & 0 & 35,587 & 43,090 & 224,403 & 2,019,392\\
		690 & 0 & 539,102 & 93,430 & 35,729 & 102,792 & 489,331 & 100,712 & 37,095 & 0 & 109,177 & 295,660 & 22,883 & 0 & 39,587 & 43,282 & 225,328 & 2,134,108\\
		700 & 0 & 541,096 & 92,705 & 35,724 & 109,507 & 490,748 & 101,362 & 37,160 & 0 & 109,176 & 295,657 & 23,428 & 0 & 38,203 & 44,497 & 225,379 & 2,144,642\\
		710 & 0 & 539,105 & 94,849 & 35,737 & 109,488 & 498,285 & 101,199 & 37,465 & 0 & 109,176 & 295,659 & 24,257 & 0 & 39,498 & 43,325 & 225,348 & 2,153,391\\
		720 & 0 & 578,184 & 92,640 & 35,741 & 109,506 & 504,337 & 101,199 & 37,170 & 0 & 109,628 & 295,660 & 24,254 & 0 & 40,993 & 44,341 & 226,845 & 2,200,498\\
		730 & 0 & 539,116 & 100,641 & 35,773 & 109,488 & 533,139 & 103,553 & 37,542 & 0 & 110,034 & 301,121 & 24,196 & 0 & 40,407 & 43,727 & 226,849 & 2,205,586\\
		740 & 0 & 539,116 & 100,127 & 36,458 & 109,506 & 533,731 & 103,696 & 37,543 & 0 & 109,644 & 295,659 & 26,864 & 0 & 41,186 & 43,656 & 226,799 & 2,203,985\\
		750 & 0 & 608,677 & 100,642 & 35,765 & 109,502 & 538,181 & 103,411 & 37,335 & 0 & 111,139 & 306,836 & 24,771 & 0 & 42,364 & 43,865 & 226,840 & 2,289,328\\
		760 & 0 & 554,130 & 100,133 & 36,901 & 109,508 & 548,456 & 105,820 & 37,574 & 0 & 111,134 & 310,317 & 26,130 & 0 & 42,729 & 44,063 & 227,490 & 2,254,385\\
		770 & 0 & 578,201 & 100,140 & 36,162 & 111,139 & 548,456 & 103,678 & 38,056 & 0 & 111,077 & 310,373 & 26,451 & 0 & 44,166 & 44,427 & 226,826 & 2,279,152\\
		780 & 0 & 605,674 & 100,644 & 36,713 & 109,497 & 573,096 & 103,511 & 37,751 & 0 & 111,137 & 310,525 & 28,132 & 0 & 43,615 & 43,926 & 227,603 & 2,331,824\\
		790 & 0 & 574,569 & 102,162 & 36,425 & 109,506 & 573,666 & 105,740 & 38,159 & 0 & 111,172 & 310,556 & 26,555 & 0 & 45,628 & 45,461 & 227,424 & 2,307,023\\
		800 & 0 & 660,596 & 101,740 & 35,796 & 109,488 & 573,265 & 105,873 & 40,383 & 0 & 111,382 & 310,558 & 27,838 & 0 & 45,209 & 44,431 & 227,925 & 2,394,484\\
		810 & 0 & 673,671 & 101,739 & 36,142 & 110,731 & 596,544 & 103,696 & 37,958 & 0 & 111,461 & 313,873 & 29,327 & 0 & 45,916 & 45,455 & 229,309 & 2,435,822\\
		820 & 0 & 683,446 & 103,740 & 37,336 & 110,732 & 602,074 & 103,696 & 39,769 & 0 & 111,144 & 314,579 & 26,768 & 0 & 48,174 & 45,518 & 228,257 & 2,455,233\\
		830 & 0 & 684,550 & 103,781 & 37,714 & 111,272 & 627,562 & 105,288 & 39,404 & 0 & 111,144 & 323,850 & 27,838 & 0 & 53,165 & 46,768 & 231,454 & 2,503,790\\
		840 & 0 & 704,906 & 103,781 & 37,730 & 110,732 & 624,029 & 104,900 & 40,776 & 0 & 111,422 & 324,798 & 29,672 & 0 & 56,909 & 45,838 & 231,406 & 2,526,899\\
		850 & 0 & 695,734 & 103,781 & 37,548 & 110,732 & 629,128 & 104,883 & 41,237 & 0 & 111,536 & 327,238 & 27,994 & 0 & 56,222 & 45,559 & 229,309 & 2,520,901\\
		860 & 0 & 710,700 & 103,780 & 37,896 & 111,255 & 645,313 & 104,936 & 40,826 & 0 & 111,144 & 346,510 & 27,626 & 0 & 65,383 & 47,817 & 228,781 & 2,581,967\\
		870 & 0 & 721,451 & 103,780 & 37,754 & 110,735 & 645,313 & 104,943 & 40,780 & 0 & 111,143 & 349,237 & 27,190 & 0 & 60,196 & 47,890 & 230,243 & 2,590,655\\
		880 & 0 & 728,244 & 103,781 & 37,737 & 111,122 & 670,418 & 105,851 & 41,485 & 0 & 111,143 & 349,044 & 30,124 & 0 & 68,273 & 47,720 & 230,584 & 2,635,526\\
		890 & 0 & 733,753 & 103,878 & 37,737 & 110,741 & 667,933 & 108,006 & 41,848 & 0 & 111,426 & 349,239 & 30,123 & 0 & 68,731 & 50,426 & 229,640 & 2,643,481\\
		900 & 0 & 721,451 & 104,674 & 38,831 & 110,741 & 679,022 & 108,605 & 41,254 & 0 & 112,351 & 349,090 & 30,101 & 0 & 68,525 & 49,024 & 231,712 & 2,645,381\\
		910 & 0 & 760,219 & 103,781 & 38,824 & 113,114 & 678,507 & 108,606 & 41,556 & 0 & 111,383 & 354,768 & 30,462 & 0 & 68,955 & 49,075 & 231,454 & 2,690,704\\
		920 & 0 & 783,932 & 103,877 & 39,144 & 110,735 & 667,913 & 108,365 & 41,848 & 0 & 112,473 & 380,991 & 30,126 & 0 & 70,110 & 48,547 & 232,085 & 2,730,146\\
		930 & 0 & 784,311 & 103,874 & 37,766 & 111,251 & 706,580 & 108,561 & 41,351 & 0 & 111,524 & 349,317 & 30,126 & 0 & 70,830 & 48,509 & 231,668 & 2,735,668\\
		940 & 0 & 792,911 & 104,294 & 38,041 & 113,113 & 680,148 & 108,600 & 41,887 & 0 & 112,348 & 352,519 & 30,126 & 0 & 71,991 & 48,319 & 231,658 & 2,725,955\\
		950 & 0 & 792,923 & 103,781 & 38,056 & 116,736 & 745,094 & 110,346 & 41,736 & 0 & 111,524 & 356,164 & 30,127 & 0 & 71,559 & 48,734 & 232,659 & 2,799,439\\
		960 & 0 & 784,307 & 103,781 & 38,041 & 115,164 & 747,014 & 111,856 & 41,978 & 0 & 112,179 & 350,829 & 30,231 & 0 & 71,595 & 49,217 & 232,699 & 2,788,891\\
		970 & 0 & 822,922 & 104,294 & 38,506 & 116,126 & 768,933 & 112,031 & 45,459 & 0 & 112,242 & 355,117 & 30,481 & 0 & 71,991 & 50,124 & 232,689 & 2,860,915\\
		980 & 0 & 849,389 & 103,782 & 39,978 & 116,143 & 760,514 & 112,031 & 42,019 & 0 & 111,676 & 363,636 & 30,584 & 0 & 71,257 & 48,549 & 233,959 & 2,883,517\\
		990 & 0 & 855,637 & 108,463 & 38,739 & 115,682 & 789,864 & 112,031 & 45,127 & 0 & 111,673 & 409,662 & 31,782 & 0 & 71,629 & 49,364 & 233,958 & 2,973,611\\
		1,000 & 0 & 858,813 & 110,270 & 38,480 & 120,974 & 789,864 & 112,031 & 42,077 & 0 & 111,575 & 370,553 & 32,159 & 0 & 72,036 & 48,745 & 233,958 & 2,941,535\\
		1,010 & 0 & 864,265 & 112,989 & 41,263 & 120,975 & 809,615 & 112,162 & 45,956 & 0 & 112,348 & 374,580 & 30,405 & 0 & 71,595 & 49,024 & 234,679 & 2,979,856\\
		1,020 & 0 & 864,585 & 110,102 & 41,263 & 120,975 & 808,755 & 112,032 & 45,458 & 0 & 111,575 & 410,255 & 31,063 & 0 & 72,408 & 50,142 & 234,463 & 3,013,076\\
		1,030 & 0 & 864,584 & 121,050 & 41,268 & 120,974 & 812,172 & 113,618 & 44,715 & 0 & 111,808 & 394,519 & 32,860 & 0 & 72,168 & 53,607 & 234,660 & 3,018,003\\
		1,040 & 0 & 861,467 & 113,172 & 41,262 & 120,975 & 811,135 & 112,032 & 45,458 & 0 & 111,674 & 407,319 & 33,937 & 0 & 72,191 & 50,142 & 234,704 & 3,015,468\\
		1,050 & 0 & 855,531 & 117,197 & 41,279 & 123,741 & 849,919 & 112,032 & 45,556 & 0 & 112,734 & 433,022 & 33,512 & 0 & 72,234 & 52,298 & 236,216 & 3,085,271\\
		1,060 & 0 & 870,203 & 126,100 & 41,270 & 120,975 & 848,518 & 112,031 & 45,708 & 0 & 112,785 & 432,222 & 33,931 & 0 & 72,866 & 52,365 & 234,473 & 3,103,447\\
		1,070 & 0 & 856,539 & 131,264 & 41,998 & 123,779 & 868,177 & 113,152 & 46,739 & 0 & 112,348 & 431,863 & 33,336 & 0 & 71,992 & 53,702 & 234,679 & 3,119,568\\
		1,080 & 0 & 866,760 & 131,265 & 41,736 & 123,734 & 878,542 & 112,032 & 45,259 & 0 & 113,403 & 412,927 & 33,654 & 0 & 72,810 & 55,434 & 235,552 & 3,123,108\\
		1,090 & 0 & 925,854 & 138,769 & 42,533 & 120,975 & 879,342 & 113,640 & 46,151 & 0 & 112,400 & 411,445 & 33,897 & 0 & 72,790 & 54,437 & 235,324 & 3,187,557\\
		1,100 & 0 & 855,644 & 140,513 & 41,740 & 125,168 & 875,749 & 113,142 & 46,318 & 0 & 112,287 & 411,231 & 33,495 & 0 & 73,529 & 53,996 & 236,698 & 3,119,510\\
		1,110 & 0 & 856,537 & 141,639 & 41,533 & 125,164 & 878,147 & 112,163 & 46,138 & 0 & 112,505 & 431,384 & 33,775 & 0 & 75,140 & 53,155 & 236,698 & 3,143,978\\
		1,120 & 0 & 856,553 & 130,470 & 41,903 & 125,165 & 917,028 & 112,162 & 46,914 & 0 & 113,562 & 411,908 & 34,018 & 0 & 73,529 & 54,785 & 237,513 & 3,155,510\\
		1,130 & 0 & 856,542 & 145,784 & 42,022 & 125,164 & 919,413 & 113,640 & 46,296 & 0 & 113,189 & 449,700 & 33,775 & 0 & 75,933 & 55,844 & 237,512 & 3,214,814\\
		1,140 & 0 & 972,429 & 168,490 & 42,601 & 125,167 & 931,599 & 113,773 & 46,597 & 0 & 113,687 & 498,070 & 33,530 & 0 & 75,132 & 55,443 & 237,488 & 3,414,006\\
		1,150 & 0 & 918,807 & 151,778 & 41,739 & 125,163 & 946,680 & 114,073 & 0 & 0 & 112,502 & 497,994 & 33,999 & 0 & 74,721 & 57,447 & 238,824 & 3,313,727\\
		1,160 & 0 & 864,101 & 183,175 & 41,997 & 125,162 & 946,868 & 113,773 & 0 & 0 & 113,703 & 498,061 & 33,775 & 0 & 74,740 & 58,579 & 237,647 & 3,291,581\\
		1,170 & 0 & 913,488 & 190,682 & 42,283 & 125,161 & 946,533 & 113,467 & 0 & 0 & 113,703 & 498,068 & 34,717 & 0 & 73,830 & 60,133 & 238,649 & 3,350,714\\
		1,180 & 0 & 998,202 & 190,529 & 42,944 & 125,160 & 972,122 & 113,525 & 0 & 0 & 113,580 & 498,000 & 34,039 & 0 & 73,891 & 58,587 & 239,854 & 3,460,433\\
		1,190 & 0 & 903,650 & 191,414 & 42,003 & 125,164 & 956,609 & 116,531 & 0 & 0 & 113,643 & 498,070 & 33,842 & 0 & 74,607 & 57,104 & 240,839 & 3,353,476\\
		1,200 & 0 & 980,745 & 199,116 & 42,726 & 125,161 & 964,864 & 118,507 & 0 & 0 & 114,447 & 514,941 & 34,786 & 0 & 74,804 & 57,054 & 243,240 & 3,470,391\\
		1,210 & 0 & 998,202 & 204,807 & 42,230 & 125,165 & 974,035 & 116,121 & 0 & 0 & 113,385 & 514,919 & 34,027 & 0 & 75,881 & 57,734 & 244,082 & 3,500,588\\
		1,220 & 0 & 875,368 & 204,620 & 42,903 & 125,161 & 992,599 & 114,556 & 0 & 0 & 0 & 515,199 & 36,567 & 0 & 75,929 & 60,306 & 246,612 & 3,289,820\\
		1,230 & 0 & 918,807 & 204,563 & 44,218 & 125,167 & 980,037 & 115,564 & 0 & 0 & 0 & 515,199 & 35,009 & 0 & 75,025 & 58,998 & 244,084 & 3,316,671\\
		1,240 & 0 & 952,818 & 213,693 & 43,269 & 125,168 & 999,888 & 115,967 & 0 & 0 & 0 & 515,702 & 34,410 & 0 & 76,462 & 58,993 & 246,417 & 3,382,787\\
		1,250 & 0 & 965,940 & 207,163 & 42,794 & 125,160 & 972,545 & 115,754 & 0 & 0 & 0 & 516,781 & 34,018 & 0 & 75,601 & 62,082 & 244,486 & 3,362,324\\
		1,260 & 0 & 965,940 & 208,145 & 44,741 & 125,165 & 979,469 & 116,805 & 0 & 0 & 0 & 547,846 & 34,839 & 0 & 75,441 & 60,416 & 246,942 & 3,405,749\\
		1,270 & 0 & 944,590 & 213,363 & 43,266 & 125,163 & 999,888 & 119,949 & 0 & 0 & 0 & 518,410 & 34,284 & 0 & 76,329 & 62,798 & 244,088 & 3,382,128\\
		1,280 & 0 & 901,358 & 209,570 & 44,741 & 125,166 & 999,888 & 116,804 & 0 & 0 & 0 & 541,551 & 36,567 & 0 & 75,933 & 61,286 & 245,328 & 3,358,192\\
		1,290 & 0 & 865,952 & 211,241 & 43,143 & 125,168 & 999,888 & 121,084 & 0 & 0 & 0 & 552,322 & 36,413 & 0 & 75,791 & 64,781 & 247,978 & 3,343,761\\
		1,300 & 0 & 998,202 & 215,577 & 44,134 & 125,163 & 999,888 & 120,923 & 0 & 0 & 0 & 551,527 & 35,780 & 0 & 76,192 & 61,084 & 244,062 & 3,472,532\\
		1,310 & 0 & 953,333 & 214,363 & 43,630 & 125,160 & 999,888 & 118,393 & 0 & 0 & 0 & 553,093 & 38,192 & 0 & 76,159 & 67,561 & 245,166 & 3,434,938\\
		1,320 & 0 & 998,202 & 215,273 & 43,269 & 125,165 & 999,888 & 123,179 & 0 & 0 & 0 & 541,889 & 37,647 & 0 & 77,286 & 67,917 & 244,362 & 3,474,077\\
		1,330 & 0 & 980,745 & 222,271 & 43,166 & 125,163 & 999,888 & 118,610 & 0 & 0 & 0 & 551,949 & 37,587 & 0 & 78,664 & 67,660 & 245,018 & 3,470,721\\
		1,340 & 0 & 998,202 & 216,695 & 45,199 & 125,168 & 999,888 & 119,283 & 0 & 0 & 0 & 542,823 & 37,394 & 0 & 77,399 & 73,218 & 246,902 & 3,482,171\\
		1,350 & 0 & 995,938 & 218,195 & 44,908 & 129,094 & 999,888 & 121,158 & 0 & 0 & 0 & 542,385 & 36,888 & 0 & 76,284 & 80,132 & 247,433 & 3,492,303\\
		1,360 & 0 & 998,202 & 216,496 & 44,752 & 125,165 & 999,888 & 124,106 & 0 & 0 & 0 & 550,187 & 36,593 & 0 & 76,472 & 79,556 & 250,522 & 3,501,939\\
		1,370 & 0 & 935,100 & 219,922 & 44,163 & 129,094 & 999,888 & 119,170 & 0 & 0 & 0 & 558,263 & 36,447 & 0 & 77,154 & 80,540 & 248,354 & 3,448,095\\
		1,380 & 0 & 998,202 & 220,552 & 44,163 & 129,070 & 999,888 & 120,845 & 0 & 0 & 0 & 555,235 & 40,831 & 0 & 76,815 & 80,398 & 249,403 & 3,515,402\\
		1,390 & 0 & 998,202 & 222,318 & 44,240 & 125,165 & 999,888 & 123,324 & 0 & 0 & 0 & 569,028 & 40,386 & 0 & 79,468 & 80,540 & 249,492 & 3,532,051\\
		1,400 & 0 & 998,202 & 220,528 & 44,240 & 128,856 & 999,888 & 123,412 & 0 & 0 & 0 & 569,011 & 40,347 & 0 & 80,026 & 81,585 & 247,980 & 3,534,075\\
		1,410 & 0 & 998,202 & 223,000 & 44,472 & 125,168 & 999,888 & 124,688 & 0 & 0 & 0 & 569,257 & 40,386 & 0 & 80,666 & 82,193 & 249,491 & 3,537,411\\
		1,420 & 0 & 998,202 & 223,004 & 44,646 & 125,166 & 999,888 & 123,516 & 0 & 0 & 0 & 564,345 & 40,423 & 0 & 80,169 & 86,759 & 250,458 & 3,536,576\\
		1,430 & 0 & 998,202 & 223,053 & 44,742 & 128,846 & 999,888 & 124,388 & 0 & 0 & 0 & 563,292 & 40,406 & 0 & 79,187 & 86,515 & 248,357 & 3,536,876\\
		1,440 & 0 & 998,202 & 223,053 & 0 & 129,074 & 999,888 & 125,640 & 0 & 0 & 0 & 558,252 & 40,347 & 0 & 80,247 & 85,048 & 248,243 & 3,487,994\\
		1,450 & 0 & 998,202 & 225,799 & 0 & 128,998 & 999,888 & 125,175 & 0 & 0 & 0 & 569,014 & 40,338 & 0 & 79,454 & 85,069 & 249,115 & 3,501,052\\
		1,460 & 0 & 998,202 & 226,520 & 0 & 129,080 & 999,888 & 124,007 & 0 & 0 & 0 & 569,144 & 40,353 & 0 & 80,349 & 84,978 & 249,084 & 3,501,605\\
		1,470 & 0 & 998,202 & 233,978 & 0 & 129,094 & 999,888 & 126,346 & 0 & 0 & 0 & 569,248 & 40,352 & 0 & 79,943 & 85,763 & 248,482 & 3,511,296\\
		1,480 & 0 & 998,202 & 233,979 & 0 & 128,850 & 999,888 & 126,234 & 0 & 0 & 0 & 569,075 & 40,430 & 0 & 81,054 & 84,882 & 249,106 & 3,511,700\\
		1,490 & 0 & 998,202 & 226,888 & 0 & 125,166 & 999,888 & 126,345 & 0 & 0 & 0 & 569,087 & 40,448 & 0 & 80,448 & 85,763 & 249,247 & 3,501,482\\
		1,500 & 0 & 998,202 & 234,424 & 0 & 128,998 & 999,888 & 126,345 & 0 & 0 & 0 & 558,146 & 40,353 & 0 & 80,330 & 86,125 & 252,544 & 3,505,355\\
		1,510 & 0 & 998,202 & 229,986 & 0 & 125,168 & 999,888 & 129,196 & 0 & 0 & 0 & 558,263 & 38,730 & 0 & 80,176 & 84,978 & 253,145 & 3,497,732\\
		1,520 & 0 & 998,202 & 228,718 & 0 & 130,562 & 999,888 & 124,864 & 0 & 0 & 0 & 558,098 & 38,735 & 0 & 79,921 & 86,757 & 252,282 & 3,498,027\\
		1,530 & 0 & 998,202 & 227,865 & 0 & 130,568 & 999,888 & 125,430 & 0 & 0 & 0 & 577,185 & 38,770 & 0 & 80,336 & 85,533 & 252,708 & 3,516,485\\
		1,540 & 0 & 998,202 & 227,401 & 0 & 131,975 & 999,888 & 125,416 & 0 & 0 & 0 & 577,167 & 38,872 & 0 & 81,306 & 89,504 & 252,281 & 3,522,012\\
		1,550 & 0 & 998,202 & 229,098 & 0 & 130,618 & 999,888 & 125,407 & 0 & 0 & 0 & 577,168 & 38,914 & 0 & 79,644 & 86,050 & 252,732 & 3,517,721\\
		1,560 & 0 & 998,202 & 229,247 & 0 & 131,975 & 999,888 & 127,334 & 0 & 0 & 0 & 577,186 & 39,420 & 0 & 0 & 85,097 & 252,282 & 3,440,631\\
		1,570 & 0 & 998,202 & 232,453 & 0 & 131,973 & 999,888 & 125,174 & 0 & 0 & 0 & 602,904 & 39,442 & 0 & 0 & 89,292 & 252,280 & 3,471,608\\
		1,580 & 0 & 998,202 & 230,762 & 0 & 130,648 & 999,888 & 125,405 & 0 & 0 & 0 & 602,904 & 42,554 & 0 & 0 & 88,549 & 252,279 & 3,471,191\\
		1,590 & 0 & 998,202 & 231,442 & 0 & 132,089 & 999,888 & 125,400 & 0 & 0 & 0 & 602,902 & 42,750 & 0 & 0 & 91,570 & 252,280 & 3,476,523\\
		1,600 & 0 & 998,202 & 234,499 & 0 & 144,295 & 999,888 & 128,951 & 0 & 0 & 0 & 602,902 & 42,554 & 0 & 0 & 91,570 & 252,282 & 3,495,143\\
		1,610 & 0 & 998,202 & 241,170 & 0 & 130,635 & 999,888 & 129,949 & 0 & 0 & 0 & 602,901 & 42,554 & 0 & 0 & 91,154 & 252,545 & 3,488,998\\
		1,620 & 0 & 998,202 & 236,568 & 0 & 135,402 & 999,888 & 128,283 & 0 & 0 & 0 & 602,903 & 42,555 & 0 & 0 & 91,569 & 253,301 & 3,488,671\\
		1,630 & 0 & 998,202 & 233,213 & 0 & 141,152 & 999,888 & 129,447 & 0 & 0 & 0 & 602,901 & 42,732 & 0 & 0 & 91,570 & 253,219 & 3,492,324\\
		1,640 & 0 & 0 & 233,823 & 0 & 141,227 & 999,888 & 132,050 & 0 & 0 & 0 & 602,901 & 42,749 & 0 & 0 & 91,570 & 254,410 & 2,498,618\\
		1,650 & 0 & 0 & 234,426 & 0 & 145,349 & 999,996 & 132,050 & 0 & 0 & 0 & 602,904 & 42,554 & 0 & 0 & 91,597 & 254,067 & 2,502,943\\
		1,660 & 0 & 0 & 235,026 & 0 & 148,595 & 999,996 & 126,851 & 0 & 0 & 0 & 602,904 & 42,555 & 0 & 0 & 91,597 & 254,067 & 2,501,591\\
		1,670 & 0 & 0 & 241,166 & 0 & 145,405 & 999,996 & 132,452 & 0 & 0 & 0 & 610,007 & 42,732 & 0 & 0 & 91,598 & 254,019 & 2,517,375\\
		1,680 & 0 & 0 & 242,049 & 0 & 141,153 & 999,996 & 127,612 & 0 & 0 & 0 & 602,904 & 43,011 & 0 & 0 & 91,913 & 254,073 & 2,502,711\\
		1,690 & 0 & 0 & 242,060 & 0 & 143,762 & 999,996 & 127,612 & 0 & 0 & 0 & 602,906 & 42,554 & 0 & 0 & 91,569 & 253,300 & 2,503,759\\
		1,700 & 0 & 0 & 235,026 & 0 & 145,123 & 999,996 & 134,553 & 0 & 0 & 0 & 603,380 & 42,555 & 0 & 0 & 91,572 & 254,019 & 2,506,224\\
		1,710 & 0 & 0 & 237,561 & 0 & 145,592 & 999,996 & 131,156 & 0 & 0 & 0 & 602,903 & 42,732 & 0 & 0 & 91,593 & 255,017 & 2,506,550\\
		1,720 & 0 & 0 & 237,945 & 0 & 146,772 & 999,996 & 129,447 & 0 & 0 & 0 & 602,904 & 42,991 & 0 & 0 & 91,597 & 254,297 & 2,505,949\\
		1,730 & 0 & 0 & 239,156 & 0 & 145,883 & 999,996 & 130,151 & 0 & 0 & 0 & 602,902 & 42,554 & 0 & 0 & 91,570 & 253,364 & 2,505,576\\
		1,740 & 0 & 0 & 241,148 & 0 & 144,295 & 999,996 & 133,432 & 0 & 0 & 0 & 602,901 & 42,701 & 0 & 0 & 91,597 & 257,256 & 2,513,326\\
		1,750 & 0 & 0 & 241,866 & 0 & 145,589 & 999,996 & 138,864 & 0 & 0 & 0 & 602,904 & 42,976 & 0 & 0 & 91,570 & 253,974 & 2,517,739\\
		1,760 & 0 & 0 & 240,187 & 0 & 146,261 & 999,996 & 131,518 & 0 & 0 & 0 & 602,906 & 42,554 & 0 & 0 & 91,569 & 254,062 & 2,509,053\\
		1,770 & 0 & 0 & 241,145 & 0 & 146,297 & 999,996 & 134,488 & 0 & 0 & 0 & 602,903 & 42,555 & 0 & 0 & 91,598 & 254,177 & 2,513,159\\
		1,780 & 0 & 0 & 238,649 & 0 & 146,560 & 999,996 & 129,677 & 0 & 0 & 0 & 602,901 & 42,750 & 0 & 0 & 91,597 & 254,394 & 2,506,524\\
		1,790 & 0 & 0 & 239,796 & 0 & 149,269 & 999,996 & 134,280 & 0 & 0 & 0 & 602,901 & 42,719 & 0 & 0 & 93,617 & 255,284 & 2,517,862\\
		1,800 & 0 & 0 & 241,754 & 0 & 145,120 & 999,996 & 129,196 & 0 & 0 & 0 & 602,905 & 42,999 & 0 & 0 & 91,597 & 253,959 & 2,507,526\\
		1,810 & 0 & 0 & 241,159 & 0 & 145,404 & 999,996 & 134,483 & 0 & 0 & 0 & 602,904 & 46,045 & 0 & 0 & 0 & 253,957 & 2,423,948\\
		1,820 & 0 & 0 & 241,323 & 0 & 148,006 & 999,996 & 135,075 & 0 & 0 & 0 & 602,904 & 42,734 & 0 & 0 & 0 & 254,780 & 2,424,818\\
		1,830 & 0 & 0 & 242,051 & 0 & 145,596 & 999,996 & 135,018 & 0 & 0 & 0 & 602,904 & 43,393 & 0 & 0 & 0 & 256,386 & 2,425,344\\
		1,840 & 0 & 0 & 241,700 & 0 & 146,719 & 999,996 & 135,466 & 0 & 0 & 0 & 611,940 & 46,081 & 0 & 0 & 0 & 253,697 & 2,435,599\\
		1,850 & 0 & 0 & 241,684 & 0 & 145,722 & 999,996 & 138,865 & 0 & 0 & 0 & 602,901 & 45,455 & 0 & 0 & 0 & 254,394 & 2,429,017\\
		1,860 & 0 & 0 & 243,046 & 0 & 151,656 & 999,996 & 135,329 & 0 & 0 & 0 & 620,604 & 46,685 & 0 & 0 & 0 & 255,283 & 2,452,599\\
		1,870 & 0 & 0 & 242,166 & 0 & 146,695 & 999,996 & 143,262 & 0 & 0 & 0 & 604,749 & 48,232 & 0 & 0 & 0 & 254,193 & 2,439,293\\
		1,880 & 0 & 0 & 241,754 & 0 & 146,056 & 999,996 & 134,972 & 0 & 0 & 0 & 602,904 & 46,144 & 0 & 0 & 0 & 256,000 & 2,427,826\\
		1,890 & 0 & 0 & 241,701 & 0 & 145,597 & 999,996 & 135,453 & 0 & 0 & 0 & 610,808 & 46,678 & 0 & 0 & 0 & 257,317 & 2,437,550\\
		1,900 & 0 & 0 & 244,512 & 0 & 145,664 & 999,996 & 136,567 & 0 & 0 & 0 & 602,901 & 47,984 & 0 & 0 & 0 & 259,159 & 2,436,783\\
		1,910 & 0 & 0 & 244,683 & 0 & 0 & 999,996 & 139,055 & 0 & 0 & 0 & 604,749 & 48,156 & 0 & 0 & 0 & 257,269 & 2,293,908\\
		1,920 & 0 & 0 & 244,022 & 0 & 0 & 999,996 & 137,000 & 0 & 0 & 0 & 602,904 & 46,740 & 0 & 0 & 0 & 257,310 & 2,287,972\\
		1,930 & 0 & 0 & 243,982 & 0 & 0 & 999,996 & 140,372 & 0 & 0 & 0 & 602,906 & 47,532 & 0 & 0 & 0 & 257,345 & 2,292,133\\
		1,940 & 0 & 0 & 245,957 & 0 & 0 & 999,996 & 137,012 & 0 & 0 & 0 & 602,901 & 47,960 & 0 & 0 & 0 & 258,416 & 2,292,242\\
		1,950 & 0 & 0 & 242,687 & 0 & 0 & 999,996 & 137,022 & 0 & 0 & 0 & 623,114 & 48,116 & 0 & 0 & 0 & 257,305 & 2,308,240\\
		1,960 & 0 & 0 & 242,282 & 0 & 0 & 999,996 & 136,982 & 0 & 0 & 0 & 634,773 & 49,061 & 0 & 0 & 0 & 258,770 & 2,321,864\\
		1,970 & 0 & 0 & 245,039 & 0 & 0 & 999,996 & 136,782 & 0 & 0 & 0 & 618,942 & 47,467 & 0 & 0 & 0 & 258,096 & 2,306,322\\
		1,980 & 0 & 0 & 255,711 & 0 & 0 & 999,996 & 136,785 & 0 & 0 & 0 & 618,868 & 47,693 & 0 & 0 & 0 & 257,363 & 2,316,416\\
		1,990 & 0 & 0 & 249,862 & 0 & 0 & 999,996 & 138,195 & 0 & 0 & 0 & 634,773 & 48,124 & 0 & 0 & 0 & 258,981 & 2,329,931\\
		2,000 & 0 & 0 & 246,463 & 0 & 0 & 999,996 & 137,086 & 0 & 0 & 0 & 620,862 & 49,060 & 0 & 0 & 0 & 258,934 & 2,312,401\\
		2,010 & 0 & 0 & 243,982 & 0 & 0 & 999,996 & 139,904 & 0 & 0 & 0 & 616,553 & 48,109 & 0 & 0 & 0 & 258,752 & 2,307,296\\
		2,020 & 0 & 0 & 250,318 & 0 & 0 & 999,996 & 141,979 & 0 & 0 & 0 & 647,906 & 48,928 & 0 & 0 & 0 & 258,729 & 2,347,856\\
		2,030 & 0 & 0 & 245,942 & 0 & 0 & 999,996 & 148,710 & 0 & 0 & 0 & 634,773 & 51,439 & 0 & 0 & 0 & 0 & 2,080,860\\
		2,040 & 0 & 0 & 244,561 & 0 & 0 & 999,996 & 147,518 & 0 & 0 & 0 & 619,027 & 48,015 & 0 & 0 & 0 & 0 & 2,059,117\\
		2,050 & 0 & 0 & 259,984 & 0 & 0 & 999,996 & 148,293 & 0 & 0 & 0 & 619,145 & 48,619 & 0 & 0 & 0 & 0 & 2,076,037\\
		2,060 & 0 & 0 & 246,271 & 0 & 0 & 999,996 & 137,023 & 0 & 0 & 0 & 622,607 & 49,764 & 0 & 0 & 0 & 0 & 2,055,661\\
		2,070 & 0 & 0 & 250,218 & 0 & 0 & 999,996 & 137,449 & 0 & 0 & 0 & 618,627 & 47,999 & 0 & 0 & 0 & 0 & 2,054,289\\
		2,080 & 0 & 0 & 248,460 & 0 & 0 & 999,996 & 141,827 & 0 & 0 & 0 & 621,211 & 48,515 & 0 & 0 & 0 & 0 & 2,060,009\\
		2,090 & 0 & 0 & 252,543 & 0 & 0 & 999,996 & 147,134 & 0 & 0 & 0 & 625,789 & 49,258 & 0 & 0 & 0 & 0 & 2,074,720\\
		2,100 & 0 & 0 & 245,942 & 0 & 0 & 999,996 & 148,727 & 0 & 0 & 0 & 629,446 & 47,910 & 0 & 0 & 0 & 0 & 2,072,021\\
		2,110 & 0 & 0 & 262,144 & 0 & 0 & 999,996 & 137,153 & 0 & 0 & 0 & 627,595 & 48,567 & 0 & 0 & 0 & 0 & 2,075,455\\
		2,120 & 0 & 0 & 243,636 & 0 & 0 & 999,996 & 137,379 & 0 & 0 & 0 & 636,360 & 49,908 & 0 & 0 & 0 & 0 & 2,067,279\\
		2,130 & 0 & 0 & 254,470 & 0 & 0 & 999,996 & 140,380 & 0 & 0 & 0 & 632,565 & 48,120 & 0 & 0 & 0 & 0 & 2,075,531\\
		2,140 & 0 & 0 & 247,867 & 0 & 0 & 999,996 & 145,721 & 0 & 0 & 0 & 633,224 & 49,131 & 0 & 0 & 0 & 0 & 2,075,939\\
		2,150 & 0 & 0 & 249,233 & 0 & 0 & 999,996 & 139,136 & 0 & 0 & 0 & 658,655 & 54,694 & 0 & 0 & 0 & 0 & 2,101,714\\
		2,160 & 0 & 0 & 264,590 & 0 & 0 & 999,996 & 137,254 & 0 & 0 & 0 & 632,096 & 48,482 & 0 & 0 & 0 & 0 & 2,082,418\\
		2,170 & 0 & 0 & 249,126 & 0 & 0 & 999,996 & 146,380 & 0 & 0 & 0 & 631,700 & 48,619 & 0 & 0 & 0 & 0 & 2,075,821\\
		2,180 & 0 & 0 & 243,538 & 0 & 0 & 999,996 & 148,089 & 0 & 0 & 0 & 634,444 & 50,318 & 0 & 0 & 0 & 0 & 2,076,385\\
		2,190 & 0 & 0 & 252,185 & 0 & 0 & 999,996 & 138,710 & 0 & 0 & 0 & 632,770 & 48,420 & 0 & 0 & 0 & 0 & 2,072,081\\
		2,200 & 0 & 0 & 249,302 & 0 & 0 & 0 & 148,294 & 0 & 0 & 0 & 633,234 & 50,106 & 0 & 0 & 0 & 0 & 1,080,936\\
		2,210 & 0 & 0 & 243,965 & 0 & 0 & 0 & 151,078 & 0 & 0 & 0 & 634,799 & 54,549 & 0 & 0 & 0 & 0 & 1,084,391\\
		2,220 & 0 & 0 & 243,965 & 0 & 0 & 0 & 140,022 & 0 & 0 & 0 & 650,155 & 50,145 & 0 & 0 & 0 & 0 & 1,084,287\\
		2,230 & 0 & 0 & 260,108 & 0 & 0 & 0 & 140,022 & 0 & 0 & 0 & 668,514 & 53,636 & 0 & 0 & 0 & 0 & 1,122,280\\
		2,240 & 0 & 0 & 260,229 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 658,678 & 50,078 & 0 & 0 & 0 & 0 & 968,985\\
		2,250 & 0 & 0 & 258,559 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 655,520 & 53,281 & 0 & 0 & 0 & 0 & 967,360\\
		2,260 & 0 & 0 & 259,987 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 637,933 & 50,216 & 0 & 0 & 0 & 0 & 948,136\\
		2,270 & 0 & 0 & 260,229 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 678,310 & 53,375 & 0 & 0 & 0 & 0 & 991,914\\
		2,280 & 0 & 0 & 259,984 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 672,549 & 56,277 & 0 & 0 & 0 & 0 & 988,810\\
		2,290 & 0 & 0 & 251,529 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 672,142 & 53,203 & 0 & 0 & 0 & 0 & 976,874\\
		2,300 & 0 & 0 & 259,989 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 677,636 & 55,058 & 0 & 0 & 0 & 0 & 992,683\\
		2,310 & 0 & 0 & 262,868 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 640,249 & 53,187 & 0 & 0 & 0 & 0 & 956,304\\
		2,320 & 0 & 0 & 247,867 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 654,298 & 54,292 & 0 & 0 & 0 & 0 & 956,457\\
		2,330 & 0 & 0 & 250,976 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 678,463 & 53,066 & 0 & 0 & 0 & 0 & 982,505\\
		2,340 & 0 & 0 & 258,264 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 655,520 & 53,647 & 0 & 0 & 0 & 0 & 967,431\\
		2,350 & 0 & 0 & 245,133 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 639,402 & 52,923 & 0 & 0 & 0 & 0 & 937,458\\
		2,360 & 0 & 0 & 256,575 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 679,750 & 53,558 & 0 & 0 & 0 & 0 & 989,883\\
		2,370 & 0 & 0 & 262,292 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 671,996 & 52,784 & 0 & 0 & 0 & 0 & 987,072\\
		2,380 & 0 & 0 & 256,662 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 668,515 & 53,359 & 0 & 0 & 0 & 0 & 978,536\\
		2,390 & 0 & 0 & 249,862 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 672,120 & 55,270 & 0 & 0 & 0 & 0 & 977,252\\
		2,400 & 0 & 0 & 250,319 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 654,317 & 53,257 & 0 & 0 & 0 & 0 & 957,893\\
		2,410 & 0 & 0 & 245,941 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 653,977 & 55,058 & 0 & 0 & 0 & 0 & 954,976\\
		2,420 & 0 & 0 & 265,286 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 640,779 & 57,589 & 0 & 0 & 0 & 0 & 963,654\\
		2,430 & 0 & 0 & 257,675 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 675,852 & 60,610 & 0 & 0 & 0 & 0 & 994,137\\
		2,440 & 0 & 0 & 254,932 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 655,888 & 58,430 & 0 & 0 & 0 & 0 & 969,250\\
		2,450 & 0 & 0 & 249,310 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 638,619 & 57,589 & 0 & 0 & 0 & 0 & 945,518\\
		2,460 & 0 & 0 & 249,305 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 638,223 & 59,476 & 0 & 0 & 0 & 0 & 947,004\\
		2,470 & 0 & 0 & 257,675 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 673,921 & 59,927 & 0 & 0 & 0 & 0 & 991,523\\
		2,480 & 0 & 0 & 253,326 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 658,695 & 60,842 & 0 & 0 & 0 & 0 & 972,863\\
		2,490 & 0 & 0 & 247,673 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 680,851 & 60,755 & 0 & 0 & 0 & 0 & 989,279\\
		2,500 & 0 & 0 & 265,822 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 653,583 & 61,229 & 0 & 0 & 0 & 0 & 980,634\\
		2,510 & 0 & 0 & 255,430 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 639,402 & 62,211 & 0 & 0 & 0 & 0 & 957,043\\
		2,520 & 0 & 0 & 254,932 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 672,122 & 62,247 & 0 & 0 & 0 & 0 & 989,301\\
		2,530 & 0 & 0 & 261,254 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 639,347 & 61,776 & 0 & 0 & 0 & 0 & 962,377\\
		2,540 & 0 & 0 & 262,292 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 654,317 & 61,595 & 0 & 0 & 0 & 0 & 978,204\\
		2,550 & 0 & 0 & 246,690 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 677,886 & 61,465 & 0 & 0 & 0 & 0 & 986,041\\
		2,560 & 0 & 0 & 257,319 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 681,548 & 60,930 & 0 & 0 & 0 & 0 & 999,797\\
		2,570 & 0 & 0 & 255,754 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 655,594 & 63,139 & 0 & 0 & 0 & 0 & 974,487\\
		2,580 & 0 & 0 & 254,469 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 639,402 & 62,051 & 0 & 0 & 0 & 0 & 955,922\\
		2,590 & 0 & 0 & 255,711 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 676,660 & 61,763 & 0 & 0 & 0 & 0 & 994,134\\
		2,600 & 0 & 0 & 259,781 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 666,267 & 63,880 & 0 & 0 & 0 & 0 & 989,928\\
		2,610 & 0 & 0 & 259,990 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 641,832 & 62,426 & 0 & 0 & 0 & 0 & 964,248\\
		2,620 & 0 & 0 & 262,004 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 642,067 & 65,285 & 0 & 0 & 0 & 0 & 969,356\\
		2,630 & 0 & 0 & 265,056 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 663,394 & 62,654 & 0 & 0 & 0 & 0 & 991,104\\
		2,640 & 0 & 0 & 247,268 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 658,759 & 64,475 & 0 & 0 & 0 & 0 & 970,502\\
		2,650 & 0 & 0 & 250,151 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 651,855 & 65,823 & 0 & 0 & 0 & 0 & 967,829\\
		2,660 & 0 & 0 & 255,035 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 668,511 & 63,050 & 0 & 0 & 0 & 0 & 986,596\\
		2,670 & 0 & 0 & 258,264 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 656,372 & 64,693 & 0 & 0 & 0 & 0 & 979,329\\
		2,680 & 0 & 0 & 263,317 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 644,274 & 65,741 & 0 & 0 & 0 & 0 & 973,332\\
		2,690 & 0 & 0 & 251,100 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 655,888 & 64,264 & 0 & 0 & 0 & 0 & 971,252\\
		2,700 & 0 & 0 & 257,808 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 653,516 & 66,618 & 0 & 0 & 0 & 0 & 977,942\\
		2,710 & 0 & 0 & 264,538 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 645,096 & 64,717 & 0 & 0 & 0 & 0 & 974,351\\
		2,720 & 0 & 0 & 250,091 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 672,639 & 62,525 & 0 & 0 & 0 & 0 & 985,255\\
		2,730 & 0 & 0 & 259,984 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 681,950 & 64,878 & 0 & 0 & 0 & 0 & 1,006,812\\
		2,740 & 0 & 0 & 246,539 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 658,678 & 67,088 & 0 & 0 & 0 & 0 & 972,305\\
		2,750 & 0 & 0 & 256,772 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 692,689 & 64,026 & 0 & 0 & 0 & 0 & 1,013,487\\
		2,760 & 0 & 0 & 245,940 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 692,465 & 65,539 & 0 & 0 & 0 & 0 & 1,003,944\\
		2,770 & 0 & 0 & 258,673 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 658,967 & 63,062 & 0 & 0 & 0 & 0 & 980,702\\
		2,780 & 0 & 0 & 250,976 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 665,942 & 64,909 & 0 & 0 & 0 & 0 & 981,827\\
		2,790 & 0 & 0 & 262,655 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 672,122 & 67,820 & 0 & 0 & 0 & 0 & 1,002,597\\
		2,800 & 0 & 0 & 256,637 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 684,682 & 64,036 & 0 & 0 & 0 & 0 & 1,005,355\\
		2,810 & 0 & 0 & 250,976 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 659,003 & 65,824 & 0 & 0 & 0 & 0 & 975,803\\
		2,820 & 0 & 0 & 264,539 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 670,557 & 63,619 & 0 & 0 & 0 & 0 & 998,715\\
		2,830 & 0 & 0 & 256,917 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 692,464 & 65,164 & 0 & 0 & 0 & 0 & 1,014,545\\
		2,840 & 0 & 0 & 250,814 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 668,514 & 62,654 & 0 & 0 & 0 & 0 & 981,982\\
		2,850 & 0 & 0 & 247,852 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 692,689 & 64,890 & 0 & 0 & 0 & 0 & 1,005,431\\
		2,860 & 0 & 0 & 256,179 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 671,996 & 67,572 & 0 & 0 & 0 & 0 & 995,747\\
		2,870 & 0 & 0 & 259,986 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 664,389 & 64,412 & 0 & 0 & 0 & 0 & 988,787\\
		2,880 & 0 & 0 & 259,984 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 693,794 & 66,687 & 0 & 0 & 0 & 0 & 1,020,465\\
		2,890 & 0 & 0 & 257,815 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 686,879 & 65,187 & 0 & 0 & 0 & 0 & 1,009,881\\
		2,900 & 0 & 0 & 257,675 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 681,718 & 64,906 & 0 & 0 & 0 & 0 & 1,004,299\\
		2,910 & 0 & 0 & 267,368 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 681,793 & 68,286 & 0 & 0 & 0 & 0 & 1,017,447\\
		2,920 & 0 & 0 & 267,368 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 678,212 & 64,906 & 0 & 0 & 0 & 0 & 1,010,486\\
		2,930 & 0 & 0 & 267,259 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 681,664 & 68,304 & 0 & 0 & 0 & 0 & 1,017,227\\
		2,940 & 0 & 0 & 265,068 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 691,514 & 64,910 & 0 & 0 & 0 & 0 & 1,021,492\\
		2,950 & 0 & 0 & 264,476 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 657,346 & 67,665 & 0 & 0 & 0 & 0 & 989,487\\
		2,960 & 0 & 0 & 268,820 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 665,558 & 64,890 & 0 & 0 & 0 & 0 & 999,268\\
		2,970 & 0 & 0 & 268,820 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 677,636 & 67,518 & 0 & 0 & 0 & 0 & 1,013,974\\
		2,980 & 0 & 0 & 268,822 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 662,265 & 64,681 & 0 & 0 & 0 & 0 & 995,768\\
		2,990 & 0 & 0 & 268,884 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 681,778 & 66,941 & 0 & 0 & 0 & 0 & 1,017,603\\
		3,000 & 0 & 0 & 266,607 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 670,519 & 64,803 & 0 & 0 & 0 & 0 & 1,001,929\\
		3,010 & 0 & 0 & 267,379 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 692,679 & 66,887 & 0 & 0 & 0 & 0 & 1,026,945\\
		3,020 & 0 & 0 & 267,379 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 666,461 & 64,312 & 0 & 0 & 0 & 0 & 998,152\\
		3,030 & 0 & 0 & 267,380 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 661,309 & 66,385 & 0 & 0 & 0 & 0 & 995,074\\
		3,040 & 0 & 0 & 268,728 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 670,365 & 63,953 & 0 & 0 & 0 & 0 & 1,003,046\\
		3,050 & 0 & 0 & 268,865 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 695,230 & 66,248 & 0 & 0 & 0 & 0 & 1,030,343\\
		3,060 & 0 & 0 & 267,115 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 687,808 & 64,908 & 0 & 0 & 0 & 0 & 1,019,831\\
		3,070 & 0 & 0 & 267,260 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 681,582 & 67,491 & 0 & 0 & 0 & 0 & 1,016,333\\
		3,080 & 0 & 0 & 267,372 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 681,582 & 64,890 & 0 & 0 & 0 & 0 & 1,013,844\\
		3,090 & 0 & 0 & 268,593 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 694,913 & 67,581 & 0 & 0 & 0 & 0 & 1,031,087\\
		3,100 & 0 & 0 & 268,847 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 690,954 & 64,906 & 0 & 0 & 0 & 0 & 1,024,707\\
		3,110 & 0 & 0 & 267,360 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 681,287 & 67,765 & 0 & 0 & 0 & 0 & 1,016,412\\
		3,120 & 0 & 0 & 267,761 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 677,896 & 64,927 & 0 & 0 & 0 & 0 & 1,010,584\\
		3,130 & 0 & 0 & 268,864 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 668,142 & 68,340 & 0 & 0 & 0 & 0 & 1,005,346\\
		3,140 & 0 & 0 & 268,761 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 667,473 & 64,927 & 0 & 0 & 0 & 0 & 1,001,161\\
		3,150 & 0 & 0 & 267,260 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 667,251 & 67,863 & 0 & 0 & 0 & 0 & 1,002,374\\
		3,160 & 0 & 0 & 267,377 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 667,287 & 64,967 & 0 & 0 & 0 & 0 & 999,631\\
		3,170 & 0 & 0 & 268,731 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 669,969 & 65,218 & 0 & 0 & 0 & 0 & 1,003,918\\
		3,180 & 0 & 0 & 267,260 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 671,459 & 65,092 & 0 & 0 & 0 & 0 & 1,003,811\\
		3,190 & 0 & 0 & 268,708 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 677,939 & 68,616 & 0 & 0 & 0 & 0 & 1,015,263\\
		3,200 & 0 & 0 & 267,260 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 686,017 & 65,768 & 0 & 0 & 0 & 0 & 1,019,045\\
		3,210 & 0 & 0 & 268,705 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 695,964 & 69,765 & 0 & 0 & 0 & 0 & 1,034,434\\
		3,220 & 0 & 0 & 267,259 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 668,925 & 66,481 & 0 & 0 & 0 & 0 & 1,002,665\\
		3,230 & 0 & 0 & 268,708 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 677,636 & 64,883 & 0 & 0 & 0 & 0 & 1,011,227\\
		3,240 & 0 & 0 & 267,260 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 692,465 & 67,672 & 0 & 0 & 0 & 0 & 1,027,397\\
		3,250 & 0 & 0 & 268,761 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 669,547 & 65,411 & 0 & 0 & 0 & 0 & 1,003,719\\
		3,260 & 0 & 0 & 267,370 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 683,458 & 69,702 & 0 & 0 & 0 & 0 & 1,020,530\\
		3,270 & 0 & 0 & 268,819 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 666,506 & 66,494 & 0 & 0 & 0 & 0 & 1,001,819\\
		3,280 & 0 & 0 & 267,376 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 683,497 & 64,890 & 0 & 0 & 0 & 0 & 1,015,763\\
		3,290 & 0 & 0 & 272,746 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 668,361 & 67,895 & 0 & 0 & 0 & 0 & 1,009,002\\
		3,300 & 0 & 0 & 268,694 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 691,472 & 65,696 & 0 & 0 & 0 & 0 & 1,025,862\\
		3,310 & 0 & 0 & 267,374 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 671,459 & 69,906 & 0 & 0 & 0 & 0 & 1,008,739\\
		3,320 & 0 & 0 & 268,874 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 663,558 & 66,687 & 0 & 0 & 0 & 0 & 999,119\\
		3,330 & 0 & 0 & 267,377 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 686,879 & 64,910 & 0 & 0 & 0 & 0 & 1,019,166\\
		3,340 & 0 & 0 & 267,260 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 672,557 & 68,576 & 0 & 0 & 0 & 0 & 1,008,393\\
		3,350 & 0 & 0 & 268,847 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 667,333 & 65,968 & 0 & 0 & 0 & 0 & 1,002,148\\
		3,360 & 0 & 0 & 267,648 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 698,519 & 71,509 & 0 & 0 & 0 & 0 & 1,037,676\\
		3,370 & 0 & 0 & 267,370 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 692,460 & 67,581 & 0 & 0 & 0 & 0 & 1,027,411\\
		3,380 & 0 & 0 & 273,649 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 685,950 & 65,539 & 0 & 0 & 0 & 0 & 1,025,138\\
		3,390 & 0 & 0 & 268,842 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 681,664 & 69,478 & 0 & 0 & 0 & 0 & 1,019,984\\
		3,400 & 0 & 0 & 268,216 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 677,896 & 66,639 & 0 & 0 & 0 & 0 & 1,012,751\\
		3,410 & 0 & 0 & 267,360 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 676,400 & 64,911 & 0 & 0 & 0 & 0 & 1,008,671\\
		3,420 & 0 & 0 & 268,868 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 677,636 & 68,991 & 0 & 0 & 0 & 0 & 1,015,495\\
		3,430 & 0 & 0 & 267,623 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 681,889 & 66,296 & 0 & 0 & 0 & 0 & 1,015,808\\
		3,440 & 0 & 0 & 267,379 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 698,626 & 74,282 & 0 & 0 & 0 & 0 & 1,040,287\\
		3,450 & 0 & 0 & 267,369 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 665,954 & 65,767 & 0 & 0 & 0 & 0 & 999,090\\
		3,460 & 0 & 0 & 266,496 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 669,348 & 66,248 & 0 & 0 & 0 & 0 & 1,002,092\\
		3,470 & 0 & 0 & 268,845 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 681,920 & 67,673 & 0 & 0 & 0 & 0 & 1,018,438\\
		3,480 & 0 & 0 & 267,380 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 671,099 & 66,774 & 0 & 0 & 0 & 0 & 1,005,253\\
		3,490 & 0 & 0 & 267,373 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 685,851 & 74,148 & 0 & 0 & 0 & 0 & 1,027,372\\
		3,500 & 0 & 0 & 267,259 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 666,463 & 69,436 & 0 & 0 & 0 & 0 & 1,003,158\\
		3,510 & 0 & 0 & 273,649 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 672,664 & 74,375 & 0 & 0 & 0 & 0 & 1,020,688\\
		3,520 & 0 & 0 & 268,884 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 698,777 & 73,968 & 0 & 0 & 0 & 0 & 1,041,629\\
		3,530 & 0 & 0 & 268,841 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 672,610 & 75,086 & 0 & 0 & 0 & 0 & 1,016,537\\
		3,540 & 0 & 0 & 268,729 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 668,511 & 74,384 & 0 & 0 & 0 & 0 & 1,011,624\\
		3,550 & 0 & 0 & 268,682 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 694,559 & 73,975 & 0 & 0 & 0 & 0 & 1,037,216\\
		3,560 & 0 & 0 & 268,844 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 680,912 & 74,516 & 0 & 0 & 0 & 0 & 1,024,272\\
		3,570 & 0 & 0 & 268,845 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 692,679 & 74,279 & 0 & 0 & 0 & 0 & 1,035,803\\
		3,580 & 0 & 0 & 268,842 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 670,557 & 75,000 & 0 & 0 & 0 & 0 & 1,014,399\\
		3,590 & 0 & 0 & 268,730 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 685,950 & 74,483 & 0 & 0 & 0 & 0 & 1,029,163\\
		3,600 & 0 & 0 & 268,708 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 692,465 & 74,148 & 0 & 0 & 0 & 0 & 1,035,321\\
		3,610 & 0 & 0 & 268,593 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 691,688 & 74,501 & 0 & 0 & 0 & 0 & 1,034,782\\
		3,620 & 0 & 0 & 268,593 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 694,425 & 74,382 & 0 & 0 & 0 & 0 & 1,037,400\\
		3,630 & 0 & 0 & 268,593 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 698,799 & 74,535 & 0 & 0 & 0 & 0 & 1,041,927\\
		3,640 & 0 & 0 & 268,841 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 671,700 & 74,487 & 0 & 0 & 0 & 0 & 1,015,028\\
		3,650 & 0 & 0 & 268,819 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 700,991 & 74,271 & 0 & 0 & 0 & 0 & 1,044,081\\
		3,660 & 0 & 0 & 268,819 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 692,464 & 74,496 & 0 & 0 & 0 & 0 & 1,035,779\\
		3,670 & 0 & 0 & 268,843 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 681,849 & 74,370 & 0 & 0 & 0 & 0 & 1,025,062\\
		3,680 & 0 & 0 & 268,865 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 675,274 & 74,508 & 0 & 0 & 0 & 0 & 1,018,647\\
		3,690 & 0 & 0 & 269,709 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 672,089 & 74,476 & 0 & 0 & 0 & 0 & 1,016,274\\
		3,700 & 0 & 0 & 266,607 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 671,015 & 75,107 & 0 & 0 & 0 & 0 & 1,012,729\\
		3,710 & 0 & 0 & 267,372 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 704,486 & 74,494 & 0 & 0 & 0 & 0 & 1,046,352\\
		3,720 & 0 & 0 & 267,375 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 698,919 & 74,313 & 0 & 0 & 0 & 0 & 1,040,607\\
		3,730 & 0 & 0 & 267,379 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 698,338 & 74,503 & 0 & 0 & 0 & 0 & 1,040,220\\
		3,740 & 0 & 0 & 268,593 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 698,318 & 74,458 & 0 & 0 & 0 & 0 & 1,041,369\\
		3,750 & 0 & 0 & 268,707 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 698,474 & 75,557 & 0 & 0 & 0 & 0 & 1,042,738\\
		3,760 & 0 & 0 & 268,765 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 700,150 & 74,315 & 0 & 0 & 0 & 0 & 1,043,230\\
		3,770 & 0 & 0 & 268,843 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 707,620 & 74,796 & 0 & 0 & 0 & 0 & 1,051,259\\
		3,780 & 0 & 0 & 268,875 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 671,317 & 74,495 & 0 & 0 & 0 & 0 & 1,014,687\\
		3,790 & 0 & 0 & 271,305 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 672,742 & 74,373 & 0 & 0 & 0 & 0 & 1,018,420\\
		3,800 & 0 & 0 & 266,304 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 681,361 & 74,532 & 0 & 0 & 0 & 0 & 1,022,197\\
		3,810 & 0 & 0 & 267,260 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 687,278 & 74,493 & 0 & 0 & 0 & 0 & 1,029,031\\
		3,820 & 0 & 0 & 267,372 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 692,469 & 74,799 & 0 & 0 & 0 & 0 & 1,034,640\\
		3,830 & 0 & 0 & 265,370 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 699,906 & 74,524 & 0 & 0 & 0 & 0 & 1,039,800\\
		3,840 & 0 & 0 & 267,256 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 672,040 & 74,490 & 0 & 0 & 0 & 0 & 1,013,786\\
		3,850 & 0 & 0 & 267,370 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 681,718 & 74,748 & 0 & 0 & 0 & 0 & 1,023,836\\
		3,860 & 0 & 0 & 267,378 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 697,758 & 74,529 & 0 & 0 & 0 & 0 & 1,039,665\\
		3,870 & 0 & 0 & 268,694 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 672,089 & 75,063 & 0 & 0 & 0 & 0 & 1,015,846\\
		3,880 & 0 & 0 & 268,846 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 692,305 & 74,644 & 0 & 0 & 0 & 0 & 1,035,795\\
		3,890 & 0 & 0 & 265,067 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 672,020 & 74,504 & 0 & 0 & 0 & 0 & 1,011,591\\
		3,900 & 0 & 0 & 267,376 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 692,333 & 74,774 & 0 & 0 & 0 & 0 & 1,034,483\\
		3,910 & 0 & 0 & 268,634 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 673,920 & 74,617 & 0 & 0 & 0 & 0 & 1,017,171\\
		3,920 & 0 & 0 & 268,846 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 692,464 & 74,504 & 0 & 0 & 0 & 0 & 1,035,814\\
		3,930 & 0 & 0 & 266,596 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 671,459 & 74,780 & 0 & 0 & 0 & 0 & 1,012,835\\
		3,940 & 0 & 0 & 267,370 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 694,927 & 74,643 & 0 & 0 & 0 & 0 & 1,036,940\\
		3,950 & 0 & 0 & 268,842 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 674,274 & 74,508 & 0 & 0 & 0 & 0 & 1,017,624\\
		3,960 & 0 & 0 & 267,370 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 694,043 & 74,784 & 0 & 0 & 0 & 0 & 1,036,197\\
		3,970 & 0 & 0 & 268,875 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 675,280 & 74,643 & 0 & 0 & 0 & 0 & 1,018,798\\
		3,980 & 0 & 0 & 265,548 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 698,558 & 74,504 & 0 & 0 & 0 & 0 & 1,038,610\\
		3,990 & 0 & 0 & 268,216 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 685,983 & 74,780 & 0 & 0 & 0 & 0 & 1,028,979\\
		4,000 & 0 & 0 & 267,374 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 670,995 & 74,624 & 0 & 0 & 0 & 0 & 1,012,993\\
		4,010 & 0 & 0 & 268,729 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 692,464 & 74,504 & 0 & 0 & 0 & 0 & 1,035,697\\
		4,020 & 0 & 0 & 269,748 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 691,475 & 75,053 & 0 & 0 & 0 & 0 & 1,036,276\\
		4,030 & 0 & 0 & 268,846 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 682,642 & 74,772 & 0 & 0 & 0 & 0 & 1,026,260\\
		4,040 & 0 & 0 & 268,695 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 676,624 & 74,619 & 0 & 0 & 0 & 0 & 1,019,938\\
		4,050 & 0 & 0 & 268,865 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 672,024 & 74,511 & 0 & 0 & 0 & 0 & 1,015,400\\
		4,060 & 0 & 0 & 268,862 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 672,061 & 74,784 & 0 & 0 & 0 & 0 & 1,015,707\\
		4,070 & 0 & 0 & 266,589 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 701,069 & 74,658 & 0 & 0 & 0 & 0 & 1,042,316\\
		4,080 & 0 & 0 & 267,259 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 700,991 & 74,518 & 0 & 0 & 0 & 0 & 1,042,768\\
		4,090 & 0 & 0 & 269,709 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 694,889 & 74,867 & 0 & 0 & 0 & 0 & 1,039,465\\
		4,100 & 0 & 0 & 266,598 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 685,051 & 74,659 & 0 & 0 & 0 & 0 & 1,026,308\\
		4,110 & 0 & 0 & 267,380 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 685,983 & 74,528 & 0 & 0 & 0 & 0 & 1,027,891\\
		4,120 & 0 & 0 & 268,843 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 684,664 & 75,417 & 0 & 0 & 0 & 0 & 1,028,924\\
		4,130 & 0 & 0 & 265,815 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 678,606 & 74,728 & 0 & 0 & 0 & 0 & 1,019,149\\
		4,140 & 0 & 0 & 273,034 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 674,283 & 74,586 & 0 & 0 & 0 & 0 & 1,021,903\\
		4,150 & 0 & 0 & 267,360 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 690,521 & 77,652 & 0 & 0 & 0 & 0 & 1,035,533\\
		4,160 & 0 & 0 & 268,847 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 685,544 & 74,776 & 0 & 0 & 0 & 0 & 1,029,167\\
		4,170 & 0 & 0 & 267,378 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 683,883 & 74,642 & 0 & 0 & 0 & 0 & 1,025,903\\
		4,180 & 0 & 0 & 268,845 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 672,142 & 74,514 & 0 & 0 & 0 & 0 & 1,015,501\\
		4,190 & 0 & 0 & 267,260 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 682,726 & 74,958 & 0 & 0 & 0 & 0 & 1,024,944\\
		4,200 & 0 & 0 & 268,708 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 681,689 & 74,703 & 0 & 0 & 0 & 0 & 1,025,100\\
		4,210 & 0 & 0 & 269,540 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 684,274 & 74,590 & 0 & 0 & 0 & 0 & 1,028,404\\
		4,220 & 0 & 0 & 272,575 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 678,788 & 76,581 & 0 & 0 & 0 & 0 & 1,027,944\\
		4,230 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 686,340 & 75,184 & 0 & 0 & 0 & 0 & 761,524\\
		4,240 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 672,396 & 74,731 & 0 & 0 & 0 & 0 & 747,127\\
		4,250 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 692,679 & 74,619 & 0 & 0 & 0 & 0 & 767,298\\
		4,260 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 698,777 & 74,511 & 0 & 0 & 0 & 0 & 773,288\\
		4,270 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 700,991 & 74,802 & 0 & 0 & 0 & 0 & 775,793\\
		4,280 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 707,662 & 74,681 & 0 & 0 & 0 & 0 & 782,343\\
		4,290 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 706,626 & 74,564 & 0 & 0 & 0 & 0 & 781,190\\
		4,300 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 690,500 & 77,707 & 0 & 0 & 0 & 0 & 768,207\\
		4,310 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 707,536 & 74,780 & 0 & 0 & 0 & 0 & 782,316\\
		4,320 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 681,890 & 74,652 & 0 & 0 & 0 & 0 & 756,542\\
		4,330 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 690,645 & 74,535 & 0 & 0 & 0 & 0 & 765,180\\
		4,340 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 695,230 & 76,437 & 0 & 0 & 0 & 0 & 771,667\\
		4,350 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 710,686 & 74,773 & 0 & 0 & 0 & 0 & 785,459\\
		4,360 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 680,350 & 74,645 & 0 & 0 & 0 & 0 & 754,995\\
		4,370 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 686,311 & 74,529 & 0 & 0 & 0 & 0 & 760,840\\
		4,380 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 694,920 & 76,092 & 0 & 0 & 0 & 0 & 771,012\\
		4,390 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 718,674 & 74,767 & 0 & 0 & 0 & 0 & 793,441\\
		4,400 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 683,425 & 74,636 & 0 & 0 & 0 & 0 & 758,061\\
		4,410 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 683,283 & 74,528 & 0 & 0 & 0 & 0 & 757,811\\
		4,420 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 691,688 & 75,956 & 0 & 0 & 0 & 0 & 767,644\\
		4,430 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 683,372 & 74,773 & 0 & 0 & 0 & 0 & 758,145\\
		4,440 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 692,466 & 74,637 & 0 & 0 & 0 & 0 & 767,103\\
		4,450 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 711,607 & 74,528 & 0 & 0 & 0 & 0 & 786,135\\
		4,460 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 683,425 & 76,186 & 0 & 0 & 0 & 0 & 759,611\\
		4,470 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 685,775 & 74,772 & 0 & 0 & 0 & 0 & 760,547\\
		4,480 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 692,465 & 74,631 & 0 & 0 & 0 & 0 & 767,096\\
		4,490 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 678,463 & 74,510 & 0 & 0 & 0 & 0 & 752,973\\
		4,500 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 683,466 & 75,211 & 0 & 0 & 0 & 0 & 758,677\\
		4,510 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 697,955 & 74,696 & 0 & 0 & 0 & 0 & 772,651\\
		4,520 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 684,395 & 74,558 & 0 & 0 & 0 & 0 & 758,953\\
		4,530 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 698,519 & 77,692 & 0 & 0 & 0 & 0 & 776,211\\
		4,540 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 683,628 & 74,774 & 0 & 0 & 0 & 0 & 758,402\\
		4,550 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 698,558 & 74,626 & 0 & 0 & 0 & 0 & 773,184\\
		4,560 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 684,689 & 74,504 & 0 & 0 & 0 & 0 & 759,193\\
		4,570 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 678,212 & 74,806 & 0 & 0 & 0 & 0 & 753,018\\
		4,580 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 694,425 & 74,664 & 0 & 0 & 0 & 0 & 769,089\\
		4,590 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 683,202 & 74,532 & 0 & 0 & 0 & 0 & 757,734\\
		4,600 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 698,589 & 76,186 & 0 & 0 & 0 & 0 & 774,775\\
		4,610 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 685,775 & 74,748 & 0 & 0 & 0 & 0 & 760,523\\
		4,620 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 718,889 & 74,617 & 0 & 0 & 0 & 0 & 793,506\\
		4,630 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 694,412 & 74,503 & 0 & 0 & 0 & 0 & 768,915\\
		4,640 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 683,425 & 86,574 & 0 & 0 & 0 & 0 & 769,999\\
		4,650 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 707,652 & 77,543 & 0 & 0 & 0 & 0 & 785,195\\
		4,660 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 694,528 & 74,781 & 0 & 0 & 0 & 0 & 769,309\\
		4,670 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 694,927 & 74,683 & 0 & 0 & 0 & 0 & 769,610\\
		4,680 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 692,465 & 86,575 & 0 & 0 & 0 & 0 & 779,040\\
		4,690 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 693,647 & 77,652 & 0 & 0 & 0 & 0 & 771,299\\
		4,700 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 692,464 & 74,785 & 0 & 0 & 0 & 0 & 767,249\\
		4,710 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 692,206 & 74,657 & 0 & 0 & 0 & 0 & 766,863\\
		4,720 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 694,674 & 86,291 & 0 & 0 & 0 & 0 & 780,965\\
		4,730 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 692,256 & 77,543 & 0 & 0 & 0 & 0 & 769,799\\
		4,740 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 684,019 & 74,806 & 0 & 0 & 0 & 0 & 758,825\\
		4,750 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 708,533 & 74,697 & 0 & 0 & 0 & 0 & 783,230\\
		4,760 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 685,349 & 86,573 & 0 & 0 & 0 & 0 & 771,922\\
		4,770 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 694,287 & 82,967 & 0 & 0 & 0 & 0 & 777,254\\
		4,780 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 684,333 & 75,732 & 0 & 0 & 0 & 0 & 760,065\\
		4,790 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 698,334 & 74,773 & 0 & 0 & 0 & 0 & 773,107\\
		4,800 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 688,826 & 74,648 & 0 & 0 & 0 & 0 & 763,474\\
		4,810 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 685,349 & 83,905 & 0 & 0 & 0 & 0 & 769,254\\
		4,820 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 684,057 & 77,708 & 0 & 0 & 0 & 0 & 761,765\\
		4,830 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 692,465 & 75,184 & 0 & 0 & 0 & 0 & 767,649\\
		4,840 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 710,686 & 74,741 & 0 & 0 & 0 & 0 & 785,427\\
		4,850 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 685,349 & 87,318 & 0 & 0 & 0 & 0 & 772,667\\
		4,860 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 692,464 & 84,149 & 0 & 0 & 0 & 0 & 776,613\\
		4,870 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 717,893 & 76,581 & 0 & 0 & 0 & 0 & 794,474\\
		4,880 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 707,011 & 74,858 & 0 & 0 & 0 & 0 & 781,869\\
		4,890 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 698,558 & 74,705 & 0 & 0 & 0 & 0 & 773,263\\
		4,900 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 699,506 & 86,576 & 0 & 0 & 0 & 0 & 786,082\\
		4,910 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 694,682 & 83,388 & 0 & 0 & 0 & 0 & 778,070\\
		4,920 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 692,465 & 76,111 & 0 & 0 & 0 & 0 & 768,576\\
		4,930 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 694,707 & 74,783 & 0 & 0 & 0 & 0 & 769,490\\
		4,940 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 696,314 & 74,681 & 0 & 0 & 0 & 0 & 770,995\\
		4,950 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 694,832 & 86,574 & 0 & 0 & 0 & 0 & 781,406\\
		4,960 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 694,345 & 82,983 & 0 & 0 & 0 & 0 & 777,328\\
		4,970 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 685,497 & 75,967 & 0 & 0 & 0 & 0 & 761,464\\
		4,980 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 685,349 & 75,107 & 0 & 0 & 0 & 0 & 760,456\\
		4,990 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 687,929 & 74,763 & 0 & 0 & 0 & 0 & 762,692\\
		5,000 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 689,266 & 86,579 & 0 & 0 & 0 & 0 & 775,845\\
		5,010 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 688,831 & 83,449 & 0 & 0 & 0 & 0 & 772,280\\
		5,020 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 688,822 & 77,543 & 0 & 0 & 0 & 0 & 766,365\\
		5,030 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 695,474 & 75,612 & 0 & 0 & 0 & 0 & 771,086\\
		5,040 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 753,927 & 74,768 & 0 & 0 & 0 & 0 & 828,695\\
		5,050 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 694,002 & 86,576 & 0 & 0 & 0 & 0 & 780,578\\
		5,060 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 696,143 & 84,150 & 0 & 0 & 0 & 0 & 780,293\\
		5,070 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 704,489 & 81,046 & 0 & 0 & 0 & 0 & 785,535\\
		5,080 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 706,583 & 75,955 & 0 & 0 & 0 & 0 & 782,538\\
		5,090 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 707,757 & 74,781 & 0 & 0 & 0 & 0 & 782,538\\
		5,100 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 716,970 & 86,576 & 0 & 0 & 0 & 0 & 803,546\\
		5,110 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 730,730 & 83,470 & 0 & 0 & 0 & 0 & 814,200\\
		5,120 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 706,583 & 81,191 & 0 & 0 & 0 & 0 & 787,774\\
		5,130 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 710,686 & 76,010 & 0 & 0 & 0 & 0 & 786,696\\
		5,140 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 723,220 & 74,799 & 0 & 0 & 0 & 0 & 798,019\\
		5,150 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 755,220 & 86,576 & 0 & 0 & 0 & 0 & 841,796\\
		5,160 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 700,991 & 83,667 & 0 & 0 & 0 & 0 & 784,658\\
		5,170 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 706,581 & 81,513 & 0 & 0 & 0 & 0 & 788,094\\
		5,180 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 708,151 & 83,019 & 0 & 0 & 0 & 0 & 791,170\\
		5,190 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 719,019 & 75,326 & 0 & 0 & 0 & 0 & 794,345\\
		5,200 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 754,648 & 81,394 & 0 & 0 & 0 & 0 & 836,042\\
		5,210 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 704,019 & 76,077 & 0 & 0 & 0 & 0 & 780,096\\
		5,220 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 706,583 & 75,694 & 0 & 0 & 0 & 0 & 782,277\\
		5,230 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 715,928 & 86,575 & 0 & 0 & 0 & 0 & 802,503\\
		5,240 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 750,619 & 83,639 & 0 & 0 & 0 & 0 & 834,258\\
		5,250 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 705,634 & 81,730 & 0 & 0 & 0 & 0 & 787,364\\
		5,260 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 712,010 & 77,675 & 0 & 0 & 0 & 0 & 789,685\\
		5,270 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 727,469 & 75,914 & 0 & 0 & 0 & 0 & 803,383\\
		5,280 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 703,931 & 90,034 & 0 & 0 & 0 & 0 & 793,965\\
		5,290 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 706,583 & 85,714 & 0 & 0 & 0 & 0 & 792,297\\
		5,300 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 724,242 & 82,527 & 0 & 0 & 0 & 0 & 806,769\\
		5,310 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 705,506 & 82,957 & 0 & 0 & 0 & 0 & 788,463\\
		5,320 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 713,640 & 86,472 & 0 & 0 & 0 & 0 & 800,112\\
		5,330 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 755,223 & 84,228 & 0 & 0 & 0 & 0 & 839,451\\
		5,340 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 710,534 & 86,289 & 0 & 0 & 0 & 0 & 796,823\\
		5,350 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 745,819 & 76,684 & 0 & 0 & 0 & 0 & 822,503\\
		5,360 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 708,533 & 81,319 & 0 & 0 & 0 & 0 & 789,852\\
		5,370 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 726,715 & 82,062 & 0 & 0 & 0 & 0 & 808,777\\
		5,380 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 706,583 & 81,860 & 0 & 0 & 0 & 0 & 788,443\\
		5,390 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 715,536 & 84,914 & 0 & 0 & 0 & 0 & 800,450\\
		5,400 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 754,249 & 87,812 & 0 & 0 & 0 & 0 & 842,061\\
		5,410 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 710,764 & 77,293 & 0 & 0 & 0 & 0 & 788,057\\
		5,420 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 755,223 & 77,691 & 0 & 0 & 0 & 0 & 832,914\\
		5,430 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 712,819 & 78,001 & 0 & 0 & 0 & 0 & 790,820\\
		5,440 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 737,941 & 81,263 & 0 & 0 & 0 & 0 & 819,204\\
		5,450 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 712,834 & 78,780 & 0 & 0 & 0 & 0 & 791,614\\
		5,460 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 706,583 & 79,962 & 0 & 0 & 0 & 0 & 786,545\\
		5,470 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 726,113 & 78,776 & 0 & 0 & 0 & 0 & 804,889\\
		5,480 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 754,894 & 88,575 & 0 & 0 & 0 & 0 & 843,469\\
		5,490 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 706,583 & 81,519 & 0 & 0 & 0 & 0 & 788,102\\
		5,500 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 721,904 & 81,270 & 0 & 0 & 0 & 0 & 803,174\\
		5,510 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 706,583 & 85,632 & 0 & 0 & 0 & 0 & 792,215\\
		5,520 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 755,224 & 86,576 & 0 & 0 & 0 & 0 & 841,800\\
		5,530 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 764,977 & 86,573 & 0 & 0 & 0 & 0 & 851,550\\
		5,540 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 770,845 & 86,894 & 0 & 0 & 0 & 0 & 857,739\\
		5,550 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 727,227 & 86,575 & 0 & 0 & 0 & 0 & 813,802\\
		5,560 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 737,466 & 86,575 & 0 & 0 & 0 & 0 & 824,041\\
		5,570 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 765,471 & 86,861 & 0 & 0 & 0 & 0 & 852,332\\
		5,580 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 779,781 & 86,573 & 0 & 0 & 0 & 0 & 866,354\\
		5,590 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 728,597 & 86,580 & 0 & 0 & 0 & 0 & 815,177\\
		5,600 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 754,787 & 86,572 & 0 & 0 & 0 & 0 & 841,359\\
		5,610 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 762,034 & 84,150 & 0 & 0 & 0 & 0 & 846,184\\
		5,620 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 852,409 & 86,576 & 0 & 0 & 0 & 0 & 938,985\\
		5,630 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 784,723 & 86,287 & 0 & 0 & 0 & 0 & 871,010\\
		5,640 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 758,824 & 85,774 & 0 & 0 & 0 & 0 & 844,598\\
		5,650 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 872,746 & 83,326 & 0 & 0 & 0 & 0 & 956,072\\
		5,660 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 838,511 & 81,864 & 0 & 0 & 0 & 0 & 920,375\\
		5,670 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 864,926 & 94,570 & 0 & 0 & 0 & 0 & 959,496\\
		5,680 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 760,567 & 82,434 & 0 & 0 & 0 & 0 & 843,001\\
		5,690 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 734,777 & 82,097 & 0 & 0 & 0 & 0 & 816,874\\
		5,700 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 755,224 & 82,184 & 0 & 0 & 0 & 0 & 837,408\\
		5,710 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 908,445 & 92,125 & 0 & 0 & 0 & 0 & 1,000,570\\
		5,720 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 790,889 & 89,279 & 0 & 0 & 0 & 0 & 880,168\\
		5,730 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 876,105 & 86,882 & 0 & 0 & 0 & 0 & 962,987\\
		5,740 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 934,965 & 86,538 & 0 & 0 & 0 & 0 & 1,021,503\\
		5,750 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 792,282 & 84,165 & 0 & 0 & 0 & 0 & 876,447\\
		5,760 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 890,925 & 82,983 & 0 & 0 & 0 & 0 & 973,908\\
		5,770 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 865,283 & 82,911 & 0 & 0 & 0 & 0 & 948,194\\
		5,780 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 922,679 & 82,833 & 0 & 0 & 0 & 0 & 1,005,512\\
		5,790 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 954,443 & 92,962 & 0 & 0 & 0 & 0 & 1,047,405\\
		5,800 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 829,482 & 89,278 & 0 & 0 & 0 & 0 & 918,760\\
		5,810 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 995,462 & 86,795 & 0 & 0 & 0 & 0 & 1,082,257\\
		5,820 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 903,693 & 86,791 & 0 & 0 & 0 & 0 & 990,484\\
		5,830 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 846,517 & 84,877 & 0 & 0 & 0 & 0 & 931,394\\
		5,840 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 917,649 & 83,649 & 0 & 0 & 0 & 0 & 1,001,298\\
		5,850 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,909 & 83,738 & 0 & 0 & 0 & 0 & 1,083,647\\
		5,860 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 898,374 & 83,427 & 0 & 0 & 0 & 0 & 981,801\\
		5,870 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 998,852 & 99,789 & 0 & 0 & 0 & 0 & 1,098,641\\
		5,880 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 971,761 & 92,904 & 0 & 0 & 0 & 0 & 1,064,665\\
		5,890 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 960,588 & 92,395 & 0 & 0 & 0 & 0 & 1,052,983\\
		5,900 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 931,762 & 88,579 & 0 & 0 & 0 & 0 & 1,020,341\\
		5,910 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 967,654 & 86,573 & 0 & 0 & 0 & 0 & 1,054,227\\
		5,920 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 993,976 & 86,278 & 0 & 0 & 0 & 0 & 1,080,254\\
		5,930 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,909 & 84,149 & 0 & 0 & 0 & 0 & 1,084,058\\
		5,940 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 910,671 & 97,803 & 0 & 0 & 0 & 0 & 1,008,474\\
		5,950 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 993,867 & 91,703 & 0 & 0 & 0 & 0 & 1,085,570\\
		5,960 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 987,170 & 87,892 & 0 & 0 & 0 & 0 & 1,075,062\\
		5,970 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,909 & 86,907 & 0 & 0 & 0 & 0 & 1,086,816\\
		5,980 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 966,775 & 86,538 & 0 & 0 & 0 & 0 & 1,053,313\\
		5,990 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 989,803 & 85,610 & 0 & 0 & 0 & 0 & 1,075,413\\
		6,000 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 982,926 & 84,509 & 0 & 0 & 0 & 0 & 1,067,435\\
		6,010 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 979,646 & 84,539 & 0 & 0 & 0 & 0 & 1,064,185\\
		6,020 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 996,570 & 84,245 & 0 & 0 & 0 & 0 & 1,080,815\\
		6,030 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 93,511 & 0 & 0 & 0 & 0 & 1,093,504\\
		6,040 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 985,097 & 88,048 & 0 & 0 & 0 & 0 & 1,073,145\\
		6,050 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 983,250 & 86,570 & 0 & 0 & 0 & 0 & 1,069,820\\
		6,060 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 84,851 & 0 & 0 & 0 & 0 & 1,084,844\\
		6,070 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 94,962 & 0 & 0 & 0 & 0 & 1,094,955\\
		6,080 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 89,222 & 0 & 0 & 0 & 0 & 1,089,215\\
		6,090 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 86,571 & 0 & 0 & 0 & 0 & 1,086,564\\
		6,100 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 84,829 & 0 & 0 & 0 & 0 & 1,084,822\\
		6,110 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 94,822 & 0 & 0 & 0 & 0 & 1,094,815\\
		6,120 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 89,244 & 0 & 0 & 0 & 0 & 1,089,237\\
		6,130 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 86,569 & 0 & 0 & 0 & 0 & 1,086,562\\
		6,140 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 84,850 & 0 & 0 & 0 & 0 & 1,084,843\\
		6,150 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 94,570 & 0 & 0 & 0 & 0 & 1,094,563\\
		6,160 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 88,996 & 0 & 0 & 0 & 0 & 1,088,989\\
		6,170 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 86,537 & 0 & 0 & 0 & 0 & 1,086,530\\
		6,180 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 84,797 & 0 & 0 & 0 & 0 & 1,084,790\\
		6,190 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,023 & 0 & 0 & 0 & 0 & 1,099,016\\
		6,200 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 89,729 & 0 & 0 & 0 & 0 & 1,089,722\\
		6,210 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 86,576 & 0 & 0 & 0 & 0 & 1,086,569\\
		6,220 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 84,900 & 0 & 0 & 0 & 0 & 1,084,893\\
		6,230 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,838 & 0 & 0 & 0 & 0 & 1,099,831\\
		6,240 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,582 & 0 & 0 & 0 & 0 & 1,099,575\\
		6,250 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,577 & 0 & 0 & 0 & 0 & 1,099,570\\
		6,260 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		6,270 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,586 & 0 & 0 & 0 & 0 & 1,099,579\\
		6,280 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,579 & 0 & 0 & 0 & 0 & 1,099,572\\
		6,290 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,575 & 0 & 0 & 0 & 0 & 1,099,568\\
		6,300 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		6,310 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 103,429 & 0 & 0 & 0 & 0 & 1,103,422\\
		6,320 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,592 & 0 & 0 & 0 & 0 & 1,099,585\\
		6,330 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,582 & 0 & 0 & 0 & 0 & 1,099,575\\
		6,340 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,578 & 0 & 0 & 0 & 0 & 1,099,571\\
		6,350 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,575 & 0 & 0 & 0 & 0 & 1,099,568\\
		6,360 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		6,370 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 103,045 & 0 & 0 & 0 & 0 & 1,103,038\\
		6,380 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,586 & 0 & 0 & 0 & 0 & 1,099,579\\
		6,390 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,580 & 0 & 0 & 0 & 0 & 1,099,573\\
		6,400 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,575 & 0 & 0 & 0 & 0 & 1,099,568\\
		6,410 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		6,420 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,571 & 0 & 0 & 0 & 0 & 1,099,564\\
		6,430 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,593 & 0 & 0 & 0 & 0 & 1,099,586\\
		6,440 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,582 & 0 & 0 & 0 & 0 & 1,099,575\\
		6,450 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,578 & 0 & 0 & 0 & 0 & 1,099,571\\
		6,460 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,574 & 0 & 0 & 0 & 0 & 1,099,567\\
		6,470 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		6,480 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 103,451 & 0 & 0 & 0 & 0 & 1,103,444\\
		6,490 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,586 & 0 & 0 & 0 & 0 & 1,099,579\\
		6,500 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,579 & 0 & 0 & 0 & 0 & 1,099,572\\
		6,510 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,575 & 0 & 0 & 0 & 0 & 1,099,568\\
		6,520 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		6,530 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 101,812 & 0 & 0 & 0 & 0 & 1,101,805\\
		6,540 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,586 & 0 & 0 & 0 & 0 & 1,099,579\\
		6,550 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,578 & 0 & 0 & 0 & 0 & 1,099,571\\
		6,560 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		6,570 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,571 & 0 & 0 & 0 & 0 & 1,099,564\\
		6,580 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,749 & 0 & 0 & 0 & 0 & 1,099,742\\
		6,590 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,583 & 0 & 0 & 0 & 0 & 1,099,576\\
		6,600 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,578 & 0 & 0 & 0 & 0 & 1,099,571\\
		6,610 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		6,620 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,571 & 0 & 0 & 0 & 0 & 1,099,564\\
		6,630 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,722 & 0 & 0 & 0 & 0 & 1,099,715\\
		6,640 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,582 & 0 & 0 & 0 & 0 & 1,099,575\\
		6,650 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,575 & 0 & 0 & 0 & 0 & 1,099,568\\
		6,660 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		6,670 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 105,631 & 0 & 0 & 0 & 0 & 1,105,624\\
		6,680 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,586 & 0 & 0 & 0 & 0 & 1,099,579\\
		6,690 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,579 & 0 & 0 & 0 & 0 & 1,099,572\\
		6,700 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		6,710 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,571 & 0 & 0 & 0 & 0 & 1,099,564\\
		6,720 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,754 & 0 & 0 & 0 & 0 & 1,099,747\\
		6,730 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,581 & 0 & 0 & 0 & 0 & 1,099,574\\
		6,740 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,575 & 0 & 0 & 0 & 0 & 1,099,568\\
		6,750 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		6,760 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,571 & 0 & 0 & 0 & 0 & 1,099,564\\
		6,770 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,761 & 0 & 0 & 0 & 0 & 1,099,754\\
		6,780 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,584 & 0 & 0 & 0 & 0 & 1,099,577\\
		6,790 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,577 & 0 & 0 & 0 & 0 & 1,099,570\\
		6,800 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		6,810 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,571 & 0 & 0 & 0 & 0 & 1,099,564\\
		6,820 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,653 & 0 & 0 & 0 & 0 & 1,099,646\\
		6,830 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,581 & 0 & 0 & 0 & 0 & 1,099,574\\
		6,840 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,575 & 0 & 0 & 0 & 0 & 1,099,568\\
		6,850 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		6,860 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 105,369 & 0 & 0 & 0 & 0 & 1,105,362\\
		6,870 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,722 & 0 & 0 & 0 & 0 & 1,099,715\\
		6,880 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,585 & 0 & 0 & 0 & 0 & 1,099,578\\
		6,890 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,578 & 0 & 0 & 0 & 0 & 1,099,571\\
		6,900 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,575 & 0 & 0 & 0 & 0 & 1,099,568\\
		6,910 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		6,920 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,571 & 0 & 0 & 0 & 0 & 1,099,564\\
		6,930 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 106,632 & 0 & 0 & 0 & 0 & 1,106,625\\
		6,940 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,722 & 0 & 0 & 0 & 0 & 1,099,715\\
		6,950 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,582 & 0 & 0 & 0 & 0 & 1,099,575\\
		6,960 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,576 & 0 & 0 & 0 & 0 & 1,099,569\\
		6,970 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		6,980 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,571 & 0 & 0 & 0 & 0 & 1,099,564\\
		6,990 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 105,369 & 0 & 0 & 0 & 0 & 1,105,362\\
		7,000 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,753 & 0 & 0 & 0 & 0 & 1,099,746\\
		7,010 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,586 & 0 & 0 & 0 & 0 & 1,099,579\\
		7,020 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,580 & 0 & 0 & 0 & 0 & 1,099,573\\
		7,030 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,576 & 0 & 0 & 0 & 0 & 1,099,569\\
		7,040 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		7,050 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,571 & 0 & 0 & 0 & 0 & 1,099,564\\
		7,060 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 103,413 & 0 & 0 & 0 & 0 & 1,103,406\\
		7,070 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,722 & 0 & 0 & 0 & 0 & 1,099,715\\
		7,080 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,585 & 0 & 0 & 0 & 0 & 1,099,578\\
		7,090 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,578 & 0 & 0 & 0 & 0 & 1,099,571\\
		7,100 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		7,110 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		7,120 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 103,514 & 0 & 0 & 0 & 0 & 1,103,507\\
		7,130 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,691 & 0 & 0 & 0 & 0 & 1,099,684\\
		7,140 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,581 & 0 & 0 & 0 & 0 & 1,099,574\\
		7,150 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,578 & 0 & 0 & 0 & 0 & 1,099,571\\
		7,160 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		7,170 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,571 & 0 & 0 & 0 & 0 & 1,099,564\\
		7,180 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 104,917 & 0 & 0 & 0 & 0 & 1,104,910\\
		7,190 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,725 & 0 & 0 & 0 & 0 & 1,099,718\\
		7,200 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,585 & 0 & 0 & 0 & 0 & 1,099,578\\
		7,210 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,578 & 0 & 0 & 0 & 0 & 1,099,571\\
		7,220 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,575 & 0 & 0 & 0 & 0 & 1,099,568\\
		7,230 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		7,240 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,571 & 0 & 0 & 0 & 0 & 1,099,564\\
		7,250 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 107,069 & 0 & 0 & 0 & 0 & 1,107,062\\
		7,260 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,795 & 0 & 0 & 0 & 0 & 1,099,788\\
		7,270 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,586 & 0 & 0 & 0 & 0 & 1,099,579\\
		7,280 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,583 & 0 & 0 & 0 & 0 & 1,099,576\\
		7,290 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,579 & 0 & 0 & 0 & 0 & 1,099,572\\
		7,300 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,575 & 0 & 0 & 0 & 0 & 1,099,568\\
		7,310 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		7,320 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,571 & 0 & 0 & 0 & 0 & 1,099,564\\
		7,330 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 101,048 & 0 & 0 & 0 & 0 & 1,101,041\\
		7,340 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,747 & 0 & 0 & 0 & 0 & 1,099,740\\
		7,350 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 101,736 & 0 & 0 & 0 & 0 & 1,101,729\\
		7,360 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,571 & 0 & 0 & 0 & 0 & 1,099,564\\
		7,370 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		7,380 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,571 & 0 & 0 & 0 & 0 & 1,099,564\\
		7,390 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,570 & 0 & 0 & 0 & 0 & 1,099,563\\
		7,400 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 101,736 & 0 & 0 & 0 & 0 & 1,101,729\\
		7,410 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,753 & 0 & 0 & 0 & 0 & 1,099,746\\
		7,420 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,586 & 0 & 0 & 0 & 0 & 1,099,579\\
		7,430 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,582 & 0 & 0 & 0 & 0 & 1,099,575\\
		7,440 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,579 & 0 & 0 & 0 & 0 & 1,099,572\\
		7,450 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,575 & 0 & 0 & 0 & 0 & 1,099,568\\
		7,460 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,573 & 0 & 0 & 0 & 0 & 1,099,566\\
		7,470 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		7,480 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,571 & 0 & 0 & 0 & 0 & 1,099,564\\
		7,490 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,571 & 0 & 0 & 0 & 0 & 1,099,564\\
		7,500 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 105,071 & 0 & 0 & 0 & 0 & 1,105,064\\
		7,510 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 100,310 & 0 & 0 & 0 & 0 & 1,100,303\\
		7,520 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,653 & 0 & 0 & 0 & 0 & 1,099,646\\
		7,530 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,586 & 0 & 0 & 0 & 0 & 1,099,579\\
		7,540 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,580 & 0 & 0 & 0 & 0 & 1,099,573\\
		7,550 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,578 & 0 & 0 & 0 & 0 & 1,099,571\\
		7,560 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,575 & 0 & 0 & 0 & 0 & 1,099,568\\
		7,570 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		7,580 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		7,590 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,571 & 0 & 0 & 0 & 0 & 1,099,564\\
		7,600 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,570 & 0 & 0 & 0 & 0 & 1,099,563\\
		7,610 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 106,587 & 0 & 0 & 0 & 0 & 1,106,580\\
		7,620 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 100,628 & 0 & 0 & 0 & 0 & 1,100,621\\
		7,630 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,691 & 0 & 0 & 0 & 0 & 1,099,684\\
		7,640 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,586 & 0 & 0 & 0 & 0 & 1,099,579\\
		7,650 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,580 & 0 & 0 & 0 & 0 & 1,099,573\\
		7,660 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,578 & 0 & 0 & 0 & 0 & 1,099,571\\
		7,670 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,575 & 0 & 0 & 0 & 0 & 1,099,568\\
		7,680 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		7,690 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		7,700 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,571 & 0 & 0 & 0 & 0 & 1,099,564\\
		7,710 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,571 & 0 & 0 & 0 & 0 & 1,099,564\\
		7,720 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,313 & 0 & 0 & 0 & 0 & 1,109,306\\
		7,730 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 101,736 & 0 & 0 & 0 & 0 & 1,101,729\\
		7,740 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,759 & 0 & 0 & 0 & 0 & 1,099,752\\
		7,750 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,586 & 0 & 0 & 0 & 0 & 1,099,579\\
		7,760 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,584 & 0 & 0 & 0 & 0 & 1,099,577\\
		7,770 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,579 & 0 & 0 & 0 & 0 & 1,099,572\\
		7,780 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,578 & 0 & 0 & 0 & 0 & 1,099,571\\
		7,790 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,575 & 0 & 0 & 0 & 0 & 1,099,568\\
		7,800 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		7,810 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		7,820 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,571 & 0 & 0 & 0 & 0 & 1,099,564\\
		7,830 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,782 & 0 & 0 & 0 & 0 & 1,109,775\\
		7,840 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 103,473 & 0 & 0 & 0 & 0 & 1,103,466\\
		7,850 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,797 & 0 & 0 & 0 & 0 & 1,099,790\\
		7,860 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,593 & 0 & 0 & 0 & 0 & 1,099,586\\
		7,870 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,586 & 0 & 0 & 0 & 0 & 1,099,579\\
		7,880 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,580 & 0 & 0 & 0 & 0 & 1,099,573\\
		7,890 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,579 & 0 & 0 & 0 & 0 & 1,099,572\\
		7,900 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		7,910 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,586 & 0 & 0 & 0 & 0 & 1,099,579\\
		7,920 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,585 & 0 & 0 & 0 & 0 & 1,099,578\\
		7,930 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,579 & 0 & 0 & 0 & 0 & 1,099,572\\
		7,940 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,578 & 0 & 0 & 0 & 0 & 1,099,571\\
		7,950 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,575 & 0 & 0 & 0 & 0 & 1,099,568\\
		7,960 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		7,970 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		7,980 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,571 & 0 & 0 & 0 & 0 & 1,099,564\\
		7,990 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 110,100 & 0 & 0 & 0 & 0 & 1,110,093\\
		8,000 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,296 & 0 & 0 & 0 & 0 & 1,109,289\\
		8,010 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 101,728 & 0 & 0 & 0 & 0 & 1,101,721\\
		8,020 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,760 & 0 & 0 & 0 & 0 & 1,099,753\\
		8,030 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,586 & 0 & 0 & 0 & 0 & 1,099,579\\
		8,040 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,584 & 0 & 0 & 0 & 0 & 1,099,577\\
		8,050 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,579 & 0 & 0 & 0 & 0 & 1,099,572\\
		8,060 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,578 & 0 & 0 & 0 & 0 & 1,099,571\\
		8,070 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,575 & 0 & 0 & 0 & 0 & 1,099,568\\
		8,080 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		8,090 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		8,100 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,571 & 0 & 0 & 0 & 0 & 1,099,564\\
		8,110 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 110,154 & 0 & 0 & 0 & 0 & 1,110,147\\
		8,120 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,311 & 0 & 0 & 0 & 0 & 1,109,304\\
		8,130 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 102,426 & 0 & 0 & 0 & 0 & 1,102,419\\
		8,140 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,792 & 0 & 0 & 0 & 0 & 1,099,785\\
		8,150 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,591 & 0 & 0 & 0 & 0 & 1,099,584\\
		8,160 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,586 & 0 & 0 & 0 & 0 & 1,099,579\\
		8,170 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,580 & 0 & 0 & 0 & 0 & 1,099,573\\
		8,180 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,578 & 0 & 0 & 0 & 0 & 1,099,571\\
		8,190 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,575 & 0 & 0 & 0 & 0 & 1,099,568\\
		8,200 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		8,210 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		8,220 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,571 & 0 & 0 & 0 & 0 & 1,099,564\\
		8,230 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,571 & 0 & 0 & 0 & 0 & 1,099,564\\
		8,240 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,769 & 0 & 0 & 0 & 0 & 1,109,762\\
		8,250 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 106,587 & 0 & 0 & 0 & 0 & 1,106,580\\
		8,260 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 101,180 & 0 & 0 & 0 & 0 & 1,101,173\\
		8,270 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,753 & 0 & 0 & 0 & 0 & 1,099,746\\
		8,280 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,586 & 0 & 0 & 0 & 0 & 1,099,579\\
		8,290 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,584 & 0 & 0 & 0 & 0 & 1,099,577\\
		8,300 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,579 & 0 & 0 & 0 & 0 & 1,099,572\\
		8,310 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,578 & 0 & 0 & 0 & 0 & 1,099,571\\
		8,320 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,575 & 0 & 0 & 0 & 0 & 1,099,568\\
		8,330 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		8,340 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		8,350 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,571 & 0 & 0 & 0 & 0 & 1,099,564\\
		8,360 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,078 & 0 & 0 & 0 & 0 & 1,112,071\\
		8,370 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,748 & 0 & 0 & 0 & 0 & 1,109,741\\
		8,380 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 108,518 & 0 & 0 & 0 & 0 & 1,108,511\\
		8,390 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 101,728 & 0 & 0 & 0 & 0 & 1,101,721\\
		8,400 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,760 & 0 & 0 & 0 & 0 & 1,099,753\\
		8,410 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 105,048 & 0 & 0 & 0 & 0 & 1,105,041\\
		8,420 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,586 & 0 & 0 & 0 & 0 & 1,099,579\\
		8,430 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,579 & 0 & 0 & 0 & 0 & 1,099,572\\
		8,440 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,577 & 0 & 0 & 0 & 0 & 1,099,570\\
		8,450 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		8,460 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 117,117 & 0 & 0 & 0 & 0 & 1,117,110\\
		8,470 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,818 & 0 & 0 & 0 & 0 & 1,109,811\\
		8,480 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 108,518 & 0 & 0 & 0 & 0 & 1,108,511\\
		8,490 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 101,050 & 0 & 0 & 0 & 0 & 1,101,043\\
		8,500 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,591 & 0 & 0 & 0 & 0 & 1,099,584\\
		8,510 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,581 & 0 & 0 & 0 & 0 & 1,099,574\\
		8,520 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,579 & 0 & 0 & 0 & 0 & 1,099,572\\
		8,530 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,576 & 0 & 0 & 0 & 0 & 1,099,569\\
		8,540 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,575 & 0 & 0 & 0 & 0 & 1,099,568\\
		8,550 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		8,560 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 118,602 & 0 & 0 & 0 & 0 & 1,118,595\\
		8,570 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 110,103 & 0 & 0 & 0 & 0 & 1,110,096\\
		8,580 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,620 & 0 & 0 & 0 & 0 & 1,109,613\\
		8,590 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 103,339 & 0 & 0 & 0 & 0 & 1,103,332\\
		8,600 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 101,055 & 0 & 0 & 0 & 0 & 1,101,048\\
		8,610 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,722 & 0 & 0 & 0 & 0 & 1,099,715\\
		8,620 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,583 & 0 & 0 & 0 & 0 & 1,099,576\\
		8,630 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,578 & 0 & 0 & 0 & 0 & 1,099,571\\
		8,640 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,574 & 0 & 0 & 0 & 0 & 1,099,567\\
		8,650 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 121,411 & 0 & 0 & 0 & 0 & 1,121,404\\
		8,660 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,182 & 0 & 0 & 0 & 0 & 1,112,175\\
		8,670 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 110,125 & 0 & 0 & 0 & 0 & 1,110,118\\
		8,680 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,571 & 0 & 0 & 0 & 0 & 1,109,564\\
		8,690 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 101,970 & 0 & 0 & 0 & 0 & 1,101,963\\
		8,700 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,760 & 0 & 0 & 0 & 0 & 1,099,753\\
		8,710 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,585 & 0 & 0 & 0 & 0 & 1,099,578\\
		8,720 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 101,783 & 0 & 0 & 0 & 0 & 1,101,776\\
		8,730 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,722 & 0 & 0 & 0 & 0 & 1,099,715\\
		8,740 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,585 & 0 & 0 & 0 & 0 & 1,099,578\\
		8,750 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,578 & 0 & 0 & 0 & 0 & 1,099,571\\
		8,760 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,578 & 0 & 0 & 0 & 0 & 1,099,571\\
		8,770 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,575 & 0 & 0 & 0 & 0 & 1,099,568\\
		8,780 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,572 & 0 & 0 & 0 & 0 & 1,099,565\\
		8,790 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 117,955 & 0 & 0 & 0 & 0 & 1,117,948\\
		8,800 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 111,765 & 0 & 0 & 0 & 0 & 1,111,758\\
		8,810 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,973 & 0 & 0 & 0 & 0 & 1,109,966\\
		8,820 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,667 & 0 & 0 & 0 & 0 & 1,109,660\\
		8,830 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 106,640 & 0 & 0 & 0 & 0 & 1,106,633\\
		8,840 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 101,941 & 0 & 0 & 0 & 0 & 1,101,934\\
		8,850 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,724 & 0 & 0 & 0 & 0 & 1,109,717\\
		8,860 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 106,680 & 0 & 0 & 0 & 0 & 1,106,673\\
		8,870 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 102,938 & 0 & 0 & 0 & 0 & 1,102,931\\
		8,880 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 101,143 & 0 & 0 & 0 & 0 & 1,101,136\\
		8,890 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,779 & 0 & 0 & 0 & 0 & 1,099,772\\
		8,900 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,592 & 0 & 0 & 0 & 0 & 1,099,585\\
		8,910 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,586 & 0 & 0 & 0 & 0 & 1,099,579\\
		8,920 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,580 & 0 & 0 & 0 & 0 & 1,099,573\\
		8,930 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,578 & 0 & 0 & 0 & 0 & 1,099,571\\
		8,940 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,575 & 0 & 0 & 0 & 0 & 1,099,568\\
		8,950 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 117,966 & 0 & 0 & 0 & 0 & 1,117,959\\
		8,960 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 120,042 & 0 & 0 & 0 & 0 & 1,120,035\\
		8,970 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,182 & 0 & 0 & 0 & 0 & 1,112,175\\
		8,980 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 111,658 & 0 & 0 & 0 & 0 & 1,111,651\\
		8,990 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,855 & 0 & 0 & 0 & 0 & 1,109,848\\
		9,000 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,472 & 0 & 0 & 0 & 0 & 1,109,465\\
		9,010 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 105,676 & 0 & 0 & 0 & 0 & 1,105,669\\
		9,020 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 104,788 & 0 & 0 & 0 & 0 & 1,104,781\\
		9,030 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 102,874 & 0 & 0 & 0 & 0 & 1,102,867\\
		9,040 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 101,143 & 0 & 0 & 0 & 0 & 1,101,136\\
		9,050 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,761 & 0 & 0 & 0 & 0 & 1,099,754\\
		9,060 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,589 & 0 & 0 & 0 & 0 & 1,099,582\\
		9,070 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,586 & 0 & 0 & 0 & 0 & 1,099,579\\
		9,080 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,580 & 0 & 0 & 0 & 0 & 1,099,573\\
		9,090 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 120,042 & 0 & 0 & 0 & 0 & 1,120,035\\
		9,100 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 113,017 & 0 & 0 & 0 & 0 & 1,113,010\\
		9,110 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,017 & 0 & 0 & 0 & 0 & 1,112,010\\
		9,120 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 110,640 & 0 & 0 & 0 & 0 & 1,110,633\\
		9,130 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,787 & 0 & 0 & 0 & 0 & 1,109,780\\
		9,140 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,304 & 0 & 0 & 0 & 0 & 1,109,297\\
		9,150 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 106,288 & 0 & 0 & 0 & 0 & 1,106,281\\
		9,160 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 104,859 & 0 & 0 & 0 & 0 & 1,104,852\\
		9,170 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 103,144 & 0 & 0 & 0 & 0 & 1,103,137\\
		9,180 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 101,255 & 0 & 0 & 0 & 0 & 1,101,248\\
		9,190 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,795 & 0 & 0 & 0 & 0 & 1,099,788\\
		9,200 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,685 & 0 & 0 & 0 & 0 & 1,099,678\\
		9,210 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,586 & 0 & 0 & 0 & 0 & 1,099,579\\
		9,220 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 119,983 & 0 & 0 & 0 & 0 & 1,119,976\\
		9,230 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,706 & 0 & 0 & 0 & 0 & 1,112,699\\
		9,240 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,238 & 0 & 0 & 0 & 0 & 1,112,231\\
		9,250 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 111,755 & 0 & 0 & 0 & 0 & 1,111,748\\
		9,260 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,970 & 0 & 0 & 0 & 0 & 1,109,963\\
		9,270 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,620 & 0 & 0 & 0 & 0 & 1,109,613\\
		9,280 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 107,275 & 0 & 0 & 0 & 0 & 1,107,268\\
		9,290 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 106,387 & 0 & 0 & 0 & 0 & 1,106,380\\
		9,300 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 105,886 & 0 & 0 & 0 & 0 & 1,105,879\\
		9,310 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 104,984 & 0 & 0 & 0 & 0 & 1,104,977\\
		9,320 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 103,404 & 0 & 0 & 0 & 0 & 1,103,397\\
		9,330 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,472 & 0 & 0 & 0 & 0 & 1,109,465\\
		9,340 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,156 & 0 & 0 & 0 & 0 & 1,112,149\\
		9,350 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,939 & 0 & 0 & 0 & 0 & 1,109,932\\
		9,360 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 108,917 & 0 & 0 & 0 & 0 & 1,108,910\\
		9,370 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 106,061 & 0 & 0 & 0 & 0 & 1,106,054\\
		9,380 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 104,749 & 0 & 0 & 0 & 0 & 1,104,742\\
		9,390 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 101,143 & 0 & 0 & 0 & 0 & 1,101,136\\
		9,400 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,792 & 0 & 0 & 0 & 0 & 1,099,785\\
		9,410 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 120,145 & 0 & 0 & 0 & 0 & 1,120,138\\
		9,420 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,380 & 0 & 0 & 0 & 0 & 1,112,373\\
		9,430 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,152 & 0 & 0 & 0 & 0 & 1,112,145\\
		9,440 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 110,076 & 0 & 0 & 0 & 0 & 1,110,069\\
		9,450 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,648 & 0 & 0 & 0 & 0 & 1,109,641\\
		9,460 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 107,401 & 0 & 0 & 0 & 0 & 1,107,394\\
		9,470 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 106,612 & 0 & 0 & 0 & 0 & 1,106,605\\
		9,480 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 105,735 & 0 & 0 & 0 & 0 & 1,105,728\\
		9,490 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 104,920 & 0 & 0 & 0 & 0 & 1,104,913\\
		9,500 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 103,045 & 0 & 0 & 0 & 0 & 1,103,038\\
		9,510 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 101,172 & 0 & 0 & 0 & 0 & 1,101,165\\
		9,520 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,938 & 0 & 0 & 0 & 0 & 1,099,931\\
		9,530 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,721 & 0 & 0 & 0 & 0 & 1,099,714\\
		9,540 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 120,033 & 0 & 0 & 0 & 0 & 1,120,026\\
		9,550 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 116,253 & 0 & 0 & 0 & 0 & 1,116,246\\
		9,560 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,355 & 0 & 0 & 0 & 0 & 1,112,348\\
		9,570 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,182 & 0 & 0 & 0 & 0 & 1,112,175\\
		9,580 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 100,133 & 0 & 0 & 0 & 0 & 1,100,126\\
		9,590 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,754 & 0 & 0 & 0 & 0 & 1,099,747\\
		9,600 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 122,039 & 0 & 0 & 0 & 0 & 1,122,032\\
		9,610 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 117,920 & 0 & 0 & 0 & 0 & 1,117,913\\
		9,620 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 103,413 & 0 & 0 & 0 & 0 & 1,103,406\\
		9,630 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 101,772 & 0 & 0 & 0 & 0 & 1,101,765\\
		9,640 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 100,222 & 0 & 0 & 0 & 0 & 1,100,215\\
		9,650 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 99,797 & 0 & 0 & 0 & 0 & 1,099,790\\
		9,660 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 123,716 & 0 & 0 & 0 & 0 & 1,123,709\\
		9,670 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 119,457 & 0 & 0 & 0 & 0 & 1,119,450\\
		9,680 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 113,017 & 0 & 0 & 0 & 0 & 1,113,010\\
		9,690 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,372 & 0 & 0 & 0 & 0 & 1,112,365\\
		9,700 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,238 & 0 & 0 & 0 & 0 & 1,112,231\\
		9,710 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 111,791 & 0 & 0 & 0 & 0 & 1,111,784\\
		9,720 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 110,187 & 0 & 0 & 0 & 0 & 1,110,180\\
		9,730 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,782 & 0 & 0 & 0 & 0 & 1,109,775\\
		9,740 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,312 & 0 & 0 & 0 & 0 & 1,109,305\\
		9,750 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 107,184 & 0 & 0 & 0 & 0 & 1,107,177\\
		9,760 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 106,456 & 0 & 0 & 0 & 0 & 1,106,449\\
		9,770 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 105,149 & 0 & 0 & 0 & 0 & 1,105,142\\
		9,780 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 106,440 & 0 & 0 & 0 & 0 & 1,106,433\\
		9,790 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 106,640 & 0 & 0 & 0 & 0 & 1,106,633\\
		9,800 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 105,813 & 0 & 0 & 0 & 0 & 1,105,806\\
		9,810 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 104,842 & 0 & 0 & 0 & 0 & 1,104,835\\
		9,820 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 102,426 & 0 & 0 & 0 & 0 & 1,102,419\\
		9,830 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 101,050 & 0 & 0 & 0 & 0 & 1,101,043\\
		9,840 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 128,199 & 0 & 0 & 0 & 0 & 1,128,192\\
		9,850 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 119,983 & 0 & 0 & 0 & 0 & 1,119,976\\
		9,860 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 115,233 & 0 & 0 & 0 & 0 & 1,115,226\\
		9,870 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 113,509 & 0 & 0 & 0 & 0 & 1,113,502\\
		9,880 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,383 & 0 & 0 & 0 & 0 & 1,112,376\\
		9,890 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,238 & 0 & 0 & 0 & 0 & 1,112,231\\
		9,900 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 111,765 & 0 & 0 & 0 & 0 & 1,111,758\\
		9,910 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 110,087 & 0 & 0 & 0 & 0 & 1,110,080\\
		9,920 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,692 & 0 & 0 & 0 & 0 & 1,109,685\\
		9,930 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 108,664 & 0 & 0 & 0 & 0 & 1,108,657\\
		9,940 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 106,640 & 0 & 0 & 0 & 0 & 1,106,633\\
		9,950 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 105,688 & 0 & 0 & 0 & 0 & 1,105,681\\
		9,960 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 104,899 & 0 & 0 & 0 & 0 & 1,104,892\\
		9,970 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 102,951 & 0 & 0 & 0 & 0 & 1,102,944\\
		9,980 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 101,299 & 0 & 0 & 0 & 0 & 1,101,292\\
		9,990 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 130,571 & 0 & 0 & 0 & 0 & 1,130,564\\
		10,000 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 119,992 & 0 & 0 & 0 & 0 & 1,119,985\\
		10,010 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 114,325 & 0 & 0 & 0 & 0 & 1,114,318\\
		10,020 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 113,417 & 0 & 0 & 0 & 0 & 1,113,410\\
		10,030 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,394 & 0 & 0 & 0 & 0 & 1,112,387\\
		10,040 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,235 & 0 & 0 & 0 & 0 & 1,112,228\\
		10,050 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 111,726 & 0 & 0 & 0 & 0 & 1,111,719\\
		10,060 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,905 & 0 & 0 & 0 & 0 & 1,109,898\\
		10,070 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,452 & 0 & 0 & 0 & 0 & 1,109,445\\
		10,080 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 107,246 & 0 & 0 & 0 & 0 & 1,107,239\\
		10,090 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 106,288 & 0 & 0 & 0 & 0 & 1,106,281\\
		10,100 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 105,108 & 0 & 0 & 0 & 0 & 1,105,101\\
		10,110 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 103,473 & 0 & 0 & 0 & 0 & 1,103,466\\
		10,120 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 101,831 & 0 & 0 & 0 & 0 & 1,101,824\\
		10,130 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 100,310 & 0 & 0 & 0 & 0 & 1,100,303\\
		10,140 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 123,191 & 0 & 0 & 0 & 0 & 1,123,184\\
		10,150 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 117,919 & 0 & 0 & 0 & 0 & 1,117,912\\
		10,160 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 113,511 & 0 & 0 & 0 & 0 & 1,113,504\\
		10,170 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 113,511 & 0 & 0 & 0 & 0 & 1,113,504\\
		10,180 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 113,388 & 0 & 0 & 0 & 0 & 1,113,381\\
		10,190 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,651 & 0 & 0 & 0 & 0 & 1,112,644\\
		10,200 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,351 & 0 & 0 & 0 & 0 & 1,112,344\\
		10,210 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,221 & 0 & 0 & 0 & 0 & 1,112,214\\
		10,220 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 111,829 & 0 & 0 & 0 & 0 & 1,111,822\\
		10,230 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 110,215 & 0 & 0 & 0 & 0 & 1,110,208\\
		10,240 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,813 & 0 & 0 & 0 & 0 & 1,109,806\\
		10,250 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,391 & 0 & 0 & 0 & 0 & 1,109,384\\
		10,260 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 108,073 & 0 & 0 & 0 & 0 & 1,108,066\\
		10,270 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 106,723 & 0 & 0 & 0 & 0 & 1,106,716\\
		10,280 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 105,990 & 0 & 0 & 0 & 0 & 1,105,983\\
		10,290 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 105,102 & 0 & 0 & 0 & 0 & 1,105,095\\
		10,300 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 104,717 & 0 & 0 & 0 & 0 & 1,104,710\\
		10,310 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 102,529 & 0 & 0 & 0 & 0 & 1,102,522\\
		10,320 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 101,143 & 0 & 0 & 0 & 0 & 1,101,136\\
		10,330 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 123,584 & 0 & 0 & 0 & 0 & 1,123,577\\
		10,340 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 119,983 & 0 & 0 & 0 & 0 & 1,119,976\\
		10,350 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 117,576 & 0 & 0 & 0 & 0 & 1,117,569\\
		10,360 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 113,511 & 0 & 0 & 0 & 0 & 1,113,504\\
		10,370 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 113,393 & 0 & 0 & 0 & 0 & 1,113,386\\
		10,380 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,940 & 0 & 0 & 0 & 0 & 1,112,933\\
		10,390 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,553 & 0 & 0 & 0 & 0 & 1,112,546\\
		10,400 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,341 & 0 & 0 & 0 & 0 & 1,112,334\\
		10,410 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,156 & 0 & 0 & 0 & 0 & 1,112,149\\
		10,420 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 111,717 & 0 & 0 & 0 & 0 & 1,111,710\\
		10,430 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 110,126 & 0 & 0 & 0 & 0 & 1,110,119\\
		10,440 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,763 & 0 & 0 & 0 & 0 & 1,109,756\\
		10,450 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,312 & 0 & 0 & 0 & 0 & 1,109,305\\
		10,460 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 107,239 & 0 & 0 & 0 & 0 & 1,107,232\\
		10,470 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 106,595 & 0 & 0 & 0 & 0 & 1,106,588\\
		10,480 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 105,813 & 0 & 0 & 0 & 0 & 1,105,806\\
		10,490 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 105,048 & 0 & 0 & 0 & 0 & 1,105,041\\
		10,500 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 104,067 & 0 & 0 & 0 & 0 & 1,104,060\\
		10,510 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 101,941 & 0 & 0 & 0 & 0 & 1,101,934\\
		10,520 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 123,580 & 0 & 0 & 0 & 0 & 1,123,573\\
		10,530 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 119,959 & 0 & 0 & 0 & 0 & 1,119,952\\
		10,540 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 117,457 & 0 & 0 & 0 & 0 & 1,117,450\\
		10,550 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 113,511 & 0 & 0 & 0 & 0 & 1,113,504\\
		10,560 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 113,376 & 0 & 0 & 0 & 0 & 1,113,369\\
		10,570 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,940 & 0 & 0 & 0 & 0 & 1,112,933\\
		10,580 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,683 & 0 & 0 & 0 & 0 & 1,112,676\\
		10,590 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 130,571 & 0 & 0 & 0 & 0 & 1,130,564\\
		10,600 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 105,224 & 0 & 0 & 0 & 0 & 1,105,217\\
		10,610 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,391 & 0 & 0 & 0 & 0 & 1,109,384\\
		10,620 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 111,830 & 0 & 0 & 0 & 0 & 1,111,823\\
		10,630 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,221 & 0 & 0 & 0 & 0 & 1,112,214\\
		10,640 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,649 & 0 & 0 & 0 & 0 & 1,112,642\\
		10,650 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 113,254 & 0 & 0 & 0 & 0 & 1,113,247\\
		10,660 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 113,511 & 0 & 0 & 0 & 0 & 1,113,504\\
		10,670 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 117,347 & 0 & 0 & 0 & 0 & 1,117,340\\
		10,680 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 138,603 & 0 & 0 & 0 & 0 & 1,138,596\\
		10,690 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 104,740 & 0 & 0 & 0 & 0 & 1,104,733\\
		10,700 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 104,266 & 0 & 0 & 0 & 0 & 1,104,259\\
		10,710 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 131,268 & 0 & 0 & 0 & 0 & 1,131,261\\
		10,720 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,312 & 0 & 0 & 0 & 0 & 1,109,305\\
		10,730 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,409 & 0 & 0 & 0 & 0 & 1,109,402\\
		10,740 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 108,664 & 0 & 0 & 0 & 0 & 1,108,657\\
		10,750 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,311 & 0 & 0 & 0 & 0 & 1,109,304\\
		10,760 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,312 & 0 & 0 & 0 & 0 & 1,109,305\\
		10,770 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,742 & 0 & 0 & 0 & 0 & 1,109,735\\
		10,780 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,862 & 0 & 0 & 0 & 0 & 1,109,855\\
		10,790 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,650 & 0 & 0 & 0 & 0 & 1,109,643\\
		10,800 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 108,579 & 0 & 0 & 0 & 0 & 1,108,572\\
		10,810 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 106,595 & 0 & 0 & 0 & 0 & 1,106,588\\
		10,820 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 105,324 & 0 & 0 & 0 & 0 & 1,105,317\\
		10,830 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 133,181 & 0 & 0 & 0 & 0 & 1,133,174\\
		10,840 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 121,090 & 0 & 0 & 0 & 0 & 1,121,083\\
		10,850 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 117,385 & 0 & 0 & 0 & 0 & 1,117,378\\
		10,860 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 113,511 & 0 & 0 & 0 & 0 & 1,113,504\\
		10,870 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,910 & 0 & 0 & 0 & 0 & 1,112,903\\
		10,880 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,378 & 0 & 0 & 0 & 0 & 1,112,371\\
		10,890 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,045 & 0 & 0 & 0 & 0 & 1,112,038\\
		10,900 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 110,187 & 0 & 0 & 0 & 0 & 1,110,180\\
		10,910 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,571 & 0 & 0 & 0 & 0 & 1,109,564\\
		10,920 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 107,112 & 0 & 0 & 0 & 0 & 1,107,105\\
		10,930 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 105,841 & 0 & 0 & 0 & 0 & 1,105,834\\
		10,940 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 104,647 & 0 & 0 & 0 & 0 & 1,104,640\\
		10,950 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 123,238 & 0 & 0 & 0 & 0 & 1,123,231\\
		10,960 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 117,950 & 0 & 0 & 0 & 0 & 1,117,943\\
		10,970 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 119,357 & 0 & 0 & 0 & 0 & 1,119,350\\
		10,980 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 121,499 & 0 & 0 & 0 & 0 & 1,121,492\\
		10,990 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 118,222 & 0 & 0 & 0 & 0 & 1,118,215\\
		11,000 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 116,302 & 0 & 0 & 0 & 0 & 1,116,295\\
		11,010 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 113,511 & 0 & 0 & 0 & 0 & 1,113,504\\
		11,020 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 113,394 & 0 & 0 & 0 & 0 & 1,113,387\\
		11,030 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,726 & 0 & 0 & 0 & 0 & 1,112,719\\
		11,040 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,374 & 0 & 0 & 0 & 0 & 1,112,367\\
		11,050 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 111,869 & 0 & 0 & 0 & 0 & 1,111,862\\
		11,060 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,936 & 0 & 0 & 0 & 0 & 1,109,929\\
		11,070 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,405 & 0 & 0 & 0 & 0 & 1,109,398\\
		11,080 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 107,115 & 0 & 0 & 0 & 0 & 1,107,108\\
		11,090 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 105,928 & 0 & 0 & 0 & 0 & 1,105,921\\
		11,100 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 104,899 & 0 & 0 & 0 & 0 & 1,104,892\\
		11,110 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 125,024 & 0 & 0 & 0 & 0 & 1,125,017\\
		11,120 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 120,042 & 0 & 0 & 0 & 0 & 1,120,035\\
		11,130 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 117,862 & 0 & 0 & 0 & 0 & 1,117,855\\
		11,140 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 114,127 & 0 & 0 & 0 & 0 & 1,114,120\\
		11,150 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 113,400 & 0 & 0 & 0 & 0 & 1,113,393\\
		11,160 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,870 & 0 & 0 & 0 & 0 & 1,112,863\\
		11,170 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 112,341 & 0 & 0 & 0 & 0 & 1,112,334\\
		11,180 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 111,787 & 0 & 0 & 0 & 0 & 1,111,780\\
		11,190 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,954 & 0 & 0 & 0 & 0 & 1,109,947\\
		11,200 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 109,370 & 0 & 0 & 0 & 0 & 1,109,363\\
		11,210 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 106,812 & 0 & 0 & 0 & 0 & 1,106,805\\
		11,220 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 105,499 & 0 & 0 & 0 & 0 & 1,105,492\\
		11,230 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 999,993 & 126,710 & 0 & 0 & 0 & 0 & 1,126,703\\
		11,240 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 119,655 & 0 & 0 & 0 & 0 & 119,655\\
		11,250 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 116,323 & 0 & 0 & 0 & 0 & 116,323\\
		11,260 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 114,303 & 0 & 0 & 0 & 0 & 114,303\\
		11,270 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,511 & 0 & 0 & 0 & 0 & 113,511\\
		11,280 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,120 & 0 & 0 & 0 & 0 & 113,120\\
		11,290 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,686 & 0 & 0 & 0 & 0 & 112,686\\
		11,300 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,348 & 0 & 0 & 0 & 0 & 112,348\\
		11,310 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,245 & 0 & 0 & 0 & 0 & 112,245\\
		11,320 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,969 & 0 & 0 & 0 & 0 & 111,969\\
		11,330 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,476 & 0 & 0 & 0 & 0 & 111,476\\
		11,340 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,165 & 0 & 0 & 0 & 0 & 110,165\\
		11,350 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,224 & 0 & 0 & 0 & 0 & 112,224\\
		11,360 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,216 & 0 & 0 & 0 & 0 & 110,216\\
		11,370 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,393 & 0 & 0 & 0 & 0 & 112,393\\
		11,380 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,319 & 0 & 0 & 0 & 0 & 112,319\\
		11,390 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,035 & 0 & 0 & 0 & 0 & 112,035\\
		11,400 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,690 & 0 & 0 & 0 & 0 & 111,690\\
		11,410 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,215 & 0 & 0 & 0 & 0 & 110,215\\
		11,420 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,815 & 0 & 0 & 0 & 0 & 109,815\\
		11,430 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,137 & 0 & 0 & 0 & 0 & 112,137\\
		11,440 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,755 & 0 & 0 & 0 & 0 & 111,755\\
		11,450 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,311 & 0 & 0 & 0 & 0 & 110,311\\
		11,460 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,845 & 0 & 0 & 0 & 0 & 109,845\\
		11,470 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,648 & 0 & 0 & 0 & 0 & 109,648\\
		11,480 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,327 & 0 & 0 & 0 & 0 & 109,327\\
		11,490 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,322 & 0 & 0 & 0 & 0 & 109,322\\
		11,500 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,321 & 0 & 0 & 0 & 0 & 109,321\\
		11,510 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 145,285 & 0 & 0 & 0 & 0 & 145,285\\
		11,520 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,002 & 0 & 0 & 0 & 0 & 112,002\\
		11,530 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,485 & 0 & 0 & 0 & 0 & 111,485\\
		11,540 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,640 & 0 & 0 & 0 & 0 & 110,640\\
		11,550 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,864 & 0 & 0 & 0 & 0 & 109,864\\
		11,560 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,712 & 0 & 0 & 0 & 0 & 109,712\\
		11,570 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,329 & 0 & 0 & 0 & 0 & 109,329\\
		11,580 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,323 & 0 & 0 & 0 & 0 & 109,323\\
		11,590 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 140,075 & 0 & 0 & 0 & 0 & 140,075\\
		11,600 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 127,625 & 0 & 0 & 0 & 0 & 127,625\\
		11,610 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 123,250 & 0 & 0 & 0 & 0 & 123,250\\
		11,620 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 119,998 & 0 & 0 & 0 & 0 & 119,998\\
		11,630 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 117,981 & 0 & 0 & 0 & 0 & 117,981\\
		11,640 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 116,811 & 0 & 0 & 0 & 0 & 116,811\\
		11,650 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 116,014 & 0 & 0 & 0 & 0 & 116,014\\
		11,660 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 115,247 & 0 & 0 & 0 & 0 & 115,247\\
		11,670 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 114,386 & 0 & 0 & 0 & 0 & 114,386\\
		11,680 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,954 & 0 & 0 & 0 & 0 & 113,954\\
		11,690 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,820 & 0 & 0 & 0 & 0 & 113,820\\
		11,700 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,511 & 0 & 0 & 0 & 0 & 113,511\\
		11,710 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,376 & 0 & 0 & 0 & 0 & 113,376\\
		11,720 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,964 & 0 & 0 & 0 & 0 & 112,964\\
		11,730 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,703 & 0 & 0 & 0 & 0 & 112,703\\
		11,740 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,383 & 0 & 0 & 0 & 0 & 112,383\\
		11,750 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,317 & 0 & 0 & 0 & 0 & 112,317\\
		11,760 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,035 & 0 & 0 & 0 & 0 & 112,035\\
		11,770 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,695 & 0 & 0 & 0 & 0 & 111,695\\
		11,780 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,201 & 0 & 0 & 0 & 0 & 110,201\\
		11,790 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,813 & 0 & 0 & 0 & 0 & 109,813\\
		11,800 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,571 & 0 & 0 & 0 & 0 & 109,571\\
		11,810 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,327 & 0 & 0 & 0 & 0 & 109,327\\
		11,820 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,322 & 0 & 0 & 0 & 0 & 109,322\\
		11,830 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 133,543 & 0 & 0 & 0 & 0 & 133,543\\
		11,840 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 125,707 & 0 & 0 & 0 & 0 & 125,707\\
		11,850 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 123,019 & 0 & 0 & 0 & 0 & 123,019\\
		11,860 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 119,828 & 0 & 0 & 0 & 0 & 119,828\\
		11,870 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 117,920 & 0 & 0 & 0 & 0 & 117,920\\
		11,880 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 116,774 & 0 & 0 & 0 & 0 & 116,774\\
		11,890 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 116,069 & 0 & 0 & 0 & 0 & 116,069\\
		11,900 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 115,275 & 0 & 0 & 0 & 0 & 115,275\\
		11,910 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 114,391 & 0 & 0 & 0 & 0 & 114,391\\
		11,920 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,956 & 0 & 0 & 0 & 0 & 113,956\\
		11,930 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,820 & 0 & 0 & 0 & 0 & 113,820\\
		11,940 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,511 & 0 & 0 & 0 & 0 & 113,511\\
		11,950 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,402 & 0 & 0 & 0 & 0 & 113,402\\
		11,960 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,017 & 0 & 0 & 0 & 0 & 113,017\\
		11,970 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,733 & 0 & 0 & 0 & 0 & 112,733\\
		11,980 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,205 & 0 & 0 & 0 & 0 & 113,205\\
		11,990 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,901 & 0 & 0 & 0 & 0 & 112,901\\
		12,000 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,649 & 0 & 0 & 0 & 0 & 112,649\\
		12,010 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,371 & 0 & 0 & 0 & 0 & 112,371\\
		12,020 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,246 & 0 & 0 & 0 & 0 & 112,246\\
		12,030 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,970 & 0 & 0 & 0 & 0 & 111,970\\
		12,040 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,612 & 0 & 0 & 0 & 0 & 111,612\\
		12,050 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,256 & 0 & 0 & 0 & 0 & 110,256\\
		12,060 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,650 & 0 & 0 & 0 & 0 & 109,650\\
		12,070 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,648 & 0 & 0 & 0 & 0 & 109,648\\
		12,080 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,327 & 0 & 0 & 0 & 0 & 109,327\\
		12,090 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 152,682 & 0 & 0 & 0 & 0 & 152,682\\
		12,100 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,552 & 0 & 0 & 0 & 0 & 109,552\\
		12,110 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,327 & 0 & 0 & 0 & 0 & 109,327\\
		12,120 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 152,708 & 0 & 0 & 0 & 0 & 152,708\\
		12,130 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 130,840 & 0 & 0 & 0 & 0 & 130,840\\
		12,140 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 125,501 & 0 & 0 & 0 & 0 & 125,501\\
		12,150 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 119,977 & 0 & 0 & 0 & 0 & 119,977\\
		12,160 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 116,707 & 0 & 0 & 0 & 0 & 116,707\\
		12,170 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 115,835 & 0 & 0 & 0 & 0 & 115,835\\
		12,180 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 114,325 & 0 & 0 & 0 & 0 & 114,325\\
		12,190 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,813 & 0 & 0 & 0 & 0 & 113,813\\
		12,200 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,402 & 0 & 0 & 0 & 0 & 113,402\\
		12,210 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,893 & 0 & 0 & 0 & 0 & 112,893\\
		12,220 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,633 & 0 & 0 & 0 & 0 & 112,633\\
		12,230 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,342 & 0 & 0 & 0 & 0 & 112,342\\
		12,240 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,137 & 0 & 0 & 0 & 0 & 112,137\\
		12,250 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,216 & 0 & 0 & 0 & 0 & 110,216\\
		12,260 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,624 & 0 & 0 & 0 & 0 & 109,624\\
		12,270 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 152,787 & 0 & 0 & 0 & 0 & 152,787\\
		12,280 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 126,967 & 0 & 0 & 0 & 0 & 126,967\\
		12,290 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 122,051 & 0 & 0 & 0 & 0 & 122,051\\
		12,300 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 119,460 & 0 & 0 & 0 & 0 & 119,460\\
		12,310 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 117,706 & 0 & 0 & 0 & 0 & 117,706\\
		12,320 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 116,447 & 0 & 0 & 0 & 0 & 116,447\\
		12,330 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 116,117 & 0 & 0 & 0 & 0 & 116,117\\
		12,340 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 115,545 & 0 & 0 & 0 & 0 & 115,545\\
		12,350 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 114,375 & 0 & 0 & 0 & 0 & 114,375\\
		12,360 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,570 & 0 & 0 & 0 & 0 & 113,570\\
		12,370 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,336 & 0 & 0 & 0 & 0 & 113,336\\
		12,380 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,708 & 0 & 0 & 0 & 0 & 112,708\\
		12,390 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 112,342 & 0 & 0 & 0 & 0 & 112,342\\
		12,400 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 111,839 & 0 & 0 & 0 & 0 & 111,839\\
		12,410 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 110,221 & 0 & 0 & 0 & 0 & 110,221\\
		12,420 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109,742 & 0 & 0 & 0 & 0 & 109,742\\
		12,430 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 135,416 & 0 & 0 & 0 & 0 & 135,416\\
		12,440 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 123,291 & 0 & 0 & 0 & 0 & 123,291\\
		12,450 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 118,687 & 0 & 0 & 0 & 0 & 118,687\\
		12,460 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 116,429 & 0 & 0 & 0 & 0 & 116,429\\
		12,470 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 115,698 & 0 & 0 & 0 & 0 & 115,698\\
		12,480 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 114,412 & 0 & 0 & 0 & 0 & 114,412\\
		12,490 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,956 & 0 & 0 & 0 & 0 & 113,956\\
		12,500 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,511 & 0 & 0 & 0 & 0 & 113,511\\
		12,510 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 113,377 & 0 & 0 & 0 & 0 & 113,377\\
		12,520 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\
		\hline
	\end{longtable}
\end{center}

==> eci_limited_cs.tex <==
\begin{figure}[!h]
	\centering
	\includegraphics[scale=0.25]{Figures/Size_allocation_stacked/URD_stacked_size_first_2000min_sum_edited.pdf}
	\vspace{-1em}
	\caption{Cache allocation for the VMs by ECI-Cache with limited SSD cache space.}
	\vspace{-1.5em}
	\label{fig:eci_limited_cs}
\end{figure}

==> eci_text.tex <==
%***********************************************************INTRODUCTION**********************************************************%
\vspace{-0.25em}
\section{Introduction}
\vspace{-0.25em}
\label{sec:introduction}
\sloppy
Virtualization is widely used in data centers and Cloud computing in order to improve the utilization of high-performance servers {\cite{virtualization}}.
%Virtualization is widely used in data centers and Clouds in order to improve the utilization of high-performance servers \cite{virtualization}. 
Integrating various \emph{Virtual Machines} (VMs) running with different operating systems on a server provides more flexibility and higher resource utilization while delivering the desired performance for each VM. In addition, virtualization provides system isolation where each VM has access only to its own resources. In a virtualized platform, shown in Fig. \ref{fig:vir}, the resource allocation of each VM is managed by a hypervisor. By employing various modules such as a VM scheduler and a memory and network manager, the hypervisor orchestrates the sharing of resources between VMs according to their demand, in order to maximize the overall performance provided by the server (and this maximizes performance-per-cost by enforcing the use of a smaller number of servers than one for each VM) \cite{uhlig2005intel,tickoo2010modeling}.

\begin{figure}
	\centering
	\includegraphics[scale=0.65]{Figures/virt_plat_2_3.pdf}
	\vspace{-1.5em}
	\caption{Example state-of-the-art virtualization platform.}
	\vspace{-1.5em}
	\label{fig:vir}
\end{figure}
\sloppy
With increasing performance requirements of data-intensive applications in data centers, storage subsystems have become performance bottlenecks of computing systems. \emph{Hard Disk Drives} (HDDs), which are used as main media for data storage in storage systems, provide large capacity and low cost, but they suffer from low performance, particularly for random access workloads. The low performance of HDD-based storage systems can be avoided by employing high-performance storage devices such as \emph{Solid-State Drives} (SSDs). Compared to HDDs, SSDs provide higher performance due to their non-mechanical structure used to retrieve and store data. SSDs, however, impose up to 10X higher cost and support only a limited number of reliable writes \cite{cai2017error}, which makes the replacement of all HDDs by SSDs usually prohibitively expensive \cite{migratetossd,agrawal2008design,salkhordeh2015operating}. 

\sloppy
In order to take advantage of the merits of both HDDs and SSDs, several studies from EMC$^2$, Facebook, FusionIO, Mercury, and VMWare \cite{migratetossd,matthews2008intel,appuswamy2012integrating,kim2011hybridstore,nitro,azor,hystor,flashcache,mercury,fusionio,vfrm,emcvfcache} employ high-performance SSDs as a caching layer for high-capacity HDDs in storage systems (as shown in Fig. \ref{fig:vir}). 
Applying such I/O caching on virtualization platforms requires a proper cache management scheme in order to achieve higher I/O performance.
In previous studies, such caches have been used as either a shared global cache \cite{emcvfcache, fusionio, vfrm} or a cache statically partitioned across VMs \cite{mercury}. 
The former scheme fails to provide a guaranteed minimum cache space for each VM. This is due to the fact that the entire cache is shared between all VMs and each VM can potentially use up an unbounded amount of the entire cache space, affecting the performance of the other VMs. The latter scheme \emph{statically} partitions SSD space between VMs where the partitioning is performed \emph{independently of} the characteristics of the workloads running on VMs. This scheme has two major shortcomings. First, the allocated cache space could be underutilized by the VM if there is low locality of reference in the workload access pattern. Second, since cache space partitioning and allocating is done statically offline, cache allocation for a new VM during runtime is \emph{not} practical using this scheme, which makes the scheme inflexible and the system underutilized. To alleviate the shortcomings of two afore-mentioned schemes, \emph{partitioned I/O caching} has been proposed. Variants of this technique dynamically estimate and allocate cache space for each VM by estimating an efficient cache size for each VM \cite{scave, vcacheshare,centaur}. 
They do so by calculating the reuse distance of the workload, i.e., the maximum distance between two accesses to an identical address \cite{parda,shards,centaur} .
%Such I/O caching schemes, however, mainly focus on cache space partitioning and estimating the required cache size for each VM. 
Unfortunately, such I/O caching schemes only focus on estimating cache size for VMs and neglect other key parameters, such as \emph{write policy} (i.e., how write requests are handled by the cache), \emph{request type} (i.e., read or write requests), and their corresponding impact on the workload \emph{reuse distance}, 
which greatly hinders the performance-per-cost and endurance  of the SSD cache, as we show in this work. 

%by assigning a single global write policy for all VMs, which affects cache performance and also SSDs lifetime as we show in this work. 

%In this paper, we propose \techname{}, a hypervisor-based high-\uline{E}ndurance and \uline{C}ost-efficient dynamic \uline{I}/O caching scheme for virtualized platforms. 
In this paper, we propose \emph{a high-\uline{E}ndurance and \uline{C}ost-efficient \uline{I}/O caching} (\techname{}) scheme which can be used for virtualized platforms in large-scale data centers.  
\techname{} aims to improve both the performance-per-cost and endurance of the SSD cache by dynamically configuring 1) an efficient cache size to maximize the performance of the VMs and 2) an effective write policy improving endurance and performance-per-cost for each VM.
To this end, we propose a metric called  \emph{Useful Reuse Distance} (URD), which minimizes the cache space to allocate for each VM while maintaining the performance of the VM.
The main objective of URD is to reduce the allocated cache space for each VM. The reduced cache space is obtained by computing workloads reuse distance based on request type without considering unnecessary writes accesses (i.e., writes without any further read access).
Employing URD in our proposed I/O caching scheme maximizes the performance-per-cost and also enhances the endurance of the SSD cache by allocating much smaller cache space compared to state-of-the-art cache partitioning schemes. 
We also propose a detailed analysis of the effect of write policy on the performance and endurance of SSD cache, clearly demonstrating the negative impact of having the same write policy for all VMs with different access patterns (as used in previous studies) on the IO performance and SSD endurance. 
%To achieve a significantly higher hit ratio and much smaller number of writes in SSD, \techname{} partitions the cache across VMs and assigns an efficient write policy for each VM by online monitoring and analysis of IO requests for each VM.
To achieve a sufficiently high hit ratio, \techname{} dynamically partitions the cache across VMs.

In the proposed scheme, we mainly focus on two approaches: 1) URD based per-VM cache size estimation and 2) per-VM effective write policy assignment by online monitoring and analysis of IO requests for each VM.
In the first approach, we allocate much smaller cache space compared to previous studies for each VM which results in improved performance-per-cost and in the second approach, we assign an effective write policy for each VM in order to improve the endurance of the I/O cache while minimizing negative impact on performance. The integration of these two approaches enables ECI-Cache to partition and manage the SSD cache between VMs more effectively.

We have implemented \techname{} on QEMU (version 2.8.0) \cite{qemu}, an open source hypervisor  (on the CentOS 7 operating system, kernel version 3.10.0-327). We evaluate our scheme on an HP ProLiant DL380 Generation 5 (G5) server \cite{hp_g5} with four 146GB SAS 10K HP HDDs \cite{hp_hdd} (in RAID-5 configuration), a 128GB Samsung 850 Pro SSD \cite{samsung_ssd}, 16GB DDR2 memory, and 8 x 1.6GHz Intel(R) Xeon CPUs. We run more than fifteen workloads from the SNIA MSR traces \cite{msr} on VMs.
Experimental results show that \techname{} 1) improves performance-per-cost by 30\% compared to the state-of-the-art cache partitioning scheme \cite{centaur}, 2) reduces the number of writes committed to the SSD by 65\% compared to \cite{centaur}, thereby greatly preserving the SSD lifetime. 

To our knowledge, we make the following contributions.
\begin{itemize}
			%\setlength\itemsep{-0.5em}
	
	\item This paper is the first to differentiate the concept of reuse distance based on the \emph{type of each request}. We propose a new metric, \emph{Useful Reuse Distance} (URD), whose goal is to reduce the cost of the SSD cache with allocating smaller cache size.
	
	\item By conducting extensive workload analyses, we demonstrate the importance of dynamically adjusting the cache \emph{write policy} on a per-VM basis which no previous I/O caching policy explicitly takes into account.
	We use these analyses to develop a mechanism that can efficiently adjust both cache size and write policy on a per-VM basis.
	%This analysis is used as a basis to find an effective cache configuration equipped with an efficient cache size and write policy for each VM. 
	
	\item We propose \techname{} which consists of two key novel components: 1) dynamic per-VM cache size estimation using the URD metric and cache partitioning and 2) per-VM write policy to improve both system performance-per-cost and SSD cache lifetime.

	\item We implement \techname{} in QEMU, an open source hypervisor. Our extensive evaluations of \techname{} on a large number of diverse workloads shows that \techname{}  significantly improves performance-per-cost over the best previous dynamic cache partitioning policy and reduces the number of writes to the SSD.
	
%	\item We will release \techname{} as an open-source framework which can be used in future research studies.
	%\item We develop an open-source framework, which will be publicly available to the community for future works.
\end{itemize}
\vspace{-1.1mm}
%The rest of the paper is organized as follows. Sec. \ref{sec:related} discusses related work. In Sec. \ref{sec:example}, we provide an illustrative example and motivation. In Sec. \ref{sec:URD}, we propose the metric of URD. In Sec. \ref{sec:arch}, we present our proposed technique. Sec. \ref{sec:results} provides experimental setup and results. Finally, Sec. \ref{sec:conclusion} concludes the paper.

%***********************************************************RELATED**********************************************************%
 \vspace{-2mm} 
\section{Related Work}
 \vspace{-1.1mm}
\label{sec:related}

%Previous studies on I/O caching in virtualization platforms can be investigated from two perspectives: one is based on where the I/O caching resides and the other is based on the cache partitioning techniques across VMs. The former classifies caching techniques based on the location of cache, while the latter focuses on the effective cache sharing and partitioning mechanisms. Based on the location of SSD cache, three main alternatives for I/O caching in virtualization platforms can be introduced as presented in Fig. \ref{fig:alternatives_caching}. In the following, we will describe the scheme of each alternative and present their pros and cons.
Previous studies on I/O caching in virtualization platforms investigate 1) the location of cache or 2) the cache partitioning policy. The former set of works explores caching techniques based on where the I/O cache resides, whereas the latter examines mechanisms for sharing and partitioning of the cache across VMs. Based on the location of the SSD cache, three main alternatives for I/O caching in virtualization platforms have been introduced as shown in Fig. \ref{fig:alternatives_caching}. 
%The location of SSD cache demonstrates whether the cache partitioning across VMs is viable or not. 
We next describe possible schemes for I/O caching and discuss their advantages and shortcomings.
 \vspace{-2mm}
\subsection{VM-based I/O Caching}
\vspace{-1mm}
In \emph{VM-based I/O caching} (Fig. \ref{fig:vmbased}), each VM in a virtualized platform has full control on a portion of the SSD cache. In this scheme, separate SSD slots are allocated for each VM and the cache management is conducted by VMs. 
%Using this scheme, VMs have best knowledge and full control of cache and provide isolation between caches of different VMs. On the other hand, by applying \emph{VM-based I/O caching} in a virtualization platform, creation and also modification of the cache is done by the guest VM. In addition, 
Cache size adjustment, cache partitioning, and sharing techniques could not be applied in this scheme. In order to employ \emph{VM-based I/O caching} scheme in a virtualized platform, caching schemes presented in \cite{migratetossd,nitro,hystor} can be applied on VMs and improve the IO performance of individual VMs where it could not be efficient in virtualized platforms.
\vspace{-2mm}
\subsection{Storage system-based I/O Caching}
\vspace{-1mm}
In \emph{Storage system-based I/O caching} (Fig. \ref{fig:storagebased}), VMs and the hypervisor have no knowledge of the SSD cache which
% is employed in storage systems. Performance management in a virtualization platform cannot be guaranteed in such scheme, since the cache is not transparent for VMs and hyprevisor. It is obvious that employment of cache partitioning and sharing techniques across VMs in such schemes would not be possible. 
prohibits advantages achieved by cache partitioning schemes.
Similar to \emph{VM-based I/O caching}, previous caching techniques such as \cite{migratetossd,nitro,hystor} can be employed in storage systems, but such techniques could not be managed in a virtualized platform.
\vspace{-2mm}
\subsection{Hypervisor-based I/O Caching}
\vspace{-1mm}
In \emph{Hypervisor-based I/O caching} (Fig. \ref{fig:hypervisorbased}), cache management is done by the hypervisor. Since the hypervisor has full knowledge about workloads running on VMs, it can perform efficient cache management and cache space partitioning across VMs. This type of I/O caching schemes have been proposed frequently in previous studies \cite{scave,vcacheshare,centaur}. These works mainly focus on the cache management, sharing, and partitioning across VMs. From the partitioning perspective, \emph{Hypervisor-based I/O caching} schmes can be divided into two groups namely: global/static and dynamic cache partitioning. We next describe state-of-the-art \emph{hypervisor-based I/O caching} schemes. 
\input{caching_alternatives}
%%\techname{} that we propose in this work is a hypervisor-based I/O caching scheme which takes advantage from options of hypervisor to provide the most efficient SSD cache for virtualization platforms.

\subsubsection{Global Caching and Static Cache Partitioning}
%Previously global I/O caching and also static cache partitioning schemes such as EMC VFCache \cite{emcvfcache}, NetApp Mercury \cite{mercury}, Fusion ioTurbine \cite{fusionio} and vFRM \cite{vfrm} have been proposed but recent experiments indicate that such schemes result in equal and fix cache size for each VM that can not maximize the overall performance.
Examples of global caching or static cache partitioning schemes include the EMC VFCache \cite{emcvfcache}, NetApp Mercury \cite{mercury}, Fusion-io ioTurbine \cite{fusionio}, and vFRM \cite{vfrm}. In the global caching, each VM can use up the entire SSD cache, thereby potentially adversely affecting the performance of the other VMs \cite{scave}. 
%Hence, this scheme fails in cache space management for VMs and cannot maximize the overall performance. 
In static cache partitioning, SSD cache space is \emph{equally} partitioned across VMs based on the number of VMs in the platform, without
% considering workloads running on VMs. Such scheme cannot fully utilize the cache slot allocated to the VMs with low IO operations which will affect the performance of VMs running IO intensive workloads. 
taking into account the data access and reuse patterns of each VM. Static cache partitioning is also unable to allocate cache space for newly-added VMs during online operation.
%In global caching scheme one VM can occupy whole space of the SSD cache and also static cache partitioning assigns equal and fix cache size for each VM. Also, static cache partitioning scheme is not able to assign cache space for a new VM which is added to the platform. In addition experimental resutls of recent studies such as \cite{vcacheshare} indicate that such schemes are not fair and could not maximize the overall performance.

\subsubsection{Dynamic Cache Partitioning}
Dynamic cache partitioning schemes alleviate the shortcoming of global and static cache partitioning \cite{cloudcache,scave,vcacheshare,centaur,argon,janus}.
These techniques partition the SSD cache across VMs based on the cache space demand of each VM, and they are aware of data access and reuse pattern of VMs.
Argon \cite{argon} presents a storage server that partitions memory cache across services based on their access patterns. This scheme allocates minimum cache space for each service to achieve a predefined fraction of hit ratio namely \emph{R-Value}. To estimate the required cache size for each service, Arogn employs online cache simulation mechanism and finds the fraction of accesses that are served by cache (namely I/O absorption ratio). 
Janus \cite{janus} partitions flash tier between workloads at the filesystem level. Janus maximizes the total read accesses served from flash tier by allocating required space for each workload. The required space is estimated based on the ratio of read operation of each workload.
S-CAVE \cite{scave} is a hypervisor-based online I/O caching scheme that allocates cache space for each VM by dynamically estimating the working set size of workloads running on VMs. To minimize the concern of data loss, S-CAVE uses \emph{Write-Through} (WT) policy in cache configuration.
vCacheShare \cite{vcacheshare} is another hypervisor-based I/O caching scheme that dynamically partitions SSD cache space across VMs. This scheme considers locality and reuse intensity (i.e., burstiness of cache hits) in order to estimate the required cache size for each VM.
vCacheShare reduces the number of writes in the SSD cache by using \emph{Write Around} policy where write operations are always directed to storage subsystem. Such scheme only shows improved performance in read operations while it has no performance improvement on write operations.
%vCacheShare only improves the performance of read operations by using write around policy, however, it reduces the number of writes on SSDs. 
Centaur \cite{centaur}, another online partitioning scheme for virtualized platforms, aims to maximize the IO performance for each VM as well as meeting QoS targets in the system. It employs \emph{Miss Ratio Curves} (MRCs) to estimate an efficient cache space allocation for each VM.
Centaur does \emph{not} consider the negative impact of write operations on SSD cache lifetime in cache size estimation, and neither in write policy assignment.
% Efficient cache size is predicted by measuring latency and miss ratio for each VM. 
Centaur employs the \emph{Write-Back} (WB) policy to maximize the IO performance without considering the impact of WB cache policy on the number of writes into the SSD.  
CloudCache \cite{cloudcache} estimates each VM's cache size by considering \emph{Reuse Working Set Size} (RWSS), which captures temporal locality and also reduces the number of writes into the SSD cache. In addition, this scheme employs a VM migration mechanism in order to handle the performance demands of VMs in the Cloud.

%\colorbox{SpringGreen!50}{
%	\parbox{0.92\columnwidth}{
{To summarize, among previous studies, S-CAVE {\cite{scave}}, vCacheShare {\cite{vcacheshare}}, Centaur {\cite{centaur}}, and CloudCache {\cite{cloudcache}} are the closest to our proposed. However, they only consider cache space partitioning and do not consider adaptive write policies. The cache size estimation scheme presented in S-CAVE, which is based on working set size estimation fails in cache size estimation for workloads with sequential access patterns and has become deprecated, as shown in {\cite{vcacheshare}}.
 vCacheShare and CloudCache perform cache size estimation based on reuse intensity. Such cache allocation schemes are based on assumptions that cannot be applied I/O cache in storage subsystem, as demonstrated in {\cite{centaur}}.
 Reuse intensity based schemes are \emph{only} effective for workloads that are aligned with their size estimation schemes and would not be accurate compared to reuse distance based schemes such as {\cite{centaur}}.
 The most state-of-the-art scheme is Centaur, which works based on MRCs and reuse distance analysis. This scheme has in common with ECI-Cache but 1) it neglects the impact of request type on reuse distance calculation and 2) it eliminates  the impact of other parameters such as write policy on endurance and also performance.}
%{To summarize, among previous studies, S-CAVE {\cite{scave}}, vCacheShare {\cite{vcacheshare}}, Centaur {\cite{centaur}}, and CloudCache {\cite{cloudcache}} are very close to ECI-Cache which only consider cache space partitioning. The cache size estimation scheme presented in S-CAVE, which is based on working set size estimation fails in cache size estimation for workloads with sequential access pattern. vCacheShare and CloudCache employ cache size estimation schemes based on reuse intensity which suffer from two problems: 1) these schemes keep a large amount of data in history tables which leads to significant memory overheads and 2) they are also not accurate enough compared to MRC based schemes.}
	
%{The last state-of-the-art scheme is Centaur which works based on MRCs. This scheme has in common with ECI-Cache but the impact of other parameters such as write policy and request type on performance and also endurance is neglected.}
%***********************************************************MOTIVATION**********************************************************%
\vspace{-2.5mm}
\section{Motivation and Illustrative Example}
\vspace{-1mm}
\label{sec:example}
%The main purpose of using SSD cache is to reduce the number of access to HDD in order to improve performance. 
The main purpose of employing a high performance cache layer is to reduce the number of accesses to the disk subsystem. Theoretically, an ideal SSD cache layer would provide access latency equal to the SSD access latency.
However, due to limited SSD size and imperfect write policy, the observed average latency of accesses sent to the SSD cache is much higher than the SSD latency.
For example, we find that the access latency of the caching technique presented in \cite{nitro} is $~$50X higher than the raw access latency of the employed SSD, as shown in Fig. \ref{fig:hdd-ssd-latency}.

\begin{figure}[!h]
	\centering
	\includegraphics[scale=0.3]{Figures/hdd-ssd-latency_edited.pdf}
		\vspace{-0.7em}
	\caption{HDD and SSD access latency vs. I/O caching\protect\footnotemark.}
		\vspace{-1em}
	\label{fig:hdd-ssd-latency}
\end{figure}

\footnotetext{\small{{All numbers in this figure are based on the results reported in \cite{nitro,hystor}.}}}

The major parameters affecting IO cache performance are cache size, write policy, and replacement policy.
%Hence, to achieve the higher performance, it is necessary to employ the efficient cache configuration. 
%Cache parameters such as size, write policy, and replacement policy can affect the performance of the cache. 
In this work, we mainly study the effect of cache size and write policy on the performance and endurance of an SSD cache. A commonly-used metric to compare the performance of different cache configurations is \emph{hit ratio}. To maximize the cache hit ratio, the cache size should be large enough to include the working set of running workload. Similar to size, write policy can also affect the performance of the cache particularly in write-intensive workloads. There are three major write policies that are fundamentally different: 1) \emph{Write-Back} (WB), 2) \emph{Write-Through} (WT), and 3) \emph{Read-Only} (RO).
WB reduces the number of accesses to the storage subsystem by buffering temporal writes in the SSD cache and writing them back to the storage subsystem only after the buffered dirty blocks are evicted. WB can improve the performance of both read and write operations, but it suffers from low reliability since the SSD cache can become a single point of failure (i.e., buffered writes can get lost before being propagated to the storage subsystem, if the SSD fails).
WT policy buffers write operations but also transfers them to the storage subsystem at the same time. This policy improves the performance of \emph{only} read operations but provides higher level of reliability by assuming that each written block is propagated immediately to the storage system. 
RO caches only the read operations and directs write operations completely to the storage subsystem without buffering them. Therefore, it is not able to improve the performance of write operations but it keeps them reliable. 
%Since a cache with RO policy does not keep write-pending operations, it has no negative effect on the reliability of write operations.
%remove space

%\afterpage{\global\setlength{\textfloatsep}{\oldtextfloatsep}}% Reset \textfloatsep
We conduct experiments to show the impact of cache size and cache write policy on IO performance and SSD endurance. To this end, we perform several experiments on a system with a 200GB HDD and 30GB SSD (our experimental setup is reported in Table \ref{table:mot_exp}). We employ EnhanceIO \cite{enhanceio} as an open source SSD caching scheme in the experiments.
\begin{table}[!h]
	%	\setlength{\textfloatsep}{0pt}% Remove \textfloatsep
	%	\begin{center}
	\centering
	\vspace{-0.5em}
	\caption{Setup of the motivational experiments.}\label{table:mot_exp}
	\vspace{-0.5em}
	\resizebox{0.45\textwidth}{!} {
		\begin{tabular}{ |l|l| }
			\hline
			\textbf{HW/SW} & \textbf{Description} \\\hline\hline
			Server & HP Proliant DL380 G5 \\  \hline
			CPU & 8x 1.6GHz Intel(R) Xeon \\  \hline
			Memory & 16 GB DDR2, Configured Clock Speed: 1600 MHz \\  \hline %, Manufacturer: Hynix Semiconductor  \\  \hline
			HDD &  438GB: four SAS 10K HP‌ HDDs in RAID5 (partition size = 200GB) \\  \hline
			SSD &  128GB Samsung 850 Pro (partition size = 30GB) \\  \hline\hline
			OS & Centos 7 (Kernel version: 3.10.0-327) \\ \hline
			Filesystem & {ext3 (Buffer cache is disabled)} \cite{tweedie2000ext3} \\ \hline
			
		\end{tabular}
	}
	%	\end{center}
\end{table}
To investigate the impact of write policy on performance and endurance, we run 30 workloads from Filebench on a fixed-size SSD cache with both the WB and RO policies. Here, our goal is to investigate the impact of write policy on the performance and endurance. We have omitted the results of WT policy, since WT has the same endurance as WB and provides less performance than WB.
 
Fig. \ref{fig:simple_exp_policy} shows the impact of write policy on both \emph{Bandwidth} (i.e., the amount of data that is transmitted for a workload in one second) and \emph{I/O Per Second (IOPS)} of eight sample workloads (Fig. \ref{fig:fileserver} through Fig. \ref{fig:singlestreamread}).
We make five major observations: 1) the SSD cache has 2.4X performance improvement with WB policy and \emph{Least Recently Used } (LRU) replacement policy in \emph{Fileserver} workload where the RO cache has only 1.6X improvement on the IO performance of this workload (Fig. \ref{fig:fileserver}). 2) WB policy improves the IO performance of \emph{RandomRW} and \emph{Varmail} workloads (Fig. \ref{fig:randomrw} and Fig. \ref{fig:varmail}).
3) \emph{Webserver} and \emph{Webproxy} workloads can be satisfied with both WB and RO write policies (Fig. \ref{fig:webserver} and Fig. \ref{fig:webproxy}). 4) Employing cache  has negative impact on the performance in the \emph{CopyFiles} workload (Fig. \ref{fig:copyfiles}).
5) RO write policy can significantly improve the performance of \emph{Mongo} and \emph{SingleSteramRead} workloads by 20\% and 48\%, respectively (Fig. \ref{fig:mongo} and Fig. \ref{fig:singlestreamread}).

%We conduct additional experiments for \emph{RandomRead} and \emph{RandomWrite} access patterns from FIO \cite{fio} benchmark. We make two observations: 1: For a workload with random read access pattern, both WB and RO caches improve the IO performance by 1.2X. 2) only WB cache has significant improvement for the workload with random write access patterns.

Our main experimental conclusions are as follows: 
\begin{enumerate}
	\item In workloads such as \emph{Fileserver}, \emph{Varmail}, and \emph{SingleStreamRead}, only a specific cache configuration can improve IO performance.
	About 45\% of the workloads prefer the WB policy and about 33\% of workloads prefer the RO policy.
	Hence, it is necessary to employ a \emph{workload-aware write policy} for the IO cache. Random access and write-intensive workloads prefer WB while random accesses and read-intensive workloads can be satisfied with RO policy.
	
	\item In 20\% of workloads, e.g., \emph{Webserver} and \emph{Webproxy}, both WB and RO write policies result in similar improvements. Hence, we can employ RO instead of WB in order to reduce the number of writes in the SSD cache. Such workloads that are random and read-intensive do not take advantage of buffering writes in the SSD cache.
	
	\item In workloads such as \emph{Mongo} and \emph{CopyFiles}, the SSD cache provides little performance improvement. Hence, one can allocate SSD cache space to other workloads that can benefit more from the available cache space. We prevent to allocate cache space for the workloads that do not benefit from allocated cache, and hence reduce the number of unnecessary writes into the SSD cache. 
\end{enumerate}
\input {fig4}
%%%%%%%%%%%%%%%URD%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-2mm}
\section{Useful Reuse Distance}
\label{sec:URD}
\vspace{-1mm}
\emph{Traditional Reuse Distance} (TRD) schemes \cite{mattson, parda, shards,ding2003predicting,zhong2009program,fang2004reuse,ding2001reuse,berg2004statcache,shen2007locality} work based on the addresses of requests \emph{without} considering type of the requests. We provide examples demonstrating the impact of considering \emph{request type} of the workloads in calculation of reuse distance. The main objective of this analysis is to present the metric of \emph{Useful Reuse Distance} (URD), which enables assigning smaller cache space to the VMs while preserving I/O performance. 
%The smaller cache size also reduces the number of unnecessary writes into the SSD cache, which enhances the cache lifetime.

We examine a sample workload (shown in Fig. \ref{fig:example_rd}) and show how reuse distance analysis assigns cache size for the workload in two cases: 1) without considering request type (TRD) and 2) considering request type (URD).
%ta inja (95-10-13)
In the sample workload given in Fig. \ref{fig:trad_rd_1}, the maximum reuse distance is due to the access of $Req_7$ to the second sector where it was previously (five requests before) accessed by $Req_2$. Hence, the maximum TRD of the workload is equal to 4, and according to TRD, we should assign cache space equal to 5 blocks in order to maximize the hit ratio of this workload.
Fig. \ref{fig:trad_rd_1} also shows the contents of the allocated cache to this workload based on TRD. 
It can be seen that when we allocate cache space based on TRD, we reserve one block of cache (the second block) to keep a data that will be written (modified) by the next request ($Req_7$) without any read access to this block.
%It can be seen that such scheme allocates one block for caching the data of a sector (the second sector) which will be written (modified) by the next request without  ($Req_7$).
\begin{figure}[!htb]
	\centering
	\subfloat[]{\includegraphics[width=.2\textwidth]{Figures/TRD_example_2.pdf}%
		\label{fig:trad_rd_1}}
	\hfil
	\subfloat[]{\includegraphics[width=.2\textwidth]{Figures/URD_example_2.pdf}%
		\label{fig:enh_rd_1}}
	
		\vspace{-1em}
		\caption{Comparison of cache size allocation (a) without  and (b) with considering request type (REQ: Request, TYP: Type, SEC: Sector, W: Write, R: Read, and CB: Cache Block).}
			\vspace{-0.5em}
		\label{fig:example_rd}
\end{figure}

Here we classify sequence of accesses in four groups based on their type (illustrated in Fig. \ref{fig:io_class}): 1) \emph{Read After Read} (RAR), 2) \emph{Write After Read} (WAR), 3) \emph{Read After Write} (RAW), and 4) \emph{Write After Write} (WAW). We show how data blocks of such accesses are stored {in both WB and WT caches (i.e., allocate on write)}.
Fig. \ref{fig:read_write_hit_miss} shows the operation of cache for both read and write requests \cite{netappflexcache}. The operation of cache is defined in two cases: 1) for read accesses, if the data is found in the cache we read data from cache. Otherwise, the data is read from disk subsystem and is stored in the cache for further accesses. 2) Write operations are directly written to the cache that may modify the previously written data in the cache.
We define cache hit only for read requests.

\begin{figure}[!t]
	\centering
	\includegraphics[scale=0.8]{Figures/io_class_2.pdf}
	\vspace{-1em}
	\caption{I/O access sequences.}
	\vspace{-1em}
	\label{fig:io_class}
\end{figure}

\begin{enumerate}
		%	\setlength\itemsep{-0.5em}
	\item RAR: In the first read access, a cache miss fetches data from HDD to the cache. The second access reads the data from the cache. In this case, caching data block of the first access improves the hit ratio at the cost of imposing one write access to the SSD.
	\item WAR: The first read access leads to fetching the data from HDD to the cache. The second access modifies the data in the cache without any read access to this block. In this case, caching the data block of the first read access does not improve the hit ratio but it comes at the cost of two writes into the SSD.
	\item RAW: The first access writes the data to the cache. The second access reads the data from the cache. In this case, caching the data block of the first access increases the hit ratio of the cache at the cost of imposing one write access into the SSD.
	\item WAW: The first access writes data to the cache. The second access modifies the data without any read access. In this case, caching the data block of the first access does not improve the hit ratio but comes at the cost of two writes to the cache.

%	Such operations impose two write accesses on the cache while it does not have any impact on the hit ratio.
\end{enumerate}

\begin{figure}[!htb]
	\centering
	\subfloat[]{\includegraphics[width=.22\textwidth]{Figures/read_hit_miss.pdf}%
		\label{fig:read_hit_miss}}
	\hfil
	\subfloat[]{\includegraphics[width=.22\textwidth]{Figures/write_hit_miss.pdf}%
		\label{fig:write_hit_miss}}
	
	\vspace{-1em}
	\caption{Flowchart of I/O cache for (a) Read (b) Write.}
	\vspace{-0.5em}
	\label{fig:read_write_hit_miss}
\end{figure}

We now show how we can allocate smaller cache size to the sample workload (shown in Fig. \ref{fig:enh_rd_1}) by distinguishing between the four different types of access patterns we just described. We call this scheme \emph{Useful Reuse Distance} (URD) as it takes into account the request type in calculating the reuse distance of the workload. URD only considers accesses to the \emph{referenced} data. It eliminates WAW and WAR access patterns from the reuse distance calculation.
{It considers only the maximum $reuse~distance$ of RAR and RAW access patterns in reuse distance calculation.}
The maximum URD of the sample workload (Fig. \ref{fig:enh_rd_1}) is equal to 1, due to read access of $Req_3$ to the first sector of disk where it was previously (two request before) written by $Req_1$. In this case, we assign cache size equal to only two blocks. Fig. \ref{fig:enh_rd_1} shows the contents of the allocated cache space based on URD for the sample workload. 
It can be seen that by employing the concept of URD, we achieve hit ratio similar to the TRD scheme while reducing the allocated cache size.
%In addition, URD helps the caching schemes to prevent caching unreferenced data which will reduce the number of unnecessary writes into the SSD‌ cache.

{To summarize, in order to show how URD is able to allocate smaller cache space compared to TRD and achieve similar hit ratio, we classify the workloads into two groups:}
	\begin{enumerate}
		%\setlength\itemsep{-0.5em}
		\item {Workloads where RAR and RAW (RA*) accesses are involved in the maximum reuse distance calculation.}
		\item {Workloads where WAR and WAW (WA*) accesses are involved in the maximum reuse distance calculation.}
	\end{enumerate}
{These workloads are characterized with the following two equations, respectively.
\begin{equation} 
\begin{cases}
\scriptsize
1: RD\text{\protect\footnotemark}(WA*) \leq  RD(RA*) \to TRD \propto RD(RA*),\\ 
~~~~URD \propto RD(RA*) \to TRD = URD  \\ 
2: RD(WA*) >  RD(RA*) \to TRD \propto RD(WA*),\\ 
~~~~URD \propto RD(RA*) \to TRD > URD
\end{cases}
\label{equ:conditions_RD}
\end{equation}
}
\footnotetext{\small{{RD: Reuse Distance.}}}
	{In the workloads of the first group (Eq. {\ref{equ:conditions_RD}}: part1), both TRD and URD work similarly in cache size estimation. On the other hand, in the workloads of the second group  (Eq. {\ref{equ:conditions_RD}}: part2), the URD of the workload is smaller than TRD and hence URD allocates smaller cache size compared to TRD. This is because URD considers only the RA* accesses. The maximum reuse distance of RA* requests is smaller than the maximum reuse distance of WA* accesses for the workloads in the second group and hence URD provides smaller maximum reuse distance and leads to allocating smaller cache space. In this case, URD achieves similar hit ratio while allocating \emph{smaller} cache space compared to TRD.} %This is because such scheme does not evict the cache block that would be referenced in future (data related to RA* accesses).}
	%***********************************************************PROPOSED**********************************************************%
\vspace{-2mm}
\section{\techname{} Architecture}
\label{sec:arch}
\vspace{-1mm}
%We performed various experiments to determine the parameters affecting the performance of the cache in Sec. \ref{sec:example}. The results revealed the significant impact of write policy as well as cache size on the performance improvement of workloads. 
In this section, we describe the architecture of  the \techname{}. \techname{} 1) collects and analyzes the access patterns of the VMs and 2) allocates an efficient and effective size and write policy to each VM. Fig. \ref{fig:\techname{}} provides an overview of the \techname{} architecture in the hypervisor of a virtualization platform. As shown in this figure, \techname{} consists of three major components: (1) \emph{Monitor}, (2) \emph{Analyzer}, and (3) \emph{Actuator}. \techname{} resides in the path of IO requests coming from VMs to the storage subsystem. \emph{Monitor} captures and collects information about IO behavior of each VM. \emph{Analyzer} decides the cache size and write policy by characterizing the IO behavior of the corresponding VM. Finally, \emph{Actuator} realizes the decisions made by \emph{Analyzer} by allocating an efficient and effective cache space and write policy for each VM in the SSD cache. We describe each component in more details:
%As shown in this figure, \techname{} module resides in the path of IO requests coming from VMs to the storage subsystem where it can capture and monitor the IO behavior of the VMs. Then \techname{} decides the cache size and write policy by characterizing the IO behavior of the corresponding VM. \techname{} consists of three major parts namely: (1) \emph{Monitor}, (2) \emph{Analyzer}, and (3) \emph{Actuator}. In the following, we elaborate each part in more details.

\begin{enumerate}
		%	\setlength\itemsep{-0.5em}
	\item{\emph{Monitor} receives all IO requests coming from VMs and extracts important information such as \emph{VM Identification Number} (\emph{VM-ID}), \emph{request type}, \emph{destination address}, and \emph{request size} by using \emph{blktrace} as a block layer IO tracing tool {\cite{blktrace}}. We modified the source code of \emph{blktrace} to extract the owner of each request (i.e., the VM that sends the request) at the hypervisor level. Such modification helps us to classify the requests and discover the access patterns of the running workloads in different VMs. The extracted information is passed to \emph{Analyzer}}.
	\item\emph{Analyzer} decides 1) the target destination of a given IO request, 2) an efficient cache size for each VM, and the write policy of the I/O cache for each VM, based on 1) the information it receives from \emph{Monitor} and 2) a database it employs, called \emph{VM Info}. \emph{Analyzer} keeps information about each VM, such as cache size, write policy, workload characteristics, and the number of VMs running in the system in the \emph{VM Info} database.
	\item\emph{Actuator} is responsible for realizing the decisions made by \emph{Analyzer}. It allocates the estimated cache space for each VM, configures the decided write policy, and also routes the IO requests to SSD cache or storage subsystem.
	\emph{Actuator} keeps logs for blocks stored in either the SSD cache or the storage subsystem which is used for responding to future requests in a table (namely \emph{Map Table}).
\end{enumerate}
\begin{figure}[!t]
	\centering
	\includegraphics[scale=0.7]{Figures/EHPCache_detailed.pdf}
		\vspace{-1em}
	\caption{Architecture of \techname{}.}
		\vspace{-1em}
	\label{fig:\techname{}}
\end{figure}
%\techname{} extends I/O caching scheme to a virtualized platform by considering given constraints.
Typically in a virtualization platform, there are several VMs running various workloads with different IO behavior. The hypervisor is responsible for partitioning the cache space efficiently between VMs.
In the workloads with sequential access pattern, there is no locality of references and hence buffering data demonstrates very poor hit ratio (Fig. \ref{fig:seq_pattern}). 
In the workloads with random access pattern, the probability of referencing to the blocks that are accessed previously is significantly greater than workloads with sequential access pattern and hence buffering data with random access pattern improves the hit ratio (Fig. \ref{fig:rand_pattern}).
Hence, in the proposed architecture, cache space will be allocated to only VMs with random read or write access pattern. Sec. \ref{sec:size_estimation} describes our proposed algorithm for cache space partitioning across VMs by online characterization of the workloads. Sec \ref{sec:policy} describes the policy assignment in more detail. 

\begin{figure}[!t]
	\centering
	\subfloat[Sequential accesses.]{\includegraphics[width=.2\textwidth]{Figures/seq_pattern_2.pdf}%
		\label{fig:seq_pattern}}
	\hfil
	\subfloat[Random accesses.]{\includegraphics[width=.2\textwidth]{Figures/rand_pattern_2.pdf}%
		\label{fig:rand_pattern}}
		\vspace{-1em}
	\caption{Cache hits in sequential and random access patterns.}
		\vspace{-0.5em}
	\label{fig:hit_pattern}
\end{figure}


\vspace{-2mm}
\subsection{Efficient Cache Size Estimation}
\vspace{-1mm}
\label{sec:size_estimation}
We propose an \techname{} size allocation algorithm which aims to allocate an efficient cache size for each VM based on the reuse distances of the running workloads. Previously, in Sec. \ref{sec:URD}, we proposed the metric of URD and provided an example that showed the impact of considering request type on 1) the reuse distance of a workload and 2) the estimated cache size. We also demonstrated that employing URD instead of TRD‌ in cache size estimation preserves the performance of the workload while reducing the allocated cache size. Such a scheme allocates a much smaller cache space to the workloads and hence improves the performance-per-cost of each VM. It also reduces the number of unnecessary writes (due to WAW and WAR operations) into the SSD cache, thereby improving SSD lifetime. 

Periodically, \techname{} calculates the URD of the running workloads in VMs and then estimates an efficient cache size for each VM. {To provide the minimum latency for all VMs, we employ optimization algorithms that meet the conditions of Eq. \ref{equ:conditions}. In this equation, $c_i$ is the allocated cache space for each $VM_i$, $C$ is the total SSD cache space, $N$ is the number of running VMs, and $h_i(c_i)$ denotes the achieved hit ratio for the running workload on $VM_i$ when we allocate cache space equal to $c_i$. In addition, $T_{hdd}$ and $T_{ssd}$ indicate the average read/write access latency to HDD and SSD, respectively.}
{
\begin{equation} 
	\begin{cases}
		\sum_{i=1}^{N}c_{i} \leq C \\
		LatencyVM_i=h_i(c_i) \times T_{ssd} + (1-h_i(c_i)) \times T_{hdd} \\
		Minimize[\sum_{i=1}^{N}LatencyVM_{i}]
	\end{cases}
	\label{equ:conditions}
\end{equation}
}
According to Eq. \ref{equ:conditions}, \techname{} partitions the cache space in a way that aims to minimize the aggregate latency of all VMs.
%In addition, the proposed scheme takes advantage from the impact of hit ratio on cache size allocation which is employed in IO characterization. 
Since allocating cache space for workloads with sequential access patterns achieves very poor hit ratio, \techname{} allocates cache space for VMs with random access patterns that have a high degree of access locality. 
{ECI-Cache estimates the true amount of cache space for each VM based on URD. The total SSD cache space should be greater than or equal to the sum of the cache sizes of all N VMs. Hence, we have two cases for the allocated cache size: (1) the sum of estimated cache sizes for all VMs using URD is less than the total SSD cache space and (2) the sum of estimated cache sizes is greater than the total SSD cache space. In the first case (i.e., when the SSD cache space is \emph{not} limited), ECI-Cache would allocate the exact estimated cache space for each VM and thus maximize overall hit ratio. In the second case (i.e., when the SSD cache space is limited), since we have shortage of cache space, it is necessary to \emph{recalculate} the cache size for each VM in order to fit each VM into the existing cache space.}
\input{size_alg}
\input{hit_func_example}
{Algorithm \ref{alg:size} shows how \techname{} estimates and allocates cache space in a virtualized platform with $N$ VMs (Algorithm \ref{alg:size_detail} in the Appendix provides a more detailed version of Algorithm \ref{alg:size}). Initially, a previously defined minimum cache size ($c_{i_{min}}$) is allocated to each VM\footnote{\small{{In the experiments, $c_{i_{min}}$ is set to $1,000$ blocks.}}}. 
At specific time intervals ({$\Delta t$}), we separately extract the traces of the running workloads on the VMs (line {\ref{lst:line:sleep}} and line {\ref{lst:line:extract}}).
	The extracted IO traces are text files with the following information: (1) destination address, (2) request size, and (3) request type.} %inja bood tahesh!!

{In the next step, we use the collected traces to calculate the URD of the workloads using the {$calculateURD$} function (line {\ref{lst:line:get_urd}}). In {$calculateURDbasedSize$} function (line {\ref{lst:line:calc_urd_size}}), based on the calculated reuse distances, we find the required cache space for each VM that maximizes the hit ratio. We check the feasibility of the estimated cache sizes to see if the sum of estimated cache sizes ({$csum$} which is calculated in line {\ref{lst:line:csum}}) is less than total SSD cache capacity (line {\ref{lst:line:if1}}). When the condition in line {\ref{lst:line:if1}} is met and the sum of estimated cache spaces for all VMs is less than or equal to the total SSD‌ cache capacity, we call the cache space allocation {\say{$feasible$}}; otherwise (when the condition in line {\ref{lst:line:elseif1}} is met) we call the allocation {\say{$infeasible$}}. In case of in-feasibility (in line {\ref{lst:line:calc_eff_size}}), we need to recalculate cache space allocations such that SSD cache capacity is not exceeded. To do so, we run the {$calculateEffSize$} function that employs an optimized minimization algorithm ({\say{$fmincon$}}) {\cite{fmincon}} to find the most efficient cache spaces that minimizes the aggregate latency of all VMs under the constraint that the total allocated cache space is less than the SSD‌ cache capacity\footnote{\small{{To this end, we use {\say{$fmincon$}} function from MATLAB Optimization toolbox \cite{fmincon}.}}}.
	The input of the minimization algorithm is (1) the existing SSD‌ cache capacity, (2) the hit ratio function of each VM (will be described in Algorithm {\ref{alg:sample_hit_ratio}}) based on allocated cache space (H(c)) that has been extracted by analyzing the reuse distances of the workloads, and (3) the estimated sizes by the algorithm which cannot be fit into the existing SSD cache capacity. Finally, in line {\ref{lst:line:allocate}} we allocate efficient cache spaces for each VM.}

{Algorithm {\ref{alg:sample_hit_ratio}} shows the structure of a hit ratio function. This function is extracted from the output of $calculateURD$ function. Hit ratio function of each VM shows the hit ratio that can be achieved in case of assigning a specific cache space to that VM. Such specific cache spaces  are calculated based on the different reuse distances where the hit ratio (that achieved based on that cache space) are the ratio of corresponding reuse distances. 
	In each time interval, in case of infeasibility, we update the hit ratio function of each VM and feed it to the minimization algorithm. Minimization algorithm uses the hit ratio function of running VMs to minimize the sum of latency of all VMs which is calculated by Eq. {\ref{equ:conditions}}.}

	%Alg. \ref{alg:sample_hit_ratio} shows an example of hit ratio function for one workload which calculates the hit ratio of the workload for a given cache size. The data of this function is extracted from reuse distance calculation function\footnote{To this end we have modified the source code of PARDA \cite{parda} to calculated URD.}. 
%In lines \ref{lst:line:delay} and \ref{lst:line:get_erd}, after a period of time ($\Delta t$), we calculate the URD of the VMs workload. \uline{Then in line \ref{lst:line:calc_urd_based_size} we calculate cache size based on URD of each VM and in line \ref{lst:line:csum} we update $csum$ which shows the sum of estimated cache sizes for the VMs based on URD. In the rest of the algorithm we check the feasibility of the cache size estimation and minimize the overall latency of the system. 
%The total SSD cache space should be greater than or equal to sum of the cache sizes of all $N$ VMs. To this end, in line \ref{lst:line:if1} we check whether the sum of estimated cache sizes based on URD (namely $csum$) is less than total SSD cache space (namely $C$) or not. Hence, we have two cases for the allocated cache size: (1) the sum of estimated cache sizes by URD is less than the total SSD cache space (when the condition in line \ref{lst:line:if1} is met) and (2) the sum of estimated cache sizes by URD is greater than the total SSD cache space (when the condition in line \ref{lst:line:elseif1} is met). In the first case (i.e., when the SSD cache space is not limited), line \ref{lst:line:allocate_urd} allocates the estimated cache space based on the URD of each VM and maximizes overall hit ratio. Otherwise, in the second case (i.e., when the SSD cache space is limited), since we have shortage of cache space, line \ref{lst:line:ceff_recalc} recalculates the cache size for each VM in order to fit each VM into the existing cache space. The main objective of the $caclulateEffSize$ function in line \ref{lst:line:ceff_recalc} is to find the most appropriate cache sizes for the running VMs such that our system is able to meet the  conditions mentioned in Eq. \ref{equ:conditions}. $calculateEffSize$ function aims to minimize the sum of $LatencyVM_i$ for all running VMs in the system by using a simulated annealing algorithm. The input of this function is the sum of $LatencyVM_i$ with the above-mentioned constraints. Finally in line \ref{lst:line:eff_allocate}, the cache with efficient size $c_{i_{eff}}$ is allocated to each $VM_i$.}

%In Algorithm \ref{alg:size}, we used $\Delta t$ as the time interval in which \techname{} checks the status of the VMs and updates the information about them. In the proposed scheme, $\Delta t$ is not constant and is dependent on the number of requests for each VM. When the number of requests for a VM becomes a multiple of a defined value $threshold$ (eg. $threshold=500$), \techname{} starts to check the hit ratio and other status of the VM. This reduces the size of \emph{VMs Info} database and also performance overhead of \techname{}.



\vspace{-2mm}
\subsection{Write Policy Estimation}
\vspace{-1mm}
\label{sec:policy}
In order to allocate the most efficient write policy for each VM, \techname{} investigates access patterns and also request types of the running workloads on the VMs. We choose between RO and WB policies for each VM.
The key idea is to use the RO policy for VMs with unnecessary writes (i.e., write operations without any further read access) and the WB policy for VMs with referenced write operations (i.e., write operations with further read access).
%Assigning WB policy on a cache improves the performance of write operations and a significant improvement can be observed in write intensive applications with a high locality of accesses. On the other hand, assigning WB policy on all caches imposes a negative impact on the lifetime of the SSD by committing unnecessary writes into the SSD. 
To diminish the number of unnecessary writes, we assign RO policy on the caches of VMs with read-intensive access patterns (including RAR and RAW accesses). RO policy improves the performance of read operations and increases the lifetime of the SSD. In addition, such a scheme would be more reliable since it does not buffer writes on the cache.

{As mentioned previously in Sec. \ref{sec:arch}, \emph{Analyzer} is responsible for write policy assignment for each VM and it does so periodically (every $\Delta$t). {\emph{Analyzer}} checks the ratio of WAW and WAR operations (namely, $writeRatio$). If the $writeRatio$ of the running workload exceeds a defined threshold, we change the write policy to RO, to prevent keeping such a large number of written blocks in the cache. This is due to two reasons: 1) such a workload includes a large amount of writes and holding such writes in the SSD cache would likely not have a positive impact on the hit ratio, 2) caching such a  large amount of writes has a negative impact on the endurance of the SSD. We select the WB cache policy when the running workload on a VM includes large percentage of \emph{RAW} accesses. In addition, we assign RO policy to the caches with larger percentage of \emph{WAW} and \emph{WAR} accesses.}

Algorithm \ref{alg:policy} shows how \techname{} assigns an efficient write policy for each VM's cache space. Initially, we assign the WB policy for a VM's cache space. Then, periodically, we analyze the behavior of the running workload and re-calculate the write policy. 
In line \ref{lst:line:delay_2} of Algorithm \ref{alg:policy}, {after a period of time ($\Delta t$), we calculate the ratio of WAW and WAR requests ($writeRatio$) for $VM_i$} (line \ref{lst:line:readratio}). In line \ref{lst:line:pol_if}, we check whether the ratio of WAW‌ and WAR requests is greater than a threshold (namely $wThreshold$) or not. If the ratio of such requests is greater than $wThreshold$, we assign the RO policy for $VM_i$ (in line \ref{lst:line:set_eff}); otherwise the policy remains as WB.

\begin{algorithm}[!htb]
	%\SetAlgoNoLine
	\scriptsize
	\DontPrintSemicolon
	\caption{\techname{} write policy assignment algorithm.}
	\label{alg:policy}
	%\begin{latin}
		\tcc{\textbf{Inputs:} Number of VMs: ($N$)}
		\tcc{\textbf{Output:} Efficient cache policy for each VM: ($P_{i_{eff}}$)}
%	// \textbf{Inputs:} Number of VMs: ($N$)\;
%	// \textbf{Output:} Efficient cache policy for each VM: ($P_{i_{eff}}$)\;
   $set(P_{i_{eff}}, VM_i) = WB$ \label{lst:line:set_wb_init} \tcc{Initialization}
	\For {$i = 1$ to $N$}
	{
		Sleep for $\Delta t$\; \label{lst:line:delay_2}
		$writeRatio = {{getNumOfWAW(VM_i)+getNumOfWAR(VM_i)} \over getNumOfReq(VM_i)}$ \label{lst:line:readratio}\;
		\If{$writeRatio \geq wThreshold$}
		{\label{lst:line:pol_if}
			$set(P_{i_{eff}}, VM_i) = RO$ \label{lst:line:set_eff}\;
		}
	}
	%\end{latin}
\end{algorithm}


%***********************************************************EXPERIMENTS**********************************************************%
\input{vms_info_table}
\vspace{-2mm}
\section{Experimental Results}
\vspace{-1mm}
\label{sec:results}
In this section, we provide comprehensive experiments to evaluate the effectiveness of \techname{}.  
\vspace{-2mm}
\subsection{Experimental Setup}
\vspace{-1mm}
To evaluate the proposed scheme, we conduct our experiments on a real test platform, an HP ProLiant DL380 Generation 5 (G5) server \cite{hp_g5} with four 146GB SAS 10K HP HDDs \cite{hp_hdd} (in RAID-5 configuration), a 128GB Samsung 850 Pro SSD \cite{samsung_ssd} used as the SSD cache, 16GB DDR2 memory from Hynix Semiconductor \cite{hynix_ram}, and 8x 1.6GHz Intel(R) Xeon CPUs \cite{intel_cpu}. 
We run QEMU hypervisor on the \emph{Centos 7} operating system (kernel version 3.10.0-327) and create different VMs running \emph{Ubuntu 15.04} and \emph{Centos 7} operating systems on the hypervisor. %We have also modified the source code of the QEMU (version 2.8.0) to extract and separate the IOs of VMs. 
{The configuration of the device layer is in the default mode where the \emph{request merge} option in the device layer is enabled for a 128-entry device queue size.} 
We have integrated \techname{} with QEMU‌ to enable dynamically partitioning the SSD‌ cache and allocating an efficient cache space and  write policy for each VM. 
\vspace{-2mm}
\subsection{Workloads}
\vspace{-1mm}

We use MSR traces from SNIA \cite{msr}, comprising more than fifteen workloads as real workload traces in our experiments. 
%Table \ref{table:vms_info} reports the information about running workloads on the VMs in the experiments. 
We  run \emph{Ubuntu 15.04} and \emph{Centos 7} operating systems on the VMs and allocate two virtual CPUs, 1GB memory, and 25GB of hard disk for each VM. The experiments are performed with 16 VMs. {Table {\ref{table:workload_def}} shows workloads run on each VM. The SSD‌ cache is shared between VMs. ECI-Cache estimates the most efficient cache size for each VM and partitions the SSD cache space between them based on their running workload IO pattern and request type. We have also implemented one of the state-of-the-art IO caching schemes for virtualized platforms, Centaur {\cite{centaur}} on our test platform. We have executed the same experiments with Centaur. Similar to ECI-Cache, Centaur works based on reuse distance but it does \emph{not} consider request type in reuse distance calculation (TRD). In addition, it does not have any control on unnecessary writes on the SSD cache.}
%the running workloads include hm\underline{\hspace{.05in}}1, mds\underline{\hspace{.05in}}0, proj\underline{\hspace{.05in}}0, prxy\underline{\hspace{.05in}}0, stg\underline{\hspace{.05in}}1, wdev\underline{\hspace{.05in}}0, rsrch\underline{\hspace{.05in}}0, src2\underline{\hspace{.05in}}0, prn\underline{\hspace{.05in}}1, src1\underline{\hspace{.05in}}2, ts\underline{\hspace{.05in}}0, web\underline{\hspace{.05in}}0, usr\underline{\hspace{.05in}}0, rsrch\underline{\hspace{.05in}}2, and mds\underline{\hspace{.05in}}1. 
\vspace{-2.5mm}
\subsection{Cache Allocation to Multiple VMs}
\label{sec:space_alloc}
\vspace{-1mm}
{
To show how ECI-Cache reduces performance, performance-per-cost, and allocated cache space to VMs compared to Centaur, we conduct experiments in two conditions: 1) when the SSD cache capacity is limited, i.e., when the total SSD cache size is less than the sum of the estimated cache spaces for the VMs. In this case, the cache size estimation by ECI-Cache and Centaur may become infeasible and 2) when the SSD cache capacity is unlimited that has enough space to allocate the required and efficient cache space for each VM\footnote{\small{{The experiments of the second case is provided in Appendix \ref{sec:unlimited_ssd}.}}}. In the experiments, VMs are run concurrently and cache space is partitioned across VMs for both ECI-Cache and Centaur schemes (we perform the same, yet separate and independent experiments for both schemes and then compare the results).}

{The experiment is performed on 16 running VMs. An initial cache space equal to $10,000$ cache blocks (block size is equal to 8KB) with WB policy is allocated to each VM. The total SSD cache capacity is 3 million blocks.}
%\vspace{-0.7em}
%\subsubsection{\textbf{Allocation in Limited SSD Cache Space}}
%\label{sec:limited_ssd}
{Cache space is calculated in 10-minute time intervals ($\Delta t$) for both ECI-Cache and Centaur. We select 10-min time intervals to reduce the time overhead of the URD calculation to less than 5\% (this trade-off has been obtained based on the reported URD‌ calculation overheads in Table {\ref{table:time_overhead}} in Appendix {\ref{sec:urd-overhead}}). Reducing the length of the time interval provides more accurate estimations but it also increases the time overhead of the URD‌ calculation.}

{Fig. {\ref{fig:centaur_limited_cs}} and Fig. {\ref{fig:eci_limited_cs}} show how Centaur and ECI-Cache allocate cache spaces for the VMs in the time interval from $t=950~min$ to $t=1,700~min$ of the experiment when the SSD cache capacity is limited to 3 million blocks.
We make two major observations: 1) Centaur becomes infeasible and reduces the allocated cache spaces of the VMs to fit in the existing SSD capacity and 2) ECI-Cache never becomes infeasible since the sum of  estimated cache spaces for the VMs is less than existing SSD capacity.
This is because Centaur estimates larger cache space without considering request type while ECI-Cache estimates much smaller cache space. When the estimated cache space becomes infeasible (here Centaur), Centaur employs an optimization algorithm to find efficient cache sizes which can be fit in the existing SSD cache capacity. To this end, Centaur should allocate smaller cache space and hence achieves less hit ratio than ECI-Cache hit ratio. In these experiments, in-feasibility does not happen for ECI-Cache, however, when ECI-Cache becomes infeasible, Centaur scheme would be infeasible, too. In such cases, both schemes should apply optimization algorithms to reduce the estimated cache spaces in order to fit in the existing SSD cache\footnote{\small{{In Section {\ref{sec:URD}}, we showed that the estimated cache space based on TRD‌ (Centaur)‌ would be greater than or equal to the estimated cache space by URD (ECI-Cache), and hence Centaur should reduce much cache space compared to ECI-Cache. In this case, the performance degradation in Centaur would be greater than performance degradation in ECI-Cache.}}}. We conclude that in infeasible cases, ECI-Cache achieves greater hit ratio and better performance as Centaur does.}
	\input{stacked_limited_TRD}
	%\input{eci_limited_cs}
	\input{limited_16_vms}
	
	{Fig. {\ref{fig:TRD_URD_Hit}} shows the details of allocated cache sizes for each individual VM by both Centaur and ECI-Cache. In addition, this figure shows the IO latency of the VMs for both schemes. During the experiment, the running workloads on the VMs finish one by one (because different workloads have different runtimes) and since VMs with the finished workload generates no more IO requests, ECI-Cache excludes those VMs from cache space partitioning. During the course of the experiment, we retrieve the allocated cache space of such VMs.
		%	Note that the VMs are run concurrently but 
		In order to provide more details, we present the results of each VM separately. The infeasible areas that lead to latency degradation in Centaur are shown by dashed circuits around latency lines. The experiments of Centaur and ECI-Cache are similar, yet separated. We observe that in infeasible states, i.e., when  SSD cache capacity is limited, ECI-Cache improves performance and performance-per-cost by 17.08\% and 30\% compared to Centaur.}
	
\vspace{-2mm}
\subsection{Write Policy Estimation}
\vspace{-1mm}
\label{sec:write_pol_ass}
\input{oper_per_time}
To show how ECI-Cache assigns an efficient write policy for each VM, we conduct experiments based on Algorithm \ref{alg:policy}. We characterize incoming requests from different VMs and calculate the ratio of \emph{WAW} and \emph{WAR} operations for the running VMs. Then, we assign an efficient write polity for the VMs cache. In the experiments, we set the value of $wThreshold$ between 0.2 and 0.9 and achieve different results based on the value of $wThreshold$. Note that we assign RO policy to a VM cache if the ratio of WAW and WAR requests is greater than or equal to $wThreshold$.

Fig. \ref{fig:all-vm-ratio} shows the ratio of different types of the requests in the running workloads. In addition, Fig. \ref{fig:oper-per-time} shows the number of WAW, WAR, RAR, and RAW accesses for the workloads of the running VMs, which are sampled in 10-minute intervals. 
Since the first access (either read or write request) to an arbitrary address within a sequence of I/O requests cannot be classified as either WAW, WAR, RAR, and RAW,
we denoted the first read and write access to an address as \emph{Cold Read} (CR) and \emph{Cold Write} (CW), respectively. 
 Here we set $wThreshold=0.5$. 
{It can be seen that in the first 70-minute interval of web\underline{\hspace{.05in}}1 (running on VM1 as shown in Fig. \ref{fig:web1-oper} and Fig. \ref{fig:all-vm-ratio}), 
neither WAW nor WAR accesses exist  and \techname{} assigns WB policy for the allocated cache. Then at $t=100~min$, WAW operations become dominant and RO policy is assigned to the cache. In VM0, with the running workload of wdev\underline{\hspace{.05in}}0, after about 50 minutes we recognize 77\% of the requests as WAW‌ and the remaining are mostly recognized as RAR operations (shown in Fig. \ref{fig:wdev0-oper} and Fig. \ref{fig:all-vm-ratio}) and thus at $t=50~min$, RO policy is assigned to the cache of VM0 by \techname{}. As shown in Fig. \ref{fig:hm1-oper} and Fig. \ref{fig:all-vm-ratio}, hm\underline{\hspace{.05in}}1 running on VM4 consists of RAR‌ operations (more than 92\%) without any WAR and WAW accesses and RO policy is assigned to this VM.
In time intervals between $t=0$ to $t=500~min$ and $t=610~min$ to $t=1200~min$, more than 86\% of the requests of proj\underline{\hspace{.05in}}0 running on VM6 are CW and WAW operations, and thus \techname{} assigns RO policy to this VM. In the remaining interval ($t=500~min$ to $t=610~min$), WB policy is assigned to this VM. \techname{} assigns RO policy for the VMs such as prxy\underline{\hspace{.05in}} and web\underline{\hspace{.05in}}0 with a large number of WAW‌ and WAR operations which minimizes the number of unnecessary writes into the cache.}
\begin{figure}[!h]
	\centering
	\includegraphics[scale=0.28]{Figures/operations_per_time/all-vms-different-write-percent.pdf}
			\vspace{-2.7em}
	\caption{Ratio of different types of requests in the workloads.}
			\vspace{-1em}
	\label{fig:all-vm-ratio}
\end{figure}

\vspace{-2mm}
\subsection{Performance and Performance-Per-Cost Improvement}
\label{sec:perf_imp}
%completed version 1
\vspace{-1mm}
The results of previous experiments on the proposed test platform show a significant performance and performance-per-cost {(i.e., performance per allocated cache space)} improvement for the running workloads on the VMs as we will show in Fig. \ref{fig:perf-per-cost}. We observed that \techname{} is able to estimate smaller cache space for the VMs compared to Centaur without any negative impact on performance {(i.e., ECI-Cache achieves similar hit ratio while allocating smaller cache space and hence improves performance-per-cost). In addition, \techname{} achieves higher performance compared to centaur in infeasible cases.}
{Cache size estimation in the proposed scheme is based on the URD metric and thus ECI-Cache allocates much smaller cache space to the VMs compared to Centaur. Centaur estimates cache space based on TRD, which does not consider the request type.}
%On the other hand, ECI-Cache works based on URD and estimates efficient cache space by considering only RAR and RAW operations. This scheme reduces the efficient cache space while achieving a similar hit ratio to that obtained by Centaur.

{Fig. \ref{fig:perf-per-cost} shows the achieved performance and performance-per-cost of the VMs by applying Centaur and \techname{} schemes. We observe that allocating cache space based on \techname{} scheme for each VM maximizes the performance and performance-per-cost compared to Centaur. We conclude that \techname{} improves performance and performance-per-cost for the running VMs by 17.08\% and 30\% with decreasing the allocated cache space.}
\begin{figure}[!htb]
	\centering
	\includegraphics[scale=0.28]{Figures/perf-per-cost/perf_and_perf-per-cost.pdf}
		\vspace{-2.2em}
	\caption{{Performance and performance-per-cost achieved by \techname{} and Centaur.}}
		\vspace{-1.3em}
	\label{fig:perf-per-cost}
\end{figure}

\vspace{-2mm}
\subsection{Endurance Improvement}
\vspace{-1mm}
{To show the endurance improvement by \techname{}, we perform experiments by applying a write policy assignment algorithm and show the impact of the proposed scheme on the number of writes and also the performance of the VMs.
Endurance of the SSD is affected by the number of writes committed to it.‌ Write operations on the SSD imposes NAND flash memory writes and increases the P/E cycles count {\cite{ssd-lifetime,tarihi2016hybrid}}. ECI-Cache has a positive impact on the endurance of the SSD because it reduces the committed writes to the SSD. While ECI-Cache can effectively manage the committed writes to the SSD, it has no control on the writes initiated by the garbage collections and wear-leveling algorithms used within the SSD.
Hence, we report endurance improvement of  SSD cache by the reduced number of writes as similar metric is used in previous system level studies such as {\cite{anlj17,elasticQ,huang2016improving,liu2014plc}}.}
%\footnote{\small{Previous system level studies such as {\cite{anlj17,elasticQ,huang2016improving,liu2014plc}} have reported the endurance improvement by reduced number of writes.}}.
Note that the total number of writes for each workload (reported in the experiments) is calculated by Eq. \ref{equ:tot_writes} which includes writes from disk subsystem to SSD and also the writes from CPU to SSD (due to missed read operations).
\begin{equation} 
	Total~Writes=\sum {(CR+CW+WAR+WAW)}
	\label{equ:tot_writes}
\end{equation}
%\vspace{-0.7em}
%\subsubsection{Endurance improvement of URD without applying write policy assignment algorithm}
%Fig. \ref{fig:writes_on_cache} shows the results of the experiments in the first condition. In this experiment, we compare the number of writes into the SSD cache for \techname{} and Centaur where WB is selected as the write policy in both schemes. 
Fig. \ref{fig:writes_on_cache_with_RO} shows the number of writes into the SSD cache and the allocated cache space with Centaur and \techname{}. As this figure shows, \techname{} assigns more efficient write policy for each VM as compared to Centaur. We re-conducted experiments of Sec. \ref{sec:write_pol_ass} and the results demonstrate that by applying RO policy we can reduce the number of writes by 44\% compared to the caches with WB policy. When ECI-Cache applies RO policy on the VMs, only writes due to CRs will be written on the cache. Applying RO policy on the VMs may has a negative impact on the hit ratio of RAW operations by 1.5\%.
%The results also reveal that \techname{} has reduced the number of writes by 65.73\% compared to Centaur. 
%\begin{figure}[!htb]
%	\centering
%	\includegraphics[scale=0.28]{Figures/writes_on_cache/num_of_writes_no_policy.pdf}
%		\vspace{-2.2em}
%	\caption{Committed writes into cache by Centaur and \techname{}.}
%		\vspace{-1em}
%	\label{fig:writes_on_cache}
%\end{figure}

As it can be seen in Fig. \ref{fig:writes_on_cache_with_RO}, applying \techname{} on the VM running hm\underline{\hspace{.05in}}1 has no impact on the number of writes into the cache. This workload mostly consists of RAR and RAW operations where it is necessary to cache referenced data by assigning the WB policy. It is important to note that as presented in Sec. \ref{sec:size_estimation} (shown in Fig. \ref{fig:perf-per-cost}), \techname{} allocates about 50\% smaller cache space to this VM which is calculated based on the reuse distance of RAR and RAW operations by using URD. Similarly, for the VMs running stg\underline{\hspace{.05in}}1, mds\underline{\hspace{.05in}}1, and prn\underline{\hspace{.05in}}1, \techname{} allocates much less cache blocks based on the calculated URD for RAR and RAW operations and assigns the WB policy. Hence, ECI-Cache has no impact on the number of writes into the SSD‌ in such VMs.  For the remaining VMs running workloads such as mds\underline{\hspace{.05in}}0, \techname{} reduces the number of writes by 80\% and the allocated cache space by 25\%. \techname{} achieves 18\% cache size reduction by 90\% reduction in number of writes for ts\underline{\hspace{.05in}}0. For proj\underline{\hspace{.05in}}0, cache size and the number of writes is reduced by 22\% and 46\%, respectively. \techname{} reduces the number of writes for prxy\underline{\hspace{.05in}}0, wdev\underline{\hspace{.05in}}0, rsrch\underline{\hspace{.05in}}0, src2\underline{\hspace{.05in}}0, and src1\underline{\hspace{.05in}}2 by 90\%, 85\%, 87\%, 85\%, and 88\%, respectively. We conclude that \techname{} assigns efficient write policy on the VMs and reduces the number of writes into the SSD‌ cache by 65\%. Write policy is assigned based on the ratio of unnecessary writes due to WAR and WAW operations.
\vspace{-0.7em}
%%%%%Inja:
%\subsubsection{Endurance improvement with applying write policy assignment algorithm}  

\begin{figure}[!htb]
	\centering
	\includegraphics[scale=0.25]{Figures/writes_on_cache/num_of_writes_with_policy_size.pdf}
		\vspace{-1.5em}
	\caption{{Writes into the SSD cache and allocated cache space to the VMs by Centaur and \techname{}.}}
		\vspace{-1em}
	\label{fig:writes_on_cache_with_RO}
\end{figure}
%

%***********************************************************CONCLUSION**********************************************************%
\vspace{-2mm}
\section{Conclusion}
\vspace{-1mm}
\label{sec:conclusion}
In this paper, we presented \techname{}, a hypervisor based I/O caching scheme for a virtualized platform which maximizes the performance-per-cost of the I/O cache by partitioning it between VMs and assigning an small and efficient cache size and write policy. The proposed scheme enhances the endurance of the SSD cache by assigning smaller cache space and also efficient write policy. \techname{} uses an online partitioning algorithm and estimates an efficient cache size for each VM. To do so, \techname{} characterizes the running workloads on the VMs and maximizes the hit ratio of the allocated caches. The proposed scheme allocates the cache space based on the metric of URD‌ which only considers RAR and RAW operations in reuse distance calculation. This metric reduces the cost of the allocated cache space for the VMs by assigning smaller cache size and caching only referenced data.
%only for the VMs with random access pattern with high locality of reference which can take advantage from the high performance of SSD and reduces the number of cache resizing which imposes negative effect on the hit ratio and performance of the allocate cache.
Efficient write policy is assigned for the allocated caches by considering the ratio of WAR and WAW operations of the workload. \techname{} assigns WB policy for the VMs with large size of referenced data due to RAW and RAR operations and RO write policy for the workloads with large size of unnecessary writes due to WAW and WAR accesses. By assigning an efficient cache size and write policy for each VM, \techname{} enhances the performance and performance-per-cost (up to 17\% and 30\%, respectively, compared to recent study \cite{centaur}) and also improves the endurance of the SSD by reducing the number of writes (by 65\%).
\vspace{-2mm}
\sloppypar
\bibliographystyle{plain}
\bibliography{ref}

\appendix
%\input{alg-functions}
\section{Cache Allocation in Feasible State}
\label{sec:unlimited_ssd}
{To show how ECI-Cache and Centaur allocate cache space for the VMs in feasible state, we conduct experiments by applying both schemes in the hypervisor when the SSD cache capacity is unlimited. The experiments are performed on 16 running VMs while an initial cache space equal to $10,000$ cache blocks (block size is equal to 8KB) with WB policy is allocated to each VM. 
Fig. {\ref{fig:TRD_URD_Hit_nl}} shows the allocated cache space by ECI-Cache and Centaur scheme for the VMs separately. In addition, this figure shows the latency of each VM.}

{We observed that for write-intensive workloads with large number of unreferenced data such as stg\underline{\hspace{.05in}}1 in $VM2$, \techname{} allocates significantly smaller cache space (about $14,000$ cache blocks) for caching referenced data while Centaur allocates about 1000X larger cache space to that VM.
The allocated cache space by \techname{} for $VM5$, $VM6$, $VM7$, and $VM12$ in some cases becomes equal to the allocated cache space by Centaur (as shown in Fig. \ref{fig:mds_0}, Fig. \ref{fig:proj_0}, Fig. \ref{fig:prxy_0}, and Fig. \ref{fig:web_0}, respectively). This is because the maximum reuse distance of the workloads is mainly affected by RAR‌ and RAW requests which have access to the referenced data in the cache. 
In Fig. \ref{fig:mds_0} at $t=600~min$, there is a hit ratio drop which is recovered by increasing the allocated cache space by both \techname{} and Centaur. It can be seen that the allocated cache space by \techname{} is much smaller than the allocated space by Centaur. In addition, there is a hit ratio drop in $VM1$ at the first 50-minute interval where increasing the cache space by Centaur scheme does not have any positive impact on the hit ratio. 
This is due to decreasing the locality of references of the requests which mostly include WAR and WAW operations affects the performance of the target VM.
It can be seen that \techname{} does not increase the cache space at this time. At $t=60~min$, \techname{} increases the allocated cache space which results in improving the hit ratio.
\techname{} allocates the minimum cache space for rsrch\underline{\hspace{.05in}}2 which is running on $VM14$ while Centaur allocates much larger cache space (more than $50,000$X). This is because this workload mostly consists of unreferenced read and write operations with poor locality of references. Hence, \techname{} achieves the same hit ratio by allocating much smaller cache space to this workload.
	We conclude that in feasible state, both ECI-Cache and Centaur achieve the same performance while ECI-Cache allocates much smaller cache space for the VMs compared to Centaur.}
	\input{non_limited_16_vms}
	\input{stacked_non_limited_TRD_URD}
	
	{Fig. {\ref{fig:centaur_non_limited_cs}} and Fig. {\ref{fig:eci_non_limited_cs_both}} show cache space allocation for the VMs in the time interval from $t=950~min$ to $t=1,700~min$ by Centarur and ECI-Cache, respectively. It can be seen that in all time intervals, ECI-Cache allocates smaller cache space to the VMs compared to Centaur. We observed that in feasible state (i.e., unlimited SSD cache), ECI-Cache allocates much smaller cache space (29.45\%, on average) and hence reduces performance-per-cost significantly.}
%As it can been in Fig. \ref{fig:TRD_URD_Hit},  the cache space allocated by \techname{} is smaller than the allocated space by Centaur (28.45\%, on average) in all VMs.
%In such condition, the achieved hit ratio by \techname{} with smaller cache size is similar to Centaur. 



\section{URD Overhead and Time Intervals Trade-off  }
\label{sec:urd-overhead}
\input{vms_urd_overhead}
{In this section, we report the average delay of calculating URD for the workloads running on the VMs in our experiments. Based on the delay of URD calculation for the workloads, we show that how we select the intervals of URD calculations in the experiments in order to limit the time overhead of URD calculation (the time that we should wait until URD‌ is calculated). Table {\ref{table:time_overhead}} reports the average time that it takes to calculate URD for each workload. As reported in the table, the maximum time that it takes to calculate URD is about 22.67 seconds, which is reported for the prn{\underline{\hspace{.05in}}}1 workload. In addition, the average time overhead of the URD calculation for all workloads is about 4.82 seconds. We selected 10 min time intervals which is calculated based on maximum URD calculation delay to reduce the time overhead of URD calculation to less than 5\% in our experiments.}
%We have selected intervals of our experiments based on time overhead of URD to limit the overall overhead less than 5\%.


\section{Details of ECI-Cache Size Estimation Algorithm}
\label{sec:size_detail_alg}
{In this section we present Algorithm \ref{alg:size_detail} which provides the
	 details of Algorithm \ref{alg:size}.
	 %In Algorithm \ref{alg:size_detail} we provide the functionality and purpose of the functions.
	 }
{
	The main objective of Algorithm \ref{alg:size_detail} (similar to Algorithm \ref{alg:size}) is to find the most appropriate cache sizes for the running VMs such that the system is able to meet the following conditions: 1) Sum of allocated cache spaces for all VMs  be less than or equal to the total SSD cache capacity. 2) Aggregate latency of all VMs be minimum. 3) Allocated cache space for each VM be less than or equal to the estimated cache space by URD.}
	{This objective is obtained by $calculateEffSize$ function by using  $ObjectiveFunction$. $ObjectiveFunction$ minimizes $diff$ which is the difference between sum of allocated cache spaces for the VMs ($csum$) and the SSD cache capacity ($C$) (i.e., assigns the maximum cache space for each VM). In addition, $ObjectiveFunction$ minimizes the aggregate latency of the running VMs.}
	

\input{size_detail}

==> limited_16_vms_test.tex <==
\begin{figure*}[!t]
	\centering
	\subfloat[VM0: wdev\underline{\hspace{.05in}}0]{\includegraphics[width=.25\textwidth]{Figures/TRD_URD_Hit/wdev_0_TRD_URD_Hit.pdf}%
		\label{fig:wdev0}}
	\hfil
	\subfloat[VM1: web\underline{\hspace{.05in}}1]{\includegraphics[width=.25\textwidth]{Figures/TRD_URD_Hit/web_1_TRD_URD_Hit.pdf}%
		\label{fig:web1}}
	\hfil
	\subfloat[VM2: stg\underline{\hspace{.05in}}1]{\includegraphics[width=.25\textwidth]{Figures/TRD_URD_Hit/stg_1_TRD_URD_Hit.pdf}%
		\label{fig:stg1}}
	\hfil
	\subfloat[VM3: ts\underline{\hspace{.05in}}0]{\includegraphics[width=.25\textwidth]{Figures/TRD_URD_Hit/ts_0_TRD_URD_Hit.pdf}%
		\label{fig:ts0}}
	\hfil
	\subfloat[VM4: hm\underline{\hspace{.05in}}1]{\includegraphics[width=.25\textwidth]{Figures/TRD_URD_Hit/hm_1_TRD_URD_Hit.pdf}%
		\label{fig:hm1}}
	\hfil
	\subfloat[VM5: mds\underline{\hspace{.05in}}0]{\includegraphics[width=.25\textwidth]{Figures/TRD_URD_Hit/mds_0_TRD_URD_Hit.pdf}%
		\label{fig:mds_0}}
	\hfil
	\subfloat[VM6:‌ proj\underline{\hspace{.05in}}0]{\includegraphics[width=.25\textwidth]{Figures/TRD_URD_Hit/proj_0_TRD_URD_Hit.pdf}%
		\label{fig:proj_0}}
	\hfil
	\subfloat[VM7: prxy\underline{\hspace{.05in}}0]{\includegraphics[width=.25\textwidth]{Figures/TRD_URD_Hit/prxy_0_TRD_URD_Hit.pdf}%
		\label{fig:prxy_0}}
	\hfil
	\subfloat[VM8: rsrch\underline{\hspace{.05in}}0]{\includegraphics[width=.25\textwidth]{Figures/TRD_URD_Hit/rsrch_0_TRD_URD_Hit.pdf}%
		\label{fig:rsrch_0}}
	\hfil
	\subfloat[VM9: src1\underline{\hspace{.05in}}2]{\includegraphics[width=.25\textwidth]{Figures/TRD_URD_Hit/src_1_TRD_URD_Hit.pdf}%
		\label{fig:src_1}}
	\hfil
	\subfloat[VM10: prn\underline{\hspace{.05in}}1]{\includegraphics[width=.25\textwidth]{Figures/TRD_URD_Hit/prn_1_TRD_URD_Hit.pdf}%
		\label{fig:prn_1}}
	\hfil
	\subfloat[VM11: src2\underline{\hspace{.05in}}0]{\includegraphics[width=.25\textwidth]{Figures/TRD_URD_Hit/src2_0_TRD_URD_Hit.pdf}%
		\label{fig:src2_0}}
	\hfil
	\subfloat[VM12: web\underline{\hspace{.05in}}0]{\includegraphics[width=.25\textwidth]{Figures/TRD_URD_Hit/web_0_TRD_URD_Hit.pdf}%
		\label{fig:web_0}}
	\hfil
	\subfloat[VM13: usr\underline{\hspace{.05in}}0]{\includegraphics[width=.25\textwidth]{Figures/TRD_URD_Hit/usr_0_TRD_URD_Hit.pdf}%
		\label{fig:usr_0}}
	\hfil
	\subfloat[VM14: rsrch\underline{\hspace{.05in}}2]{\includegraphics[width=.25\textwidth]{Figures/TRD_URD_Hit/rsrch_2_TRD_URD_Hit.pdf}%
		\label{fig:rsrch_2}}
	\hfil
	\subfloat[VM15: mds\underline{\hspace{.05in}}1]{\includegraphics[width=.25\textwidth]{Figures/TRD_URD_Hit/mds_1_TRD_URD_Hit.pdf}%
		\label{fig:mds_1}}
	\hfil
	
%		\vspace{-1.1em}
	\caption{{Allocating cache space to VMs in infeasible state with limited SSD cache capacity (ECI-Cache vs. Centuar).}}
%		\vspace{-1em}
	\label{fig:TRD_URD_Hit}
\end{figure*}

==> size_alg_short.tex <==
\begin{algorithm}[!htb]
	%\SetAlgoNoLine
	\scriptsize
	\DontPrintSemicolon
	\caption{ECI-Cache size allocation algorithm.}
	\label{alg:size}
	\tcc{\textbf{Inputs:} Number of VMs: ($N$), SSD cache size: ($C$), HDD Delay: ($D_{HDD}$), SSD Delay: ($D_{SSD}$)}
	\tcc{\textbf{Output:} Efficient cache size for each VM: ($c_{eff}[1..N]$)}
	\textbf{BEGIN}\;
	Sleep for $\Delta t$\; \label{lst:line:delay} \label{lst:line:sleep}
	\For {$i = 1$ to $N$}
	{
		$URD[i]=calculateURD(VM[i])$\; \label{lst:line:get_urd}
		$size_{urd}[i]=calculateURDbasedSize(URD[i])$\; \label{lst:line:calc_urd_size}
		$csum+=size_{urd}[i]$\; \label{lst:line:csum}
	}
	\tcc{Check the feasibility of size estimation and minimize overall latency for estimated $size_{urd}[1..N]$}
	\If{csum $< C$}
	{\label{lst:line:if1}
		%$LatencyVM_i=$\; \label{lst:line:utility}
		$c_{eff}[1..N]=size_{urd}[1..N]$\;\label{lst:line:feasible_alloc} 
	}\ElseIf{csum $> C$}
	{\label{lst:line:elseif1}
		%$LatencyVM_i=$\; \label{lst:line:utility}
		Create hit ratio function of VMs ($H_i(c)$).\;\label{lst:line:create_hit_func}
		$c_{eff}[1..N]=calculateEffSize(size_{urd}[1..N], C)$\; \label{lst:line:calc_eff_size}
	}
	$allocate(c_{eff}[1..N], VM[1..N])$\; \label{lst:line:allocate}
	\textbf{END}
\end{algorithm}

==> stacked_non_limited_URD.tex <==
\begin{figure}[!h]
	\centering
	\includegraphics[scale=0.25]{Figures/Size_allocation_stacked/URD_stacked_size_first_2000min_sum_edited.pdf}
	\vspace{-1em}
	\caption{Cache allocation for the VMs by ECI-Cache with unlimited SSD cache space.}
	\vspace{-1.5em}
	\label{fig:eci_non_limited_cs}
\end{figure}
